From K.A.M. Tori to Isospectral Invariants and Spectral Rigidity of Billiard Tables

This article is a part of a project investigating the relationship between the dynamics of completely integrable or close to completely integrable billiard tables, the integral geometry on them, and the spectrum of the corresponding Laplace-Beltrami operators. It is concerned with new isospectral invariants and with the spectral rigidity problem for families of Laplace-Beltrami operators with Dirichlet, Neumann or Robin boundary conditions, associated with C^1 families of billiard tables. We introduce a notion of weak isospectrality for such deformations. The main dynamical assumption on the initial billiard table is that the corresponding billiard ball map or an iterate of it has a Kronecker invariant torus with a Diophantine frequency and that the corresponding Birkhoff Normal Form is nondegenerate in Kolmogorov sense. Then we obtain C^1 families of Kronecker tori with Diophantine frequencies. If the family of the Laplace-Beltrami operators satisfies the weak isospectral condition, we prove that the average action on the tori and the Birkhoff Normal Form of the billiard ball maps remain the same along the perturbation. As an application we obtain infinitesimal spectral rigidity for Liouville billiard tables in dimensions two and three. Applications are obtained also for strictly convex billiard tables of dimension two as well as in the case when the initial billiard table admits an elliptic periodic billiard trajectory. Spectral rigidity of billard tables close elliptical billiard tables is obtained. The results are based on a construction of C^1 families of quasi-modes associated with the Kronecker tori and on suitable KAM theorems for C^1 families of Hamiltonians.

==> s10-KAM_parameters_1.tex <==
\section{KAM theorem with parameters}\label{Sec:KAM-parameters}
The  theorems formulated above follow from a KAM theorem with parameters. A complete and very comprehensive proof of it has been given by P\"oschel \cite{Poe1} and Kuksin  \cite{Kuk} in the analytic case. It can be  extended to the case of smooth Hamiltonians using suitable approximation and inverse approximation lemmas. In the case of Gevrey Hamiltonians this has been done in \cite{P4}. The advantage of this approach is that frequencies are separated from action variables which makes it easier to obtain smoothness with respect to them. Moreover, it allows one to prove sharp   H\"older estimates of the transformations putting  the Hamiltonian to a normal form. Here, the normal form of the Hamiltonian is  $N(I;\omega):= \langle\omega,I\rangle$.
The perturbation is a  real valued function $(\theta,I;\omega,t) \mapsto P(\theta,I;\omega,t)$ defined in $\A^n\times \Omega\times [0,a]$, where $\A^n:= \T^n\times B(0,\rho_0)$, $B(0,\rho_0)\subset \R^n$ is the ball centered at $I=0$ with radius $\rho_0\in (0,1]$ and $\Omega$ is a bounded domain in $\R^n$. Hereafter, we assume that
\begin{equation}
P\in C^k\left([0,a];C_0^\infty(\A^n\times\Omega)\right), \quad k\in \{0;1\},
\label{eq:families-of-perturbations}
\end{equation}
i.e. the map
  $t\to P_t:=P(\cdot,t)\in C_0^\infty(\T^n\times B(0,\rho_0)\times \Omega)$ is  $C^k$-smooth on the interval $[0,a]$.  This means that  the support of the function   $(I,\omega) \to P(\theta,I;\omega,t)$ is contained in a fixed  compact subset of  $B(0,\rho_0)\times \Omega$ independent of  $(\theta,t)\in \T^n\times [0,a]$ and 
that the maps  
\[
t\to P_t:=\partial_t^q P(\cdot,t)\in C^j(\T^n\times B(0,\rho_0)\times \Omega), \quad 0\le q\le k, 
\]
are continuous in $t\in [0,a]$ for  $j\in \N$. 
Given  $\ell>0$ and $0<r,\kappa\le 1$, $r\le \rho_0$, ???? we denote by $\|P_t\|_{\ell;r,\kappa}$ the  weighted H\"older norm 
\begin{equation}\label{eq:norm-rho-kappa}
\|P_t\|_{\ell;r,\kappa} := \|P_t\circ \sigma_{r,\kappa}\|_{C^\ell(\sigma_{r,\kappa}^{-1}(\A^n\times\Omega))}
\end{equation}
where  $\sigma_{r,\kappa}$ is  the partial dilation  $\sigma_{r,\kappa}(\varphi,I;\omega):= (\varphi, rI; \kappa \omega)$. The H\"older norms are defined in Section \ref{Sec:ApprLemma} (see also \cite{Poe}). 


Fix  $0<\vartheta_0 < 6(\tau +1)$ 
%such that $2\tau  + \vartheta_0$ is not an integer  
and set 
\begin{equation}
\ell_0:=\tau + 2 + \vartheta_0 ??? \quad \mbox{and} \quad  \ell(m):=  m(\tau + 1)+ \ell_0 \, , \quad m \in \N. 
\label{eq:ell-def}
\end{equation} 


Denote the Hamiltonian vector field associated to  the Hamiltonian $(\theta,I)\to N(I;\omega)=\langle\omega,I\rangle$ by ${\mathcal L}_\omega := X_N(\cdot,\omega)=\langle \omega, \partial/\partial \theta\rangle$.  We consider $C^k$-families, $ k\in \{0;1\}$,  of Hamiltonians $t \to  H_{t,\omega}$, $t\in [0,\delta]$, where
\[
H_{t,\omega}(\theta,I):= H(\theta,I; \omega,t) = N(I;\omega) + P(\theta,I; \omega,t)
\]
and $P$ satisfies \eqref{eq:families-of-perturbations}. Recall that for given $0<\kappa\le 1$ and $\tau>n-1$, the set $\Omega_{ \kappa}=\widetilde D (\kappa,\tau)\cap \overline{\Omega-\kappa}$ consists of all $(\kappa,\tau)$-Diophantine frequencies  $\omega$ in $\Omega$ ($\omega$ satisfies \eqref{eq:sdc1}) such that the distance from $\omega$ to the complement of $\Omega$ in $\R^n$ is greater or equal to $\kappa$. 
The following result is an analogue of Theorem A in \cite{Poe1}. 
\begin{Theorem}\label{Theo:A}
 There exists a  positive constant $\epsilon= \epsilon(n,\tau,\vartheta_0)>0$  depending only  on $n$, $\tau$ and  $\vartheta_0$ such that, for any $a>0$, $0<\kappa<1$, $0<r < \rho_0$ and  any real valued Hamiltonian  $H=N+P$, where $N(I;\omega)=\langle\omega,I\rangle $ and  $P$ satisfies   \eqref{eq:families-of-perturbations}  and the smallness hypothesis
\begin{equation}
   \sup_{t\in [0,a]} \, \| P_t\|_{\ell_0;r,\kappa} \  \le \ \epsilon \kappa r \, ,
\label{eq:smallness-condition3}
\end{equation}
 the following holds.

\vspace{0.3cm}
\noindent
There exist $C^k$ families of maps 
\[
[0,a]\ni t \mapsto \phi_t\in C^\infty(\Omega;\Omega) \quad \mbox{and} \quad [0,a]\ni t \mapsto \Psi_t=(U_t,V_t)\in C^\infty(\T^n \times\Omega;\T^n\times B(0,r)) \ 
\] 
such that   ${\rm supp\,}(\phi_t-{\rm id})\subset \Omega-\kappa/2$, ${\rm supp\,}\big((U_t,V_t)-({\rm id},0)\big)\subset \T^n\times (\Omega-\kappa/2)$,  and 
\begin{enumerate}
\item[(i)]
For each $\omega \in \Omega_\kappa$ and $t\in [0,a]$ the map 
$\Psi_{t,\omega} := \Psi_t(\cdot,\omega):{\T}^n  \rightarrow
 {\T}^n\times B(0,r)$ 
is a smooth embedding, 
$\Lambda_t(\omega)  := \Psi_{t,\omega}({\T}^n)$ is an embedded Lagrangian 
torus invariant  with respect to the Hamiltonian flow of 
$ H_{t,\phi_t(\omega)}(\theta,I) := H(\theta, I; \phi_t(\omega),t)$, and 
\[
X_{H_{t,\phi_t(\omega)}} \circ \Psi_{t,\omega} = 
D \Psi_{t,\omega} \cdot {\mathcal L}_\omega \quad \mbox{on}\  {\T}^n ,  
\]
\item[(ii)]
For any $m\in \N$ there is $C_m>0$ depending only on  $n$, $\tau$, $\vartheta_0$ and $m$, such that
for any $\alpha,\beta\in \N^n$ of length $|\alpha|+|\beta|\le m$ and $0\le q\le k$ the following estimate holds
\[ 
\begin{array}{lrc}
\left|\partial_\theta^{\alpha}(\kappa \partial_\omega)^{\beta}
\partial_t^q(U_t(\theta;\omega) - \theta)\right|\,  + \,
r ^{-1}
\left|\partial_\theta^{\alpha}(\kappa \partial_\omega)^{\beta}\partial_t^q V_t(\theta;\omega)\right|  
+ \kappa^{-1} \left|(\kappa \partial_\omega)^{\beta}
\partial_t^q(\phi_t(\omega) - \omega)\right|
\\    [0.5cm]  
\displaystyle \leq\    C_{m}\, 
 (\kappa  r )^{-1}\, \sup_{0\le p\le q} \,  \sup_{t\in [0,a]} \,\|\partial_t^p P_t\|_{\ell(m);r,\kappa} 
\end{array}
\]
 uniformly in  $(\theta,\omega,t)\in {\T}^n\times \Omega_\kappa\times [0,a]$. 
\end{enumerate}
\end{Theorem}
\begin{Remark}\label{rem:analiticity-t}
If $P$ is analytic with respect to $t$ in  the disc $B(0,a):= \{t\in \C:\, |t|<a\} $  and \eqref{eq:smallness-condition3} holds for $t\in B(0,a)$, then $\Psi$ and $\phi$ can be chosen to be  analytic with respect to $t$ in $B(0,a)$. Moreover, 
for any $\alpha,\beta\in \N^n$ of length $|\alpha|+|\beta|\le m$ and $0<\delta<a$,  the following estimate holds
\[ 
\begin{array}{lrc}
\left|\partial_\theta^{\alpha}(\kappa \partial_\omega)^{\beta}
(U_t(\theta;\omega) - \theta)\right|\,  + \,
r ^{-1}
\left|\partial_\theta^{\alpha}(\kappa \partial_\omega)^{\beta} V_t(\theta;\omega)\right|  
+ \kappa^{-1} \left|(\kappa \partial_\omega)^{\beta} (\phi_t(\omega) - \omega)\right|
\\    [0.5cm]  
\displaystyle \leq\    C_{m,\delta}\, 
(\kappa  r )^{-1}\,  \sup_{t\in B(0,a)} \,\|\partial_t^p P_t\|_{\ell(m);r,\kappa} 
\end{array}
\]
uniformly in  $(\theta,\omega,t)\in {\T}^n\times \Omega_\kappa\times B(0, a-\delta)$, where $C_{m,\delta}>0$ depending only on $n$, $\tau$, $\vartheta_0$,$\delta$, $m$. 
\end{Remark} 
Before starting the proof of Theorem \ref{Theo:A} and Remark \ref{rem:analiticity-t}
we are going to list several comments. 
For each $t\in[0,\delta]$ and $\omega\in \Omega$ 
denote by 
\[
\Phi_{t,\omega}^s := \exp\left(s X_{H_{t,\omega}} \right) ,\ s\in\R,
\]
the flow of the Hamiltonian vector field $X_{H_{t,\omega}}$ of the Hamiltonian $H_{t,\omega}$ and set
\[
g_\omega^s(\theta) = \theta + p(s \omega) ,\ \theta \in\T^n,\ s\in \R, \ \omega\in \Omega,
\] 
where $p:\R^n\to \T^n$ is the canonical projection. 
\begin{Remark}\label{rem:Kronecker} 
The assertion (i) of Theorem \ref{Theo:A} means that for each $\omega\in\Omega_\kappa$ the family $[0,\delta]\ni t \rightarrow \Lambda_t(\omega)$ is a $C^k$ family of Kronecker invariant tori with respect to the flow $\Phi_{t,\widetilde\omega}^s$, where $\widetilde\omega=\phi_t(\omega)$. More precisely, for each $t\in[0,\delta]$, $\omega\in\Omega_\kappa$, and $s\in\R$, the following diagram is commutative 
\[
\displaystyle{\begin{array}{cccl} 
\displaystyle \T^{n}&\stackrel{g_{\omega}^s}{\longrightarrow}&\T^{n}\cr
\downarrow\lefteqn{\Psi_{t,\omega}}& &\downarrow\lefteqn{\Psi_{t,\omega}} \cr
\displaystyle \Lambda_t(\omega)&\stackrel{\Phi_{t,\widetilde\omega}^s}{\longrightarrow}&\Lambda_t(\omega)&  
\end{array} } 
\]
\end{Remark}
\begin{Remark}\label{rem:kam} - \\
1. The Theorem can be obtained  for any $k\in \N$ (then $C_m$ depends on $k$ as well). We suppose here that $ k\in \{0;1\}$ to simplify the proof. 
%If $k$ is sufficiently large or $k=+\infty$ in a neighborhood of $t=0$, then one can consider $t\in\T$ as an additional angle variable and then applying  the Theorem to the Hamiltonian $(\theta,t,I,I_{n+1})\to $.
\\
2. We point out that the constant $\varepsilon>0$ does not depend on the parameters $\kappa$ and $r$, the domain $\Omega$, the annulus $\A^n= \T^n\times B(0,\rho_0)$, the interval $[0,a]$,  as well as on the particular Hamiltonian $P$ satisfying \eqref{eq:families-of-perturbations} and \eqref{eq:smallness-condition3}.\\
3. (i) still holds if $P\in C^k([0,1];C_0^{\ell_0}(\A^n\times\Omega))$. Then $t\to \Psi_{t,\omega}$ is a $C^k$ map with values in $C^{q}(\T^n,\A^n)$,  $q=1+\vartheta_0/6$,  which agrees with the KAM theorem for H\"older Hamiltonians first proved by Moser (cf. \cite{Poe} Theorem A, \cite{Sa-Ze} Theorem 2 and \cite{Sa} Theorem 2). \\
4. (ii) still holds if $P\in C^k([0,1];C_0^{\ell(m)}(\A^n\times\Omega))$.  Better estimates for the derivatives of $U_t$ and $V_t$ could be obtained  following \cite{Poe} as in \cite{P2} and \cite{P3}. Here we prefer the  method given by P\"oschel in \cite{Poe1} since it makes it easier to follow  along the proof the dependence of $\Psi_t$ with respect to the parameters $\kappa$, $r$ and $t\in [0,a]$. 
\end{Remark}
The proof of Theorem \ref{Theo:A} and Remark \ref{rem:analiticity-t} is organized as follows. In Sect. \ref{Sec:kamstep} we prove the KAM Lemma and choose the parameters for the next iteration. The KAM Lemma is close to that of P\"oschel in \cite{Poe1} but one needs additional arguments to estimate the derivatives with respect $t$. To this end we give a complete prove of it skipping some details. 
 In Sect. \ref{Sec:Iteration} we iterate the KAM Step infinitely many times. The choice of the parameters leads to an exponentially converging scheme. Additional efforts are needed to  get convergence for the derivatives with respect to $t$ and to obtain the corresponding estimates in the Iterative Lemma.  In Sect. \ref{Sect.i} we prove (i). In Sect. \ref{Sect.ii} we state a suitable Whitney extension theorem and prove an Inverse Approximation Lemma which implies  (ii).  The Approximation and  Inverse Approximation Lemmas are stated in  Sect. \ref{Sec:ApprLemma}.





==> s12-KAM_iterative_211118.tex <==

\subsection{Iteration}
\label{Sec:Iteration}
\subsubsection{\it Choice of the small parameters.}
\label{Sec:choice-parameters}
As in \cite{Poe1} we are going to iterate the KAM step 
infinitely many times choosing appropriately the parameters $0<s,r,\sigma, 
h,\eta<1$ and so on. Our goal is to get a convergent scheme. We are going
to define suitable strictly decreasing sequences of positive numbers 
$\{s_j\}_{j=0}^\infty$, 
$\{r_j\}_{j=0}^\infty$ and  $\{h_j\}_{j=0}^\infty$, tending to $0$.   
Using the notations introduced in the beginning of Sect. \ref{Sec:kamlemma} we set 
\begin{equation}\label{eq:complex-V}
D_j := D_{s_j,r_j}\, ,\ O_j:=O_{h_j} \, ,\ {\cal V}_j := D_j\times
O_j .
\end{equation}
Set 
\begin{equation}
\label{eq:s}
s_j = s_0 \delta^j\, ,\ \sigma_j = \sigma_0 \delta^j\, ,\ 
s_0 = 5 \sigma_0(1-\delta)^{-1}\in (0,1) \, ,
\end{equation}
where $\delta=\delta(n,\tau,\vartheta) < 1/6$ is given by \eqref{eq:delta+eta}.

Given $m\in \N$, we define an increasing sequence $ \nu(m):=(\nu_j(m))_{j\in\N}$ as follows. We set 
% and we define the sequences $ \nu(m):=(\nu_j(m))_{j\in\N}$ and $ (\ell_j)_{j\le J(m)}$  by
\begin{equation}
\nu_j(m) = \left\{
\begin{array}{lcrr}
\vartheta \quad \mbox{for}\quad j < J(m)  \\[0.3cm]
m(\tau +1) +\vartheta\quad  \mbox{for}\ j \ge J(m),
\end{array}
\right.
\label{eq:secuence-nu-m}
\end{equation} 
where $0<\vartheta <\min (\vartheta/6, 1)$, and 
\begin{equation}
\label{eq:J(m)}
J(m)\ge m(\tau+1)\vartheta^{-1}
\end{equation}
is an integer which will be determined in Sect. \ref{sec:nu+epsilon}.  If $m=0$ we have  $\nu_j(0)=\vartheta$ for any $j\in\N$ and we set $J(0)=0$. 


%\begin{equation}
%\label{eq:nu}
%\left\{
%\begin{array}{lcrr}
%\vartheta = \vartheta_0/6=\nu_0\le \nu_1\le \cdots\,  ,\\[0.3cm]
%\displaystyle 2(\nu_j-\nu_0) \, \le \, \Sigma_{q=0}^{j-1}  \, \nu_q,  \quad j\ge 1, \\[0.3cm]
%\nu_j   \le C(n,\tau)(j +1),  \quad j\ge 1, 
%\end{array}
%\right.
%\end{equation}
%where $C(n,\tau)\ge 1$ may depend only on $n$ and $\tau$. 
%The first inequality will be used to obtain \eqref{eq:E-and-eta} for $j\ge 1$. 
Taking into account  \eqref{eq:r-and-s},  \eqref{eq:delta+eta} and  \eqref{eq:E+}, we define the sequences  $\{r_j\}_{j\in\N}$, $\{\eta_j(m)\}_{j\in\N}$  and   $\{E_j(m)\}_{j\in\N}$ as follows.
Fix $0<r<1$, $0<r_0=s_0r<1$ and $\eta_0^2 =\delta^{\tau +2+2\vartheta} $,   and set
\begin{equation}
\label{eq:r}
\left\{
\begin{array}{lcrr}
\displaystyle \eta_j=\eta_j(m):= \delta^{\nu_j-\nu_{j-1} }\eta_{j-1} =\delta^{\nu_j-\nu_{0} }\eta_{0} =\delta^{\nu_j+ (\tau+2)/2} ,  \quad j\ge 1, \\[0.3cm]
\displaystyle r_j := \delta  r_{j-1}=r_0\delta^{j}, 
\end{array}
\right. 
\end{equation}   
and 
\begin{equation}
\label{eq:E}
E_j =E_j(m):= \delta^{2\nu_{j-1}} E_{j-1}= \delta^{2\nu_0 + \cdots +2\nu_{j-1}}E_0, \quad j\ge 1 . 
\end{equation}
%To indicate the dependence of $E_j$ of the sequence $\nu=(\nu_j)_{j\in\N}$, we write $E_j=E_j(\nu)$. 
Take the positive number $E_0=E_0(n,\tau,\vartheta_0)$ sufficiently small so that $ E_0< \eta_0^2= \delta^{\tau +1+2\vartheta} $. 
The inequality  \eqref{eq:J(m)} implies that 
$$
\nu_j-\nu_0\le \nu_0 + \cdots + \nu_{j-1}, \quad j\ge 1.
$$
Indeed, if $m=0$ then $\nu_j=\nu_0= \vartheta>0$ for each $j$. Let $m\ge 1$. 
For $j<J(m)$  have $\nu_j=\nu_0= \vartheta>0$ and for $j\ge J(m)$ we get 
$$
\nu_j-\nu_0 = m(\tau+1)\le J(m)\vartheta \le j\vartheta \le \nu_0 + \cdots + \nu_{j-1}
$$ 
which yields  the inequality for any $m\in \N$ and $ j\in \N$. 
Hence, 
\begin{equation}\label{eq:E-eta-j}
0<E_j<\eta_j^2\le \eta_0^2<1/64, \quad j\in\N.
\end{equation}
Taking into account   \eqref{eq:def-of-epsilon},  we put
\begin{equation}
\label{eq:epsilon}
\varepsilon_j:=  \hat\varepsilon \kappa  r_j\sigma_j^{\tau + 1}  E_j = 
  \hat\varepsilon \kappa  r_0\sigma_0^{\tau + 1}  E_0 \delta^{q_j}, 
\end{equation}
where $q_0=0$ and 
\[
q_j:= j(\tau +2) + 2(\nu_0+\cdots+\nu_{j-1}),\quad  j\ge 1.
\] 
The parameter  $0<\hat\varepsilon \le 1 $   will be  chosen later. 
Finally, taking into account \eqref{eq:K} we set
\begin{equation}
\label{eq:h-and-K}
K_j= \sigma_j^{-1}\ln^2(\sigma_j)\quad \mbox{and}\quad  2 h_j = \kappa K_j^{-\tau-1} =\kappa \big(\sigma_j/\ln^2(\sigma_j)\big)^{\tau+1},\  j\in\N.
\end{equation}
We have
\begin{equation}
\label{eq:recurrence-relations}
\displaystyle s_{j+1} = s_j - 5\sigma_j,\ 
\sigma_j = 5^{-1}(1-\delta)s_j \quad \mbox{and}\quad h_{j+1}/h_j< \delta^{\tau+1}< 1/4
\end{equation}
in view of \eqref{eq:h+} and \eqref{eq:s}. Moreover, $ s_{j+1}-5s_{j+1}=\delta (s_{j}-5s_{j})$ and  \eqref{eq:constants} holds for each $j\in\N$. 
We are going to show that  hypothesis (a) - (d) of Proposition \ref{Prop:kam-step} and Remark  \ref{Rem:estimates} are satisfied for any $j\in \N$. More generally, we have the following 
\begin{Lemma}\label{Lemma:a b and c}  
	There exist  positive constants  $\widetilde E_0(n,\tau,\vartheta_0)<1/64$  and $\widetilde \sigma_0(n,\tau,\vartheta_0)<(1-\delta)/5$, depending only on $n,\tau$ and $\vartheta_0$, and   such that \eqref{eq:constants}, \eqref{eq:sigma-eta}, \eqref {eq:E-eta-j},  and the hypothesis (a)-(d)  hold for any $j\in \N$ provided that    $0<E_0\le \widetilde E_0$ and  $0<  \sigma_0 \le \widetilde \sigma_0$ . 
\end{Lemma}
\noindent
{\em Proof.}  We have already obtained \eqref{eq:constants} and \eqref {eq:E-eta-j} for $j\in\N$. Choosing $E_0 \le \widetilde E_0(n,\tau,\vartheta_0)\le c_0$ we get (a) for any $j\in\N$, while \eqref{eq:h-and-K} implies (c). 
On the other hand, (b)  holds if $E_j$ and $\sigma_j$ verify  
\eqref{eq:condition-b}. Since $0<\delta < 1$ and $\vartheta=\nu_0\le \nu_1\le \cdots$,  we get from \eqref{eq:s}  and \eqref{eq:E} that the sequence $\big(\ln^{2}(\sigma_j)E_j\big)_{j\in\N}$ is decreasing, which implies  b). Moreover, (d) holds since $K_j \sigma_j  =\ln^2(\sigma_j)>1$. 

It remains to prove \eqref{eq:sigma-eta}. Consider the function
\[ f(\sigma):= \sigma^{-n} \exp(-K\sigma) = \sigma^{-n} \exp\left(-\ln^2(\sigma)\right). \]
It is strictly increasing in an  interval $\big(0, \exp(-n/2)\big]$. 
 %We have 
 %\[  f'(\sigma) = \sigma^{-1} f(\sigma)\big(\vartheta (\tau+1)^{-1}\sigma^{-\vartheta (\tau+1)^{-1}}-n\big),\] 
 We take  $\widetilde \sigma_0$ in that interval so  that 
 $f(\widetilde\sigma_0)\le \eta_0^2= \delta^{ \tau+2+2\vartheta } $, which implies \eqref{eq:sigma-eta} for $j=0$. Suppose now that $j\ge 1$. 
 Notice that 
 $$\nu_j(m)\le (j+1)\vartheta < 2(j+1)(\tau+1)$$ 
 for $j\in\N$ in view of \eqref{eq:secuence-nu-m} and \eqref{eq:J(m)}. For $j\ge 1$, this implies 
 \[  
 f(\sigma_j) \eta_j^{-2} < \sigma_j^{-n} \exp\left(-\ln^2(\sigma_j)\right)\delta^{-4(j+2)(\tau+1)}\le \sigma_j^{-n-12(\tau+1)}\exp\left(-\ln^2(\sigma_j)\right) \le 1
 \]
 for  $0<\sigma_0\le \tilde \sigma_0(n,\tau,\vartheta)$, taking  $\tilde \sigma_0$ sufficiently small. 
This yields \eqref{eq:sigma-eta} for any $j\in\N$.
\finishproof 

\noindent
Using \eqref{eq:b-again},  \eqref{eq:secuence-nu-m}, and  \eqref{eq:E}, we get as in the proof of b) the inequality
\begin{equation}
\frac{\varepsilon_j}{r_jh_j} \le 2 \ln^{2\tau +2}(\sigma_j)E_j   \le  
 C(n,\tau,\vartheta) \sigma_j^{\vartheta}E_0 .
\label{eq:epsilon-by-rh}
\end{equation}
We fix   $0<\sigma_0< (1-\delta)/5$ 
ones forever by 
\begin{equation}\label{eq:sigma-0}
0<\sigma_0 = \min\big(\frac{1}{37}, \widetilde \sigma_0(n,\tau,\vartheta\big).
\end{equation}
The choice of $\sigma_0 $ is motivated by \eqref{eq:u-0}. 
\begin{Remark}\label{rem:dependence-of-m}
The sequences of $\eta_j=\eta_j(m)$ and weighted errors $E_j=E_j(m)$ depend on the choice of $m\in\N$, but $\sigma_j$, $r_j$, $h_j$ and $K_j$ do not depend on $m$. 
\end{Remark}

\subsubsection{\it Analytic smoothing of $P_t$.}
\label{Sec:analytic-smoothing}
The Hamiltonian $P_t$ is not analytic and one can not apply directly the KAM step to it. We are going to approximate it by real analytic functions. To this end 
we recall some facts about the analytic smoothing technique in Section \ref{Sec:ApprLemma}. 
We are going to apply the Approximation Lemmas \ref{Lemma:approximation-lemma} and   \ref{Rem:approximation} to the real valued Hamiltonian  $P\in C^k\left([0,a];C_0^L(\A^n\times\Omega)\right)$, where $a>0$, $0<L\le \infty$ and the partial dilation is given by $\sigma_{r,\kappa}(\theta,I;\omega)=(\theta,rI;\kappa\omega)$. 
Set  
\begin{equation}
\label{eq:u-v-w-sequences}
u_j = u_0 \delta^j \ ,\ v_j = w_0 \delta^{j}  =r u_j, \    \ w_j = \kappa u_j ,\ j\in\N,
\end{equation}
where 
\begin{equation}
\label{eq:u-0}
0<u_0= 6 s_0= 30 (1-\delta)^{-1} \sigma_0 \le 36 \sigma_0< 1,\ w_0=6r_0=6s_0 r<1,
\end{equation}
the small parameter $0<\delta=\delta(n,\tau,\vartheta_0)<1/6$ is given by \eqref{eq:delta+eta} and $\sigma_0=1/37$. Note that
\[
\sup\{s_j/u_j,  r_j/v_j,h_j/w_j\} \le \frac{1}{6}   ???????
\]
for $j\in\N$. 
Let us denote by  ${\cal U}_j$ the complex strips  in  
${\C}^n/{\Z}^n \times  {\C}^n \times  {\C}^n$ consisting of all
$(\theta, I; \omega)$ such that 
\begin{equation} 
|{\rm Im\, } \theta| < u_j\, ,\  
|{\rm Im\, } I| <  v_j\, ,\ 
|{\rm Im\, } \omega| <  w_j\, 
\label{eq:u-v-w}
\end{equation}
and by 
$A({\cal U}_j)$ the set of all real-analytic  bounded functions in ${\cal
	U}_j$ equipped with the sup-norm $|\cdot|_{u_j,v_j,w_j}$. 
Let 
\begin{equation}\label{eq:approximation-of-P}
P_t^j:= S_{u_j,v_j,w_j}P_t\, ,\quad j\in\N.
\end{equation}
This is  a $C^k$ family with respect to $t\in[0,1]$ of real analytic  functions in ${\C}^n/{\Z}^n \times  {\C}^n \times  {\C}^n$. Lemma \ref{Rem:approximation} with $\rho_0=u_j$,  $\tilde\rho_0=u_{j-1}=\delta^{-1} u_j$ and $a=(r,\kappa)$, yields  the estimate 
\[
\left|\partial_t^p(P_t^{j} -  P_t^{j-1} )  \right|_{u_j,v_j,w_j} \le C_0 u_{j-1}^{\ell}\|\partial_t^p P_t\|_{\ell;r,\kappa} =C u_j^{\ell}\|\partial_t^p P_t\|_{\ell;r,\kappa}
\]
for each finite $\ell$, $0\le \ell\le L$ and $0\le p\le k$, where $C=C(\ell,n,\tau, \vartheta_0)=C_0(n,\ell)\delta^{-\ell}$ is a positive constant depending only on $\ell,n,\tau, \vartheta_0$. Moreover, 
\[
\left|\partial_t^p P_t^{0}  \right|_{u_0,v_0,w_0} \le C_0 \|\partial_t^p P_t\|_{0} \le \widetilde C u_0^{\ell}\|\partial_t^p P_t\|_{\ell;r,\kappa} 
\]
where $\widetilde C = C_0(n)u_0^{-\ell}$. The positive constant $C_\ell := \max(c, \widetilde c)=C_\ell(n,\tau,  \vartheta_0)$ depends only on $\ell, n,\tau$ and $\vartheta_0$. 
Hence, 
\begin{equation}
\label{eq:approximation-estimates1}
\left|\partial_t^p P_t^{0}    \right|_{u_0,v_0,w_0} \le \widetilde\varepsilon_{\ell,0,p}\quad \mbox{and} \quad \left|\partial_t^p P_t^{j} -  \partial_t^p P_t^{j-1}   \right|_{u_j,v_j,w_j} \le \widetilde\varepsilon_{\ell,j,p} \quad \mbox{for} \quad j\ge 1
\end{equation}
for any finite $\ell$, $0\le \ell\le L\le \infty$, where 
\begin{equation}
\label{eq:approximation-estimates2}
\widetilde\varepsilon_{\ell,j,k}\, :=\,  C_\ell u_j^{\ell}\sum_{p=0}^k \sup_{0\le t \le a} \|\partial_t^p P_t\|_{\ell;r,\kappa} 
\end{equation}
and $C_\ell=C(\ell,n,\tau,\vartheta_0)>0$ depends only on $\ell$, $n$, $\tau$ and $\vartheta_0$. 

We would like to deal with $P^{j}$ at the $j$-th iteration putting $P^{j}-P^{j-1}$ in the error term. 
To this end   we need for $0\le p\le k$ the following inequalities
\begin{equation}
\label{eq:approximation6-0}
\left|\partial_t^p P_t^{0}    \right|_{u_0,v_0,w_0} \le \frac{\varepsilon_{1}}{2} \quad \mbox{and} \quad \left|\partial_t^p P_t^{j} -  \partial_t^p P_t^{j-1}   \right|_{u_j,v_j,w_j} \le \frac{\varepsilon_{j+1}}{4} \quad \mbox{for} \quad j\ge 1. 
\end{equation}
These inequalities will be obtained in Sect. \ref{sec:nu+epsilon}, choosing appropriatelly the sequence $\nu$ and the small constants $\epsilon$ and $\hat{\varepsilon}$. 
\subsubsection{\it Iterative Lemma.}
\label{Sec:iteration-lemma}
We are ready to make the iterations. Consider the real analytic in 
${\cal U}_j$ Hamiltonian  
\[
H_t^j(\varphi,I;\omega)= H^j(\varphi,I;\omega,t) := N_0(I;\omega) + P_t^j(\varphi,I;\omega),
\] 
where 
$ N_0(I;\omega) := \langle \omega,I\rangle$ and ${\cal U}_j$ is defined by \eqref{eq:u-v-w}.   Set $\widetilde D_{j}:= D_{s_j/2, r_j/2}$, $\widetilde O_{j}:=O_{h_j/2}$ and denote by ${\cal U}_j^0$ the subset of 
${\C}^n/{\Z}^n \times  {\C}^n \times  {\C}^n$ consisting of all
$(\theta, I; \omega)$ such that 
\[
|{\rm Im\, } \theta| < \frac{1}{2}u_j\, ,\  
|{\rm Im\, } I| < \frac{1}{2} v_j\, ,\ 
|{\rm Im\, } \omega| <  \frac{1}{2} w_j\, .
\]
One can easily check that $2s_j < u_j$, $2r_j < v_j$, and $2h_j <w_j$, which yields 
$ D_j\times O_j\subset {\cal U}_j^0$. 
Then we  obtain
\[
D_{j+1}\times O_{j+1} \subset \widetilde D_{j}\times \widetilde O_{j} \subset  D_j\times O_j \subset {\cal U}_j^0\subset {\cal U}_j
\]
since $s_{j+1}/s_{j},\, r_{j+1}/r_{j}, \, h_{j+1}/ h_{j}\le \delta <1/2$. 
For any $j\in {\N}$,
let us  denote by ${\cal D}_j$ the class of  real-analytic 
diffeomorphisms 
\[
{\cal F}_{j}: D_{j+1}\times  O_{j+1} \to \widetilde D_{j}\times  \widetilde O_{j}
\]
of the form  
\begin{equation}
\label{eq:transformation-F}
{\cal F}_j(\theta,I;\omega)\ =\  (\Phi_j(\theta,I;\omega),\phi_j(\omega))\, ,\ 
\Phi_j(\theta,I;\omega)\ =\ (U_j(\theta;\omega),V_j(\theta,I;\omega))\, ,                            
\end{equation}
where $V_j(\theta,I;\omega)$ is affine  linear  with respect to $I$,  
and  
$(\theta, I) \to \Phi_j(\theta,I;\, \omega)$ 
is a canonical transformation   for  any fixed $\omega$. To simplify the notations we
denote the sup-norm of functions $f:D_{j}\times  O_{j}\to \C$ by $|f |_j=|f|_{s_j,r_j,h_j}$. Obviously, 
$D_{j}\times  O_{j} \subset {\cal U}_j$. Fix $k\in \{0;1\}$.


 
\begin{Prop}[Iterative Lemma] \label{Prop:IterativeLemma} 
Let  $P^j\in C^k([0,a], {\mathcal A}({\mathcal U}_j))$, $j\in \N$,  be a $C^k$ family of  real analytic Hamiltonians in ${\mathcal U}_j$ satisfying \eqref{eq:approximation6-0} and $H^j=N_0+P^j$.  
Then for each $j\in \N$ there is a normal form 
$N_j(I;\omega,t) 
= e_j(\omega,t) + \langle \omega,I\rangle$ and  a $C^k$ family of  real analytic 
transformations 
\begin{equation}
{\cal F}^j\in  C^k([0,a], {\mathcal A}( D_{j}\times O_{j}, (D_0\times O_0) \cap {\cal
U}_{j}^0)), \quad {\cal F}^j_t = {\cal F}^j(\cdot,t),
\label{eq:range-F-0}
\end{equation}
such that
\begin{enumerate}
	\item 
${\cal F}^0 = {\it
id}$ and  ${\cal F}^{j+1}_t = {\cal F}_{t,0}\circ\cdots\circ {\cal F}_{t,j}$ where 
\begin{equation}
{\cal F}_j\in C^k([0,a], {\mathcal A}( D_{j+1}\times O_{j+1}, \widetilde D_{j}\times \widetilde O_{j}))\quad \mbox{and}\quad {\cal F}_{t,j}(\cdot,t):={\cal F}_{j}(\cdot,t)\in {\cal D}_j, \quad j\ge 0;  
\label{eq:range-F}
\end{equation}
	\item 
$H^j\circ {\cal F}^{j+1} = N_{j+1} + R_{j+1}$ and  
$\displaystyle | \partial_t^p R_{j+1} |_{j+1}  \le \varepsilon_{j+1}/2$  for $0\le p\le k$;
	\item The following estimates hold
\begin{equation} 
\displaystyle  |\overline{W}_j \partial_t^p({\cal F}_{t,j} - {\rm id} )|_{j+1} \ +\ 
|\overline{W}_j \partial_t^p(D {\cal F}_{t,j} - {\rm Id} )
\overline{W}_j^{\, -1}|_{j+1} \ <   
 \frac{C_0 \varepsilon_j}{r_jh_j} , 
                         \label{eq:estimates-F1} 
\end{equation}
\begin{equation} 
\displaystyle  |\overline{W}_0\partial_t^p({\cal F}^{j+1}_t - {\cal F}^j_t)|_{j+1} \, 
< \frac{C_0 \varepsilon_j}{r_jh_j} ,
                          \label{eq:estimates-F2} 
\end{equation} 
for $0\le p\le k$ and uniformly with respect to $t\in [0,a]$,  where $C_0 =C_0(n,\tau,\vartheta_0)>0$,   $D {\cal F}^{j}_t$
stands for the Jacobian of ${\cal F}^{j}_t$ with respect to
$(\theta,I;\omega)$, and \\
$\overline{W}_j = {\rm diag}\, \left({\sigma_j}^{-1}{\rm Id}, 
{r_j}^{-1}{\rm Id},{h_j}^{-1}{\rm Id}\right)$.   
\end{enumerate}
\end{Prop} 
{\em Proof}. For $k=0$ the proof is similar to that of the Iterative Lemma in 
\cite{Poe1} and it is done in \cite{P4} in the case of Gevrey Hamiltonians independent of $t$. Additional efforts are required for the proof of the estimates \eqref{eq:estimates-F1} and \eqref{eq:estimates-F2} in the case when $p=k=1$.  


Consider firstly the Hamiltonian $H^0= N_0+P^0$. It satisfies the hypothesis of Proposition \ref{Prop:kam-step} in $D_0\times O_0$ for $t\in [0,a]$ in view of \eqref{eq:approximation6-0} and Lemma \ref{Lemma:a b and c}. 
Hence, applying the KAM step to the Hamiltonian $H^0$  we find 
${\cal F}^{1} = {\cal F}_{0}$ such that 
$H^0 \circ {\cal F}^1 =  N_1 + R_{1}$, where $R_{1}(\cdot,t)$ is real analytic
in $D_1\times O_1$ and $| \partial_t^p R_{1}(\cdot,t)|_{1} \leq \varepsilon_1/2$. Moreover, \eqref{eq:estimates-F1} holds for $j=0$. 



Given $j\ge 1$ we suppose that the Proposition holds for all indexes $0\le l\le j-1$. We are going to prove it for $l=j$. We are looking for a transformation 
${\cal F}^{j+1} = {\cal F}^{j}\circ {\cal
	F}_{j}$, where ${\cal F}_j$  belongs to ${\cal D}_j$. 
By the inductive
assumption we have 
\[
H^{j-1} \circ {\cal F}^{j} = N_j + R_{j},
\] 
where 
$N_j(I;\omega,t) = e_j(\omega,t) + \langle \omega, I\rangle$, $R_{j}(\cdot,t)$ is real analytic   in $D_j\times
O_j$, and  $ |  \partial_t^p R_{j} (\cdot,t)|_{j}  \leq  \varepsilon_{j}/2$. 
Then we write  
$$
H^j \circ {\cal F}^{j+1} = (N_0 + P^{j-1})\circ {\cal F}^{j+1} + 
(P^{j} - P^{j-1})\circ {\cal F}^{j+1} 
$$
$$
= \left(H^{j-1} \circ {\cal F}^{j}\right)\circ {\cal F}_{j} 
+ (P^{j} - P^{j-1})\circ {\cal F}^{j+1} 
$$
$$
= \left(N_j + R_{j}+ (P^{j} - P^{j-1})\circ {\cal
F}^{j}\right) \circ {\cal F}_{j} .     
$$
Consider the Hamiltonian $\widetilde H_j= N_j+ R_j + (P^{j} - P^{j-1})\circ {\cal
	F}^{j}$   in $D_j\times O_j$ for $t\in [0,a]$ and set $R_j^1= (P^{j} - P^{j-1})\circ {\cal
	F}^{j}$. Using \eqref{eq:approximation6-0}  we get
\[
|(P_t^{j} - P_t^{j-1})\circ {\cal F}^{j}(\cdot,t)|_{j} 
\leq |P_t^{j} - P_t^{j-1}|_{{\cal U}_{j}^0} 
\leq \frac{\varepsilon_{j}}{4} .
\]
On the other hand, using \eqref{eq:approximation6-0},  \eqref{eq:range-F-0}  and \eqref{eq:estimates-F1} we obtain 
\[
|\partial_t((P_t^{j} - P_t^{j-1})\circ {\cal F}^{j}(\cdot,t))|_{j} \le 
 |\partial_t P_t^{j} - \partial_t  P_t^{j-1}|_{{\cal U}_{j}^0} + |(D(P_{j} - P_t^{j-1})\circ {\cal F}^{j} (\cdot,t))\, \partial_t {\cal F}^{j}(\cdot,t)|_{j} .
\]
The firs term of the right hand side is estimated by $\frac{\varepsilon_{j}}{4} $ in veiw of \eqref{eq:approximation6-0}. Using \eqref{eq:range-F-0} we estimate the second one by
\[
|D(P_t^{j} - P_t^{j-1})W_j^{-1}|_{{\cal U}^0_{j}}\, |W_j\partial_t {\cal F}^{j}(\cdot,t)|_{j} 
\]
(here we consider $\overline W_{j}$ as a linear operator acting on  $\C^{3n}$). 
Now Cauchy estimates (see Remark \ref{Rem:Cauchy} ), \eqref{eq:u-v-w-sequences} and \eqref{eq:approximation6-0} yield 
\begin{equation}\label{eq:Cauchy-P}
\begin{array}{rcll}
\displaystyle \left|D(P_t^{j} - P_t^{j-1})W_j^{-1}\right|_{{\cal U}^0_{j}}  = \left|\left(s_j\nabla_{\theta}, r_j\nabla_{I},h_j\nabla_{\omega}\right)(P_t^{j} - P_t^{j-1})W_j^{-1}\right|_{{\cal U}^0_{j}} \\ [0.4cm]
\le \displaystyle\sqrt{\left({\frac{2s_j}{u_j}}\right)^2 + \left({\frac{2r_j}{v_j}}\right)^2+\left({\frac{2h_j}{w_j}}\right)^2 } |P_t^{j} - P_t^{j-1}|_{{\cal U}_{j}} 
\le \displaystyle 2\sqrt{3}\times \frac{1}{6} \times\frac{\varepsilon_{j}}{4} <  \frac{\varepsilon_{j}}{4} . 
\end{array}
\end{equation}
Moreover, \eqref{eq:estimates-F1} and \eqref{eq:epsilon-by-rh} imply that $|W_j\partial_t {\cal F}^{j}(\cdot,t)|_{j} \le 1$. Finally, we obtain 
$$
|\partial_t^p R_j + \partial_t^p R_j^0|_{j} < \varepsilon_{j}\, , \quad p\in \{0;1\}. 
$$
We apply the KAM step  - Proposition \ref{Prop:kam-step} - to the $C^k $ family of
Hamiltonians $\widetilde H_j$. 
 Using Remark \ref{Rem:Cauchy}, \eqref{eq:new-error2} and  \eqref{eq:epsilon-by-rh} as well,  
we find a $C^k$ family of real-analytic maps 
\[
{\cal F}_{j}(\cdot,t): 
D_{j+1} \times O_ {j+1} \to  \widetilde D_j \times \widetilde O_j
\]
which belongs to the class ${\cal D}_{j}$, satisfies \eqref{eq:estimates-F1} and such that 
$(N_j + R_{j})\circ {\cal F}_{j} = N_{j+1} + R_{j+1}$, where 
$$ 
|\partial_t^p R_{j+1}|_{j+1} \leq 
 \frac{1}{2} 
 \hat\varepsilon_j  \kappa r_{j+1}\sigma_{j+1}^{\tau +1}
E_{j+1}   \le \frac{1}{2} 
 \hat\varepsilon_{j+1}  \kappa r_{j+1}\sigma_{j+1}^{\tau +1}
E_{j+1} = \frac{\varepsilon_{j+1}}{2} .  
$$ 
%Moreover,  ${\cal F}_{j}$ satisfies
%(\ref{eq:estimates-F1}) in view of Remark \ref{Rem:estimates} and Lemma \ref{Lemma:a b and c}. ????? 
We are going to show that 
\begin{equation}
{\cal F}^{j+1} : D_{j+1} \times O_{j+1}\  \longrightarrow \ {\cal
U}_{j}^0 .
                                  \label{eq:map-F}
\end{equation}
%This implies
%$$
%|\partial_t^p(P_{j} - P_{j-1})\circ {\cal F}^{j+1}|_{j+1} 
%\leq |\partial_t^p(P_{j} - P_{j-1})|_{{\cal U}_{j}} 
%\leq \frac{\varepsilon_{j+1}}{2} ,   
%$$
%and  we obtain  
%$H^j\circ {\cal F}^{j+1} = N_{j+1} + R_{j+1}$, where
%$|\partial_t^p R_{j+1}|_{j+1} \le \varepsilon_{j+1}$ for $0\le p\le k \le 1$. 
To prove (\ref{eq:map-F}) we estimate the norm of the linear operator  $W_q \overline W_{q+1}^{\, -1}$. We have
\[
|\overline W_q \overline W_{q+1}^{\, -1}| = 
\sup \left\{s_{q+1}/s_q,r_{q+1}/r_q ,h_{q+1}/h_q
\right\} =  s_{q+1}/s_q = \delta, 
\]
since $r_{q+1}/r_q \le \delta ^{\tau +1} < \delta$ and $h_{q+1}/h_q \le 
\delta ^{\tau +1} < \delta$ for any $q\in {\N}$ by \eqref{eq:r} and \eqref{eq:recurrence-relations}. 
Recall that  $\delta$ and $E_0$ depend only on $n$, $\tau$ and $\vartheta_0$. 
Then using \eqref{eq:epsilon-by-rh} and  (\ref{eq:estimates-F1}), 
we  estimate the Jacobian of ${\cal
F}^{j+1}$ in $D_{j+1}\times O_{j+1}$ as follows (see also \cite{Poe1})
\[
\begin{array}{rcl}
\left|\overline W_0 D{\cal F}^{j+1}\overline W_{j}^{\, -1}\right|_{j+1}
\,  &=& \, 
\left|\overline W_0 D ({\cal F}_{0}\circ \cdots \circ 
{\cal F}_{j})\overline W_{j}^{\, -1}\right|_{j+1}       \\[0.3cm]
&\le& \displaystyle \prod_{q=0}^{j-1}
\left(\left|\overline W_q D {\cal F}_{q}\overline W_q ^{\, -1}\right|_{q+1}\, 
\left|\overline W_q \overline W_{q+1}^{\, -1}\right|\right)
\left|\overline W_j D {\cal F}_{j}\overline W_{j}^{\, -1}\right|_{j+1}\, 
 \\[0.3cm]
&\le& \displaystyle\delta^{j}  \prod_{k=0}^\infty\, 
\left(1 +  \frac{C \varepsilon_k}{r_kh_k} \right) \le \displaystyle \delta^{j} 
\exp\left(\sum_{k=0}^\infty 
 \frac{C \varepsilon_k}{r_kh_k}\right)\\[0.3cm] 
 &\le& \displaystyle  \delta^{j}\exp\left(C(1-\delta^{\vartheta/2}) ^{-1}E_0^{1/2}\right) , 
\end{array}
\]
where $C=C(n,\tau,\vartheta_0)$ stands for different positive constants depending only on $n$, $\tau$ and $\vartheta_0$. 
Choosing the parameter $E_0 =E_0(n,\tau,\vartheta_0)>0$ sufficiently small 
we obtain  
\begin{equation}
 \left|\overline W_0 D{\cal F}^{j+1}\overline W_{j}^{\, -1}\right|_{j+1}  <  \sqrt{3}\delta^{j}, \quad j\in \N.
 \label{eq:estimate-differential-F}
\end{equation}
Set 
\[
z=(\theta,I,\omega) =x +iy\in D_{j+1}\times  O_{j+1},
\]
where  $x$
and $y$ are respectively the real and the imaginary part of $z$. Then 
\[
\begin{array}{lcrr}
\displaystyle {\cal F}^{j+1}(x+iy) \, =\,  {\cal F}^{j+1}(x) +  i
\overline W_0^{\, -1} T_{j+1}(x,y)\overline W_{j}\,  y \, ,\\ [0.3cm]
\displaystyle  T_{j+1}(x,y) = \displaystyle {  \int_0^1 \,  \overline W_0 
D{\cal F}^{j+1}(x + ity) \overline W_{j}^{\, -1} \, dt \,  } 
\end{array} 
\]
(here we consider $\overline W_{j}$ as a linear operator acting in $\R^{3n}$). 
Moreover,   
$|T_{j+1}(x,y)| < \sqrt{3} \, \delta^{j}$ and using that  
$|\overline W_{j} \,  y| \le \delta|\overline W_{j+1} \,  y| \le \delta\sqrt 3\le \sqrt 3/6$ we
get 
\[
|T_{j+1}(x,y)\overline W_{j}\,  y| <  \frac{1}{2}  \, \delta^{j}\,  
,\quad x+iy\in D_{j+1}\times  O_{j+1} \, . 
\]
Set  $\overline Y_j =  
{\rm diag \, }\left(u_j^{-1}{\rm Id \, }, v_j^{-1}{\rm Id \, },   w_j^{-1}{\rm Id \, }\right)$ and denote by $Z_{j+1}(x,y)$ the imaginary  part of ${\cal F}^{j+1}(x+iy) $.  
Since ${\cal F}^{j+1}(x)$ is
real valued, $Z_{j+1}(x,y)$ is equal to  the real  part of $\overline W_0^{\, -1} T_{j+1}(x,y)\overline W_{j}\,  y $. Then we get
\[
|\overline Y_j Z_{j+1}(x,y)| \le \delta^{-j}|\overline Y_0 \overline W_0^{\, -1} ||T_{j+1}(x,y)\overline W_{j}\,  y|  <  \frac{1}{2}  \,  
,\quad x+iy\in D_{j+1}\times  O_{j+1} \, ,
\]
and we obtain \eqref{eq:map-F}. 


It remains to prove \eqref{eq:estimates-F2}. In the case when $p=0$ it follows from the arguments in \cite{Poe1}. Suppose now that $p=k=1$.  
Denote by $D{\cal F}^{j}(z)$  the differential of ${\cal F}^{j}$ with respect to $z=(\theta,I,\omega)$ acting on vectors $\eta\in \C^{3n}$ by 
$\eta\to D{\cal F}^{j-1}(z)\, .\, \eta$,   and by  $(\xi,\eta)\to D^2 {\cal F}^{j}(z)[\xi,\eta]$  the symmetric bilinear form corresponding to the second differential of $ {\cal F}^{j}$ at $z$. 
Consider
\[
\begin{array}{lcrr}
\displaystyle \partial_t({\cal F}^{j+1} - {\cal F}^{j}) = \partial_t(
{\cal F}^{j}\circ{\cal F}_{j} - {\cal F}^{j})\\ [0.3cm]
\displaystyle = \partial_t\, \int_0^1 \, D{\cal F}^{j} (x{\cal F}_{j} +(1-x) {\,  id\, }) \, . \, ({\cal F}_{j} - {\it id\, })\ dx = \Sigma_1 + \Sigma_2 +\Sigma_3, 
\end{array} 
\]
where 
\[
\begin{array}{lcrr}
\displaystyle \Sigma_1:=  \int_0^1 \, D{\cal F}^{j} (x{\cal F}_{j} +(1-x) {\,  id\, }) \, . \, \partial_t\, {\cal F}_{j} \ dx \, ,\\ [0.3cm]
\displaystyle \Sigma_2:=  \int_0^1 \, D(\partial_t\, {\cal F}^{j} )(x{\cal F}_{j} +(1-x) {\,  id\, }) \, . \, ({\cal F}_{j} - {\it id\, })\ dx \, ,\\ [0.3cm]
\displaystyle \Sigma_3:=  \int_0^1 \, D^2 {\cal F}^{j} (x{\cal F}_{j} +(1-x) {\,  id\, }) \,  [x \partial_t {\cal F}_{j}, {\cal F}_{j} - {\it id\, }]\ dx \, .
\end{array} 
\]
We are going to estimate $\Sigma_l$, $1\le l\le 3$. By  \eqref{eq:range-F}, \eqref{eq:estimates-F1} and \eqref{eq:estimate-differential-F} we get for any $j\ge 1$ 
\[
 \left|\overline W_0  \Sigma_1 \right|_{j+1} < \left|\overline W_0 D{\cal F}^{j}\overline W_{j}^{\, -1}\right|_{j} \left|\overline W_{j}\partial_t\, {\cal F}_{j} \right|_{j+1}  < C_0  \delta^{j-1}  \frac{\varepsilon_j}{r_jh_j} 
\]
since $\left|W_{j-1}W_{j}^{\, -1}\right|\le \delta<1$. 

Consider $\overline W_0  \Sigma_2$ now. Set ${\cal F}^{0}={\cal F}_{-1}= id$ and put ${\cal G}^{q}= {\cal F}_{q}\circ \cdots \circ  {\cal F}_{j-1}$ for $q\le j-1$ and ${\cal G}^{j}= id$. 
For $j\ge 1$  we have 
\[
\partial_t {\cal F}^{j} = 
\partial_t \left( {\cal F}_{0}\circ \cdots \circ  {\cal F}_{j-1}\right) = \sum_{q=0}^{j-1} (D{\cal F}^{q}\circ{\cal G}^{q})\, .\, 
((\partial_t  {\cal F}_{q})\circ{\cal G}_{q+1}) \, .
\]
Using \eqref{eq:range-F}, \eqref{eq:estimates-F1},  \eqref{eq:estimate-differential-F} and \eqref{eq:epsilon-by-rh}  we get as above 
\[
\begin{array}{lcrr}
 \displaystyle  \left|\overline W_0  \partial_t {\cal F}^{j} \right|_{j} < \sum_{q=0}^{j-1} \left|\overline W_0  D{\cal F}^{q}W_{q}^{\, -1}\right|_{q} \, 
\left|\overline W_q \partial_t  {\cal F}_{q}\right|_{q+1} \\ [0.3cm]
\displaystyle  \le C \sum_{q=0}^{j} \frac{\varepsilon_q}{r_qh_q } \le C(1-\delta^{\vartheta/2}) ^{-1}E_0^{1/2},
\end{array} 
\]
where $C$ stands for different constants depending only on $n$, $\tau$ and $\vartheta_0$. By Cauchy this implies 
\[
 \left|\overline W_0  D\partial_t {\cal F}^{j} \overline W_{j} \right| \le C
\]
uniformly on $\widetilde D_j \times \widetilde O_j\times [0,a]$, 
and we get 
\[
 \left|\overline W_0  \Sigma_2 \right|_{j+1}\,  \le\,  \sup_{\widetilde D_j \times \widetilde O_j\times [0,a]}\, \left|\overline W_0 D \partial_t{\cal F}^{j}\overline W_{j}^{\, -1}\right|  \left|\overline W_{j}( {\cal F}_{j} - id) \right|_{j+1}  \le C   \frac{\varepsilon_j}{r_jh_j} 
\]
where $C=C(n,\tau,\vartheta_0)$ stands for different positive constants depending only on $n$, $\tau$ and $\vartheta_0$.
In the same way, by \eqref{eq:estimate-differential-F} and Cauchy we get the estimate
\[
 \left|  D^2\overline W_0 {\cal F}^{j}(z)[W_{j}^{\, -1}\xi,W_{j}^{\, -1}\eta]\right| \,   \le \,  C \|\xi\|_{\C^{3n}}\|\eta\|_{\C^{3n}}  
\]
uniformly in  $z\in  \widetilde D_{j}\times \widetilde O_{j}$, $t\in [0,a]$ and $\xi,\eta\in \C^{3n}$. Setting $\xi = x \overline W_{j}\partial_t {\cal F}_{j}(\theta,I;\omega,t)$ and $\eta=\overline W_{j}({\cal F}_{j}(\theta,I;\omega,t) - (\theta,I;\omega))$,  we obtain as above
\[
 \left|\overline W_0  \Sigma_3 \right|_{j+1}  \le C    \frac{\varepsilon_j^2}{(r_jh_j)^2} .
\]
This proves \eqref{eq:estimates-F2} for $p=k=1$. In the case when $p=0$ we use the same arguments. 
This completes the proof of Proposition \ref{Prop:IterativeLemma}. 
\finishproof

\begin{Remark}[Uniqueness by construction in the Iterative Lemma]\label{rem:uniqueness-Iteration}
	The transformations ${\mathcal F}_{t,j}$, the normal forms $N_{t,j}:= N_{j}(\cdot,t)$ and the error terms $P_{t,j}:=P_{j}(\cdot,t)$   do not depend on the choice of the integer $m\in\N$ in \eqref{eq:secuence-nu-m} in the following sense. 
	Let $m'\in\N$  and ${\mathcal F}_{t,j}'$,  $N'_{t,j}$ and $P'_{t,j}$,  be the corresponding transformations,  normal forms and  error terms. 
	Then ${\mathcal F}'_{t,j}={\mathcal F}_{t,j}$,  $N'_{t,j}= N_{t,j}$  and $P'_{t,j}= P_{t,j}$ on the intersection of their domains of definition. 
\end{Remark}
Remark \ref{rem:uniqueness-Iteration} follows from Remark \ref{rem:uniqueness-KAM} and Remark \ref{rem:dependence-of-m} by induction whit respect to $j\in \N$. 

%-----------------------------------------------------------------------------------

\subsubsection{\it Choice of  the  sequence $\nu $ and the small the constants $\epsilon$ and $\hat{\varepsilon}$.}\label{sec:nu+epsilon}

Given  $m\in\N$ we consider the sequence $(\nu_j(m))_{j\in \N}$ introduced in \eqref{eq:secuence-nu-m} and set 
\begin{equation}
\label{eq:secuence-ell-m}
\ell_j(m)= \left\{
\begin{array}{lcrr}
\ell_0 = \tau +2 +\vartheta_0 \ &\mbox{for}&\  j<J(m), \\ [0.3cm]
\ell_m=m(\tau +1) +\ell_0 \ &\mbox{for}&\  j\ge J(m), 
\end{array}
\right.
\end{equation}
where $J(0)=0$ and $J(m)$, $m\ge 1$,  will be  a suitable integer satisfying \eqref{eq:J(m)}. 


Consider  the family of functions $P_t^j$, $j\in\N$,  defined by \eqref{eq:approximation-of-P}. In order to apply the Iterative Lemma to that family, we have to show  that it satisfies \eqref{eq:approximation6-0}, To this end we will choose appropriately  the small constants $\epsilon$ and $\hat{\varepsilon}$ as well as  the integer $J(m)$ for each $m\ge 1$.  
By  \eqref{eq:approximation-estimates1} and \eqref{eq:approximation-estimates2}, it suffices to prove for each $j\in \N$ that 
\begin{equation}
\label{eq:approximation6-1}
C_{\ell_j(m)} u_j^{\ell_j(m)}\, \sum_{p=0}^k \, \sup_{0\le t \le a} \|\partial_t^p P_t\|_{\ell_j(m);r,\kappa} \, \le \, \frac{\varepsilon_{j+1}}{4} \, 
=\,  \frac{1}{4}\hat\varepsilon \kappa  r_{j+1}(m)\sigma_{j+1}^{\tau + 1}  E_{j+1} (m) . 
\end{equation}
Here $r_j(m)$ and $E_j(m)$  are given by \eqref{eq:r} and \eqref{eq:E}, respectively, $\hat\varepsilon\in (0,1]$.
%, which will be determined below. To satisfy \eqref{eq:approximation6-1}, we shall choose $\hat\varepsilon\in (0,1]$ appropriately. 
In view of  \eqref{eq:u-v-w-sequences} and \eqref{eq:r}-\eqref{eq:epsilon}, the relation  \eqref{eq:approximation6-1} becomes
\begin{equation}
\label{eq:approximation6-2}
\sum_{p=0}^k \, \sup_{0\le t \le a}\|\partial_t^p P_t\|_{\ell_j(m);r,\kappa}\,  \le \,   \hat\varepsilon \kappa  r_0\sigma_0^{\tau + 1}   \frac{\left(\delta/ 4 s_0\right)^{\ell_j(m)}}{4C_{\ell_j(m)}} \delta^{M_j(m)} ,
\end{equation}
where 
\begin{equation}
\label{eq:M(nu)}
M_j(m) := q_{j+1}-(j+1)\ell_j(m) \, =\,( j+1)(\tau +2-\ell_j(m)) + 2(\nu_0(m)+\cdots+\nu_{j}(m)).
\end{equation}
Since  $r_0=s_0 r>\sigma_0 r$, 
the inequality \eqref{eq:approximation6-2} will follow from the following one 
\begin{equation}
\label{eq:approximation6-3}
\sup_{0\le p \le k} \, \sup_{0\le t \le a}\|\partial_t^p P_t\|_{\ell_j(m);r,\kappa}\,  \le \,    \hat\varepsilon \, \epsilon_j(m) \kappa  r \delta^{M_j(m)} ,
\end{equation}
where
\begin{equation}\label{eq:epsilon-ell}
\epsilon_j(m):= \sigma_0^{\tau + 2}  E_0 \frac{\left(\delta/ 4 s_0\right)^{\ell_j(m)}}{8C_{\ell_j(m)}} .
\end{equation}
We have
\[
\epsilon_j(m) 
= \left\{
\begin{array}{lcrr}
\epsilon_0 =  \sigma_0^{\tau + 2}  E_0 \frac{\left(\delta/ 4 s_0\right)^{\ell_0}}{8C_{\ell_0}} \quad  &\mbox{for}& \ j<J(m); \\ [0.3cm]
\epsilon_m=  \sigma_0^{\tau + 2}  E_0 \frac{\left(\delta/ 4 s_0\right)^{\ell_m}}{8C_{\ell_m}}   \quad  &\mbox{for}&\ j\ge J(m). 
\end{array}
\right.
\]
%depends only on $n,\tau, \vartheta, \vartheta_0$ and $m$. 
%If   $m=0$, then we  have 
%$M(j,\ell_0,(\nu(0)))=-(\vartheta_0-2\vartheta)(j+1)$ for any $j\in\N$,  and the estimates \eqref{eq:approximation6-3}  become
%\begin{equation}
%\label{eq:smallness0}
%\sup_{0\le p \le k} \,  \sup_{0\le t \le a} \| \partial_t^p P_t\|_{\ell_0;r,\kappa} \le   \hat\varepsilon \, \epsilon(0) \kappa  r \delta^{-(\vartheta_0-2\vartheta)(j+1)}\,   , \quad  \forall j\in\N.
%\end{equation}
Moreover, taking into account \eqref{eq:M(nu)},\eqref{eq:secuence-nu-m} and \eqref{eq:secuence-ell-m}, we obtain
\begin{equation}\label{eq:M(m)}
M_j(m) 
= \left\{
\begin{array}{lcrr}
-(j+1)(\vartheta_0-2\vartheta)\, \mbox{for}\,  j< J(m)\\ [0.3cm]
-(j+1)(m(\tau+1) +\vartheta_0-2\vartheta)  + 2m(\tau+1)  \, \mbox{for}\,  j\ge J(m).
\end{array}
\right.
\end{equation}
The relation  \eqref{eq:approximation6-3} becomes 
\begin{equation}
\label{eq:smallness0}
 \left\{
\begin{array}{lcrr}
\displaystyle \sup_{0\le p \le k} \, \sup_{0\le t \le a} \|\partial_t^p P_t\|_{\ell_0;r,\kappa} \le  \kappa r \hat\varepsilon \, \epsilon_0 \delta^{-(j+1)(\vartheta_0-2\vartheta)}  , \  &j&<J(m) ;\\ [0.3cm]
  \displaystyle   \sup_{0\le p \le k} \, \sup_{0\le t \le a} \|\partial_t^p P_t\|_{\ell_m;r,\kappa} \le  \kappa r  \hat\varepsilon \, \epsilon_m  \delta^{-(j+1)(m(\tau+1)+\vartheta_0-2\vartheta)}\delta^{2m(\tau+1)}   , \ & j&\ge J(m) .
\end{array}
\right.
\end{equation}




Our aim now is to satisfy  \eqref{eq:smallness0} for each $m\in\N$ and $j\in \N$, choosing  appropriately  $\hat\varepsilon\in (0,1]$ and $J(m)$.  

\vspace{0.2cm}
\noindent
{\em\large (1) \quad The case when $k=0$.}
\vspace{0.2cm}

\noindent
Suppose firstly that  $m=0$ and take $J(0)=0$. Then 
%To illustrate the construction, we firstly  take  $m=0$,  set 
%This case will be used to prove item  3 of Remark \ref{rem:kam}. $\ell =\ell_0=\ell(0)= \tau + 1+ \vartheta_0$,  and  consider the sequence  $\nu=(\vartheta)$, where  $\nu_j=\vartheta=\vartheta_0/6$, $ j\in\N$. 
%We have 
 \eqref{eq:smallness0}  becomes
\begin{equation}
\label{eq:smallness1}
\sup_{0\le t \le a} \|P_t\|_{\ell_0;r,\kappa} \le   \hat\varepsilon \, \epsilon_0 \kappa  r \delta^{-(\vartheta_0-2\vartheta)(j+1)}\,   , \quad  \forall j\in\N.
\end{equation}
%To satisfy \eqref{eq:smallness1} for $p=0$   we fix the small  constant $\epsilon$ in \eqref{eq:smallness-condition3} and $\hat\varepsilon_0$ by 
Let us set 
\begin{equation}
\label{eq:small-constant}
\epsilon := \epsilon_0 = \sigma_0^{\tau + 2}  E_0 \frac{\left(\delta/ 4 s_0\right)^{\ell_0}}{4C_{\ell_0}} \quad \mbox{and}\quad 
\hat\varepsilon=\hat\varepsilon_0:= (\kappa r\varepsilon)^{-1}\sup_{0\le t \le a} \|P_t\|_{\ell_0;r,\kappa}. 
\end{equation}
Then  \eqref{eq:smallness1} holds for any $j\in\N$.  Moreover,  \eqref{eq:smallness-condition3} just means that  
$$
0<\hat\varepsilon_0\le 1. 
$$ 
Notice that $\epsilon $ depends only on $n$, $\tau$ and $\vartheta_0$ since $c_{\ell_0}$, $\delta$, $\sigma_0$, $s_0$ and $E_0$ depend only on $n$, $\tau$ and $\vartheta_0$ by  \eqref{eq:delta+eta}, \eqref{eq:sigma-0} and  \eqref{eq:recurrence-relations}. Hence, one can apply the Iterative Lemma. 
%In this way one can obtain a family of continuous with respect to $t$ invariant tori of finite H\" older regularity. 
%In order to get $C^\infty$ families (with respect to $\omega$)  of regular tori and to prove  item (ii) of Theorem \ref{Theo:A},    we set 
%\begin{equation}\label{eq:secuence-ell-m}
%\ell_j=\ell_0 \ \mbox{for}\  j<J(m), \quad  \ell_m=\ell(m)=m(\tau +1) +\ell_0, 
%\end{equation}
%where $J(m)$ is a suitable integer satisfying \eqref{eq:J(m)}.  

%set  $J(q)=0$ for $q<m$ and we define the sequences $ \nu(m):=(\nu_j(m))_{j\in\N}$ and $ (\ell_j)_{j\le J(m)}$  by
%and  $(\ell_j)_{j\le J(m)}$ 
%Given an integer $J(m)\ge 1$ which will be fixed below, we set 
%\begin{equation}
%\ell_j = \left\{
%\begin{array}{lcrr}
%\ell_0 \quad \mbox{for}\quad j < J(m), \\[0.3cm]
%2m(\tau + 1) + \ell_0\quad  \mbox{for}\ j \ge J(m)
%\end{array}
%\right.
%\label{eq:l-j}
%\end{equation} 
%and  
%Notice that  \eqref{eq:approximation6-3} is satisfied for  $0\le  j< J(m)$ in view of \eqref{eq:smallness1} and \eqref{eq:small-constant}.  

Suppose now that $m\ge 1$. 
We still have \eqref{eq:smallness0}  for  $j<J(m)$, $p=k=0$,  and $\hat\varepsilon$ given by \eqref{eq:small-constant}. 
 On the other hand, for  $j \ge J(m)$ and $k\in\{0;1\}$,  the inequality   \eqref{eq:smallness0}  becomes 
\begin{equation}
\label{eq:smallness-A}
A_j^k(m):= C_0(m) \delta^{(j+1)(m(\tau+1) +\vartheta_0-2\vartheta)}  \frac{1}{\kappa r } \sum_{p=0}^k \ \sup_{0\le t \le a}\|\partial_t^p P_t\|_{\ell(m);r,\kappa} \le    \hat\varepsilon ,
\end{equation}
where $C_0(m) = \delta^{-2m(\tau +1)} \epsilon_m^{-1}$. 

The sequence $(A_j^0(m))_{j\in \N}$ is decreasing and it tends to zero. 
Let $J(m)$ be the smallest integer 
\[
j \ge m(\tau+1)\vartheta^{-1}  
\]
such that $A_{j}^0(m)\le \hat\varepsilon$.  By definition, $J(m)$ satisfies \eqref{eq:J(m)}. We claim that there exist 
$$
\widetilde C_m=\widetilde  C_m(n,\tau,\vartheta,\vartheta_0)> 0,
$$
depending only on $n,\tau,\vartheta,\vartheta_0$ and $m$, such that
\begin{equation}\label{eq:A-m}
 \widetilde  C_m \hat\varepsilon   \le A_{J(m)}^0(m)  \le \hat\varepsilon . 
\end{equation} 
Indeed, if  $J(m)-1\ge m(\tau+1)\vartheta^{-1}$, then $A_{J(m)-1}^0(m) >\hat\varepsilon$, and we get 
$$
\hat\varepsilon \ge A_{J(m)}^0(m)= \delta^{m(\tau+1) +\vartheta_0-2\vartheta}A_{J(m)-1}^0(m) >\hat\varepsilon  \delta^{m(\tau+1) +\vartheta_0-2\vartheta }.
$$
If $J(m)<m(\tau+1)\vartheta^{-1} + 1$, then 
$$
\begin{array}{rcll}
\displaystyle \hat\varepsilon  &\ge&   \displaystyle A_{J(m)}^0(m)   \ge 
C_0(m) \delta^{(J(m)+1)(m(\tau+1) +\vartheta_0-2\vartheta)} \epsilon \frac{1}{\kappa r \epsilon} \sup_{0\le t \le a}\|P_t\|_{\ell_0;r,\kappa}\\
 &\ge&      \displaystyle C_0(m)\epsilon \,    \delta^{(m(\tau+1)\vartheta^{-1} + 2)(m(\tau+1) +\vartheta_0-2\vartheta)} \hat\varepsilon   
 \end{array}
$$
and we obtain \eqref{eq:A-m} since $ C_0(m) \epsilon$  and $\delta$ depend only on  $n,\tau,\vartheta, \vartheta_0$ and $m$. 


\vspace{0.2cm}
\noindent
{\em\large (2)\quad The case when $k=1$.}

\vspace{0.2cm}
\noindent
Choosing  $\hat\varepsilon$ and  $J(m)$ as in the case (1), and we obtain that $P_t$ satisfies   \eqref{eq:smallness0}  for $p=0$. 
To satisfy  \eqref{eq:smallness0} for  $p=1$,  we need an additional argument. 
 We rescale $t$ by setting  $\tilde t = t T(m)\in [0,\tilde a(m)]$, where $\tilde a(m) = a T(m)$ and 
\begin{equation}\label{eq:T}
\displaystyle T(m)\, :=\,   \frac{1}{\hat \varepsilon \kappa r \epsilon} \,   \sup_{p\in\{0;1\}}  \,   \sup_{0\le t \le a} \|\partial_t^p P_t\|_{\ell_m;r,\kappa} = 
 \frac{\displaystyle  \sup_{p\in\{0;1\}}  \,   \sup_{0\le t \le a} \|\partial_t^p P_t\|_{\ell_m;r,\kappa} }{\displaystyle  \sup_{0\le t \le a} \|P_t\|_{\ell_0;r,\kappa} }    \ge  1.
\end{equation}
Then $\widetilde P_{\tilde t}$ satisfies  \eqref{eq:smallness0} for $p=0$. Moreover, 
%the derivative of $\widetilde P_{\tilde t} :=  P_{\tilde t/T}$ with respect to $\tilde t$ satisfies \eqref{eq:smallness0} by construction, hence,   $\widetilde P_{\tilde t}$ verifies \eqref{eq:smallness0} for $k=1$. 
%Indeed,
\[
\|\partial_{\tilde t} \widetilde P_{\tilde t}\|_{\ell_0;r,\kappa} \le  \frac{1}{T}\|\partial_{\tilde t} \widetilde P_{\tilde t}\|_{\ell_m;r,\kappa} = \|P_{t}\|_{\ell_0;r,\kappa} 
\]
and
\[
\|\partial_{\tilde t} \widetilde P_{\tilde t}\|_{\ell_m;r,\kappa} = \|P_{t}\|_{\ell_0;r,\kappa} \le  \|P_{t}\|_{\ell_m;r,\kappa} 
\]
and we obtain  \eqref{eq:smallness0} for $p=1$. 
Replacing $P_t$ with $\widetilde P_{\tilde t}$, we can  
apply Proposition \ref{Prop:kam-step} to $\widetilde P_{\tilde t}^j$ for $\tilde t\in [0,\widetilde a]$ at each iteration 
(recall that the constants in Proposition \ref{Prop:kam-step} do not depend on $a$). 
%In this way we will obtain a convergent scheme for $\widetilde P_{\tilde t}$. 
%Then scaling back with respect to $t$ we will obtain the corresponding  for $P_t$.  ??????
%To get (ii) for $P_t$ and $q=1$ we use the inequality $T\ge 1$.  
%In this way, 
%replacing  $P_t$ by  $\widetilde P_{\widetilde t}$  and  $a$ by $\widetilde a(m)$,  we may assume that \eqref{eq:smallness1} holds for $0 \le p\le k\le 1$ with $\epsilon$ and $\hat\varepsilon$ given by \eqref{eq:smallness0}. \\





We summarize the above construction by the following
\begin{Lemma}\label{Lemma:approximation}
	Fix the positive constants $\epsilon$ and $\hat\varepsilon\le 1$ by \eqref{eq:small-constant}. Then 
	\begin{itemize}
	\item[(i)] If 	$k=0$  then 
	for each  $m\in\N$  the sequence  $(\widetilde\varepsilon_{\ell_j(m),j,0})_{j\in\N}$ defined in \eqref{eq:approximation-estimates2}    satisfies \eqref{eq:approximation6-1}  and 
	the Iteration Lemma holds for any $m\in \N$; 
	\item[(ii)]  If $k=1$, then  $\tilde P_{\tilde t}$, $\tilde t\in [0, \tilde a(m)]$, satisfies  \eqref{eq:approximation6-1}  and the Iteration Lemma holds for any $m\in \N$. 
\end{itemize}
\end{Lemma}
How do the maps $\Phi^j$ and $\phi^j$, $j\in\N$,  depend on $m\in\N$? The answer of this question is given by the following 
\begin{Lemma}[Uniqueness by construction] \label{Lemma:dependence-of-m}
We have 	the following:
\begin{itemize}
	\item[(i)] The transformations $\Phi_{j,t}$ and $\phi_{j,t}$, $j\in\N$, do not depend on $m$ in the following sense. If  $m'\in\N$  and $\Phi_{t,j}'$ and $\phi'_{t,j}$,  are the corresponding transformations, 
	then $\Phi'_{t,j}=\Phi_{t,j}$ and $\phi'_{t,j}= \phi_{t,j}$ on the intersection of their domains of definition. 
	\item[(ii)] Let $\widetilde\Phi_{\tilde t,j}$ and $\widetilde \phi_{\tilde t,j}$, $j\in\N$, be the transformations corresponding to $\widetilde P_{\tilde t}$, where $\tilde t = t T(m)$. Then $\widetilde\Phi_{\tilde t,j}=\Phi_{t,j}$ and $\widetilde\phi_{\tilde t,j}=\phi_{ t,j}$. 
\end{itemize}
\end{Lemma}	
In order to prove (ii), Theorem \ref{Theo:A}, we need  the following
\begin{Lemma}\label{lem:estimate-eps-b}
	For each $m\in \N$ there exists 	$C_m=C_m(n,\tau,\vartheta, \vartheta_0)>0$ depending only on $m,n,\tau,\vartheta,\vartheta_0$ such that 
	\[
	\hat\varepsilon E_{j}(m) \le  C_m \sigma_{j+1}^{m(\tau+1)+ \vartheta_0} \frac{1}{\kappa r } \sup_{0\le t \le a}\|P_t\|_{\ell(m);r,\kappa} , \quad j\in\N.
	\]
\end{Lemma}
{\em Proof.}\quad 
If $m=0$ the estimate holds in view of the choice of  $\varepsilon$. Suppose now that $m\ge 1$. 
Using \eqref{eq:smallness-A}  and \eqref{eq:A-m} we obtain 
\[ 
\begin{array}{rcll}
	\displaystyle \hat\varepsilon E_{j}(m) &\le& \displaystyle \widetilde  C_m ^{-1} A_{J(m)}^0(m)E_{j}(m) \\ [0.3cm]
		&=&  \displaystyle \widetilde  C_m ^{-1}  C_0(m) \delta^{(J(m)+2)(m(\tau+1) +\vartheta_0-2\vartheta)} E_{j}(m)\frac{1}{\kappa r } \sup_{0\le t \le a}\| P_t\|_{\ell(m);r,\kappa} \\  [0.3cm]
		 &=&  \displaystyle C_1(m)   \delta^{  F_m(j) } \frac{1}{\kappa r } \sup_{0\le t \le a}\| P_t\|_{\ell(m);r,\kappa} ,
\end{array}	
 \]
 where $C_1(m)= C_m ^{-1} C_0(m)\delta^{-(m(\tau+1) +\vartheta_0)}  $ depends only on $n,\tau,\vartheta_0$ and $m$, and
 \[ 
 F_m(j) := (J(m)+2)(m(\tau+1) +\vartheta_0-2\vartheta) +2(\nu_0 + \cdots +\nu_{j-1}) + 2\vartheta.
  \]
  Let  $ j\le J(m)+1$. Using \eqref{eq:secuence-nu-m}, we get 
  $$
  F_m(j) \ge   (J(m)+2)(m(\tau+1) +\vartheta_0-2\vartheta) +2(j+1)\vartheta \ge (j+1)(m(\tau+1) +\vartheta_0). 
  $$ 
 If $ j\ge J(m)+1$, then   ?????
  $$
  \begin{array}{rcll}
  \displaystyle 
  F_m(j) &>& 2(m(\tau+1) +\vartheta_0-2\vartheta)+ 2(\nu_0 + \cdots +\nu_{j-1}) \\
  &=& 
  2(m(\tau+1) +\vartheta_0-2\vartheta)+ 2j(m(\tau+1) +\vartheta) \ge (j+1)(m(\tau+1) +\vartheta_0), 
  \end{array}	
  $$
 since   $0<6\vartheta <\vartheta_0< \tau+1$ and $m\ge 1$. This  proves the lemma.  \finishproof












%-----------------------------------------------------------------------------------------------------------------------

\noindent


We are ready to prove the statements (i) and (ii) of Theorem  \ref{Theo:A}. 
Set 
\[
{\cal F}^{j}(\theta,I;\omega,t)= (\Phi^j(\theta,I;\omega,t),\phi^j(\omega,t))
\] 
where  $\Phi^j(\theta,I;\omega,t)= (U^j(\theta;\omega,t),V^j(\theta,I;\omega,t))$ and $V^j$ is affine linear in $I$ by construction. Set
\begin{equation}
\label{eq:limits}
\left\{
\begin{array}{lcrr}
\displaystyle \Psi(\theta;\omega,t)=(U(\theta;\omega,t),V(\theta;\omega,t))=\lim_{j\to\infty} \Phi^{j}(\theta,0;\omega, t),\\[0.3cm]
\displaystyle \phi(\omega,t)=\lim_{j\to\infty} \phi^{j}(\omega, t),\ (\theta,\omega,t)\in \T^n \times \Omega_\kappa\times [0,a]. 
\end{array}
\right.
\end{equation}
Using Remark \ref{rem:analytisity-t-KAMstep} and Cauchy one obtains 
\begin{Remark}\label{rem:analyticity-t-iteration}
	If $P^j$ are analytic with respect to $t$ in $B(0,a)$ and satisfy \eqref{eq:approximation6-0} for $t\in B(0,a)$, then ${\cal F}_j$ are analytic with respect to $t$ in $B(0,a)$ and the estimates \eqref{eq:estimates-F1} and \eqref{eq:estimates-F2} hold for $p=0$ and $t\in B(0,a)$. Moreover, $\Psi$ and $\phi$ are analytic in $t$ in $B(0,a)$. 
\end{Remark}

\subsection{Proof of (i)}
\label{Sect.i}
Choose $\nu_j=\vartheta$ and $ \hat\varepsilon_j = \hat\varepsilon_0$ as in \eqref{eq:small-constant} (Case 1). 
As in Sect. 5.d, \cite{Poe1}, we obtain that
\[
\left| X_{H^j} \circ {\cal F}^j - D \Phi^j \cdot X_N\right| \le 
\frac{c\varepsilon_j}{r_jh_j}
\]  
on ${\T}^n \times \{0\}\times \Omega_\kappa$ for all $j\ge 0$,
where $ X_{H^j}$ and $X_{N}={\mathcal L}_\omega$ stand for the Hamiltonian vector fields of 
$H^j(\theta,I;\omega,t)$ and $N(\theta,I;\omega)=\langle \omega,I \rangle $,
respectively. On the other hand, $\nabla_{(\theta,I)} H^j$ converges uniformly to 
$\nabla_{(\theta,I)} H$ as $j\to \infty$ in view of \eqref{eq:approximation-estimates1} and \eqref{eq:approximation-estimates2}, hence, 
$$
X_{H(\cdot;\phi(\omega,t),t)} \circ \Psi(\cdot;\omega,t) = D \Psi(\cdot;\omega,t)  \cdot {\mathcal L}_\omega
$$
on ${\T}^n \times \{0\}\times \Omega_\kappa$. Moreover, by \eqref{eq:estimates-F1} and \eqref{eq:epsilon-by-rh} we obtain 
\[
|\partial_t^p(U_{j}(\cdot;\cdot,t) - {\rm id} )|_{j+1}  <   
 \frac{C_0 \sigma_j \varepsilon_j}{r_jh_j}  \le 
 C \hat\varepsilon_0 \sigma_j^{1+\vartheta/2} E_0^{1/2}
\]
for $0\le p\le k$ with some constants $C>0$ depending only on $n$, $\tau$ and $\vartheta_0$. Then 
the Inverse Approximation Lemma \ref{Lemma:inverse-approximation-lemma} implies that 
$$
U(\cdot,\omega,\cdot)= \lim U_{j}(\cdot,\omega,\cdot)\in C^k([0,1], C^{1+\vartheta/2}(\T^n)) , \quad \omega \in \Omega_\kappa.
$$ 
The corresponding H\"older norm is estimated by
\[
\|U(\cdot;\omega,t) - {\rm id} \|_{1+\vartheta/2}  <
 C(n,\tau, \vartheta_0) \hat\varepsilon_0  E_0^{1/2} \le  C(n,\tau, \vartheta_0)  E_0^{1/2}  \ll   1 ,
\]
choosing $E_0$ small enough in a function of $n$, $\tau$ and $\vartheta_0$, 
hence, $U(\cdot,\omega,t)$ is  an embedding. 
Then 
\[
t\to \{\Psi(\theta;\omega,t):\, \theta\in {\T}^n\}
\] 
is a $C^k$ family of  embedded  invariant
tori  
of the Hamiltonians $(\theta,I) \to H(\theta,I;\phi(\omega,t),t)$
with frequency $\omega \in \Omega_\kappa$. They are Lagrangian by
construction (see also \cite{Her}, Sect. I.3.2). In particular, we prove Remark \ref{rem:kam}, 3,(i).

\subsection{K.A.M. theorem with parameters in H\"older classes.}
\label{Sect.ii}

Fix $m\in \N$ and $0<\vartheta_1< \vartheta_0 (\tau+1)^{-1}$. Recall that $\ell_0=\tau+2+\vartheta_0$, and $\ell(m)= m(\tau+1) + \ell_0$, $m\in \N$, where $0<\vartheta_0<\tau+1$. We suppose that $\ell(m)\notin \N$ for each $m\in \N$.   ????  
Fix $k\in\{0;1\}$. 

\begin{Theorem}\label{Theo:Holder}
	There exists a  positive constant $\epsilon= \epsilon(n,\tau,\vartheta, \vartheta_0)>0$  depending only  on $n$, $\tau$, $\vartheta_0$ and  $\vartheta_1$ such that, for any $a>0$, $0<\kappa<1$, $0<r < \rho_0$, and  any real valued Hamiltonian  $H=N+P$, where $N(I;\omega)=\langle\omega,I\rangle $ and  $P\in C^k\big([0,a];C_0^{\ell(m)}(\A^n\times\Omega)\big)$ satisfies   \ the smallness condition
	\begin{equation}
	\sup_{t\in [0,a]} \, \| P_t\|_{\ell_0;r,\kappa} \  \le \ \epsilon \kappa r \, ,
	\label{eq:smallness-condition-4}
	\end{equation}
	the following holds.
	
	\vspace{0.3cm}
	\noindent
	There exist families of maps 
	\begin{equation}\label{eq:maps-Holder}
	[0,a]\ni t \mapsto \phi_t\in C^{1+\vartheta_1}(\Omega;\Omega)\, ,\ [0,a]\ni t \mapsto \Psi_t=(U_t,V_t)\in C^{1+\vartheta_1}(\T^n \times\Omega;\T^n\times B(0,r)) \ 
	\end{equation}
	such that   ${\rm supp\,}(\phi_t-{\rm id})\subset \Omega-\kappa/2$, ${\rm supp\,}\big((U_t,V_t)-({\rm id}_{\T^n},0)\big)\subset \T^n\times (\Omega-\kappa/2)$,  and 
	\begin{enumerate}
		\item[(i)] For any $\alpha,\, \beta\in \N^n$ such that $|\alpha| +  |\beta| (\tau+1)\le \ell(m)$, the partial derivatives $\partial_\omega^{\beta}\phi_t$ and $\partial_\theta^{\alpha}\partial_\omega^{\beta}\Psi_t$ exist and belong to $C^{\vartheta_1}(\Omega;\Omega)$ and $C^{\vartheta_1}(\T^n \times\Omega;\T^n\times B(0,r))$, respectively. Moreover, 
		$$\partial_\omega^{\beta}\phi\in C^k\big([0,a];C^{0}(\Omega;\Omega)\big)\, , \quad \partial_\theta^{\alpha}\partial_\omega^{\beta}\Psi\in C^k\big([0,a];C^{0}(\T^n \times\Omega;\T^n\times B(0,r))\big).$$	
		\item[(ii)]
		For each $\omega \in \Omega_\kappa$ and $t\in [0,a]$ the map 
		$\Psi_{t,\omega} := \Psi_t(\cdot,\omega):{\T}^n  \rightarrow
		{\T}^n\times B(0,r)$ 
		is an embedding, 
		$\Lambda_t(\omega)  := \Psi_{t,\omega}({\T}^n)$ is an embedded Lagrangian 
		torus invariant  with respect to the Hamiltonian flow of 
		$ H_{t,\phi_t(\omega)}(\theta,I) := H(\theta, I; \phi_t(\omega),t)$, and 
		\[
		X_{H_{t,\phi_t(\omega)}} \circ \Psi_{t,\omega} = 
		D \Psi_{t,\omega} \cdot {\mathcal L}_\omega \quad \mbox{on}\  {\T}^n ,  
		\]
		\item[(iii)]
		For any integer $0\le m\le b$ there is $C_m>0$ depending only on  $n$, $\tau$, $\vartheta_0$, $\vartheta_1$,  and $m$, (but not on $b$) such that
		for any $\alpha,\beta\in \N^n$ satisfying the inequality $|\alpha| +  |\beta| (\tau+1)\le \ell(m)$ and $0\le q\le k$ the following H\"older estimate holds
		\[ 
		\begin{array}{lrc}
		\|\partial_\theta^{\alpha}(\kappa \partial_\omega)^{\beta}
		\partial_t^q(U_t - {\rm id}_{\T^n})\|_{\vartheta_1}\,  + \,
		r ^{-1}
		\|\partial_\theta^{\alpha}(\kappa \partial_\omega)^{\beta}\partial_t^q V_t\|_{\vartheta_1} 
		\\    [0.5cm]  
		\displaystyle + \kappa^{-1} \|(\kappa \partial_\omega)^{\beta}
		\partial_t^q(\phi_t - {\rm id})\|_{\vartheta_1}  \leq\    C_{m}\, 
		(\kappa  r )^{-1}\, \sup_{0\le p\le q} \,  \sup_{t\in [0,a]} \,\|\partial_t^p P_t\|_{\ell(m);r,\kappa} 
		\end{array}
		\]
		uniformly in  $t\in [0,a]$. 
		\item[(iv)]The restriction of $\phi_t$ and $\Psi_t$ to $\Omega_{ \kappa}$ and $\T^n\times \Omega_{ \kappa}$, respectively,  does not depend on $m\in \N$.
		\item[(v)] If $P$ is analytic with respect to $t$ in an open  disc  $B(0,R_0)\subset \C$ of radius $R$ and \eqref{eq:smallness-condition-4} holds for any $t\in B(0,R_0)$ , then $\phi$ and $\Psi$ are analytic in $t\in B(0,R)$ for any $0<R<R_0$, and the inequalities in $(iii)$ hold uniformly  in $t\in B(0,R)$ for  $q=k=0$, where the constant $C_m$ depends on $R$ as well. 
	\end{enumerate}
\end{Theorem}
\begin{Remark}
	Item (iii) means that for any integers $0\le m_1<m_2\le m$ the restriction of the  corresponding maps \eqref{eq:maps-Holder} to $\Omega_{ \kappa}$ and $\T^n\times \Omega_{ \kappa}$, respectively, coincide (uniqueness by construction).
\end{Remark}
\noindent
{\em Proof of Theorem \ref{Theo:Holder}.}\quad 
We are going to prove that the limit of  ${\cal F}^{j}$ as $j\to\infty$ gives a H\"older smooth function on $\T^n\times\Omega_\kappa\times [0,a]$ in a Whitney sens. To this end we use a suitable Inverse Approximation Lemma (cf \cite{Poe}, \cite{Sa} Lemma 4,   \cite{Sa-Ze} Lemma 4). 

We are going to show that the limits \eqref{eq:limits} define Whitney jets in $C^k([0,a], C^\infty(\T^n\times \Omega_\kappa))$. 
Set $\T^n_j:= \{\theta\in \C^n/ \Z^n:\, |{\rm Im\,} \theta |< s_j/2\}$ and 
recall that 
\[
\widetilde D_j =  \T^n_j\times \{I\in \C^n :\, |I|<r_j/2\}, \quad 
\widetilde O_j = \{\omega\in {\C}^n:\ |\omega - \Omega_\kappa
|<h_j/2\} \, .   
\]
For any $j\in\N$ we denote by ${\mathcal S}_j$ the jet $\left( S_j^\beta\right)_{\beta\in\N^n}$, where 
\[
S_j^\beta(\theta,\omega,t) := \partial^\beta_\omega {\cal F}^{j+1}(\theta, 0;\omega,t) - \partial^\beta_\omega {\cal F}^j(\theta, 0;\omega,t), 
\quad (\theta,\omega,t)\in\T^n_{j+1}\times \widetilde O_{j+1}\times  [0,a]\, . 
\]
We set  
\[
\left\{
\begin{array}{lcrr}
\displaystyle \left(T^N_{\omega } 
 {\cal S}_j\right)_\beta(\theta,\omega',t) := \displaystyle 
 \sum_{|\beta +\gamma|\le N}(\omega'-\omega) ^{\gamma} 
S_j^{\beta+\gamma}(\theta, \omega,t ) /\gamma !\\[0.3cm]
\left(R^N_{\omega } 
 {\cal S}_j\right)_\beta(\theta,\omega',t) := 
  S_j^\beta(\theta,\omega',t) - \left(T^N_{\omega } 
 {\cal S}_j\right)_\beta(\theta, \omega',t) \, ,
 \end{array}
\right.
\]
Fix $m\in \N$ and choose the numbers $\nu_j$ and $\hat\varepsilon_j$ as in \eqref{eq:p-j} (Case 2). $m\le b$ ???????
 \begin{Lemma} \label{Lemma:inverse-approximation} (Inverse Approximation Lemma) Under the assumptions of Proposition \ref{Prop:IterativeLemma} we have  the following estimates
\[
\left\{
\begin{array}{lcrr}
\displaystyle
|\overline{W}_0 \partial_t^p \partial_\theta^\alpha 
S_j^\beta(\theta,\omega,t)| \,   \le \,  \displaystyle   C\kappa^{-|\beta|}\, 
 \sigma_{j+1}^{\vartheta_0-5\vartheta} \, \frac{1 }{\kappa  r } \sum_{p=0}^k \ \|\partial_t^p P_t\|_{\ell(m);r,\kappa}\, ,   ?????
\\ [0.3cm]
\mbox{for}\quad |\alpha|+|\beta|(\tau+1)\le m(\tau+1)  \end{array} 
\right.
\]
and $(\theta,\omega,t) \in  \T^n_{j+1}\times \widetilde O_{j+1}\times  [0,a]$, and 
\[
\left\{
\begin{array}{lcrr}
\displaystyle
|\overline{W}_0 \partial_t^p \partial_\theta^\alpha \left(R^q_{\omega } 
 {\cal S}_j\right)_\beta(\theta,\omega',t)|\,
\le \,   \displaystyle  C \kappa^{-|\beta|-q}\, 
 \sigma_{j+1}^{\vartheta_0-5\vartheta} \, |\omega-\omega'|^{q+|\beta|+1} \, \frac{ 1}{\kappa r } \sum_{p=0}^k \ \|\partial_t^p P_t\|_{\ell(m);r,\kappa},   ????
\\ [0.3cm]
\mbox{for}\quad |\alpha| + (q+|\beta|+1)(\tau +1) \le m(\tau+1)\, ,
    \end{array} 
    \right.
\]
and $(\theta,t)\in  {\T}^n\times  [0,a],\ \omega, \omega '\in \Omega_\kappa$,  and for any for $j\in \N$, 
where $C>0 $ depends only on $m$, $n$, $\tau$, $\vartheta$ and $\vartheta_0$.    
\end{Lemma} 
{\em Proof}. Using \eqref{eq:estimates-F2} and applying the Cauchy  estimate \eqref{eq:Cauchy1}
to the analytic function 
\[
(\theta,\omega)\ \to\  {\cal S}^{j}(\theta,\omega,t)
\] 
in  $\T^n_{j+1}\times \widetilde O_{j+1} \subset D_{j+1}\times O_{j+1}$, 
we  evaluate $\partial_t^p\partial_\theta^\alpha 
S_j^{\beta}$  for any $j\in \N$ and 
$\alpha,\beta\in \N^n$ in  
$\T^n_{j+1}\times  \widetilde O_{j+1}$ by
\begin{equation}
\left| \overline{W}_0  \partial_t^p\partial_\theta^\alpha 
S_j^{\beta}( \theta,\omega,t)\right| 
\, \le  \,   C_0\,  \alpha!\beta! \, 2^{|\alpha|+|\beta|}\, 
\frac{
\varepsilon_j}{{r_jh_j s_{j+1}^{|\alpha|}} h_{j+1}^{|\beta|}}, 
\label{eq:Cauchy}
\end{equation}
where $C_{\alpha,\beta}$ is a positive constant depending only on $\alpha$, $\beta$, $n$, $\tau$ and $\vartheta_0$. 


Given $\mu,\nu\in\N$, we consider 
\[
\widetilde\varepsilon_{j,\mu,\nu} \, := \, \frac{
	\varepsilon_j}{{r_jh_j s_{j+1}^{\mu}} h_{j+1}^{\nu}} = \kappa  \hat\varepsilon (b) 
\frac{
\sigma_j^{\tau+1}E_j}{{h_j s_{j+1}^{\mu}} h_{j+1}^{\nu}}. 
\]
%By \eqref{eq:s}, \eqref{eq:E},  \eqref{eq:epsilon},  and \eqref{eq:epsilon-j}  we get for $j\ge 0$ 
%\[
%\begin{array}{lcrr}
%\displaystyle\widetilde\varepsilon_{j,\mu,\nu} = \frac{	\varepsilon_j}{{r_jh_j s_{j+1}^{p}} h_{j+1}^{q}}=\hat\varepsilon (b) \kappa 
%\frac{	\sigma_j^{\tau+1}E_j}{{h_j s_{j+1}^{\mu}} h_{j+1}^{\nu}}\\[0.5cm] 
%\displaystyle \le  C_{m,\mu}\, \kappa \, 
%\frac{\sigma_j^{\tau+1}\sigma_{j+1}^{m(\tau+1)+\vartheta-\mu}}{h_j  h_{j+1}^{\nu}}, 
%\end{array}
%\]
%where $C_{m,\mu} >0$ 
%depends only on $m$, $\mu$, $\tau$, $n$ and $\vartheta_0$. 
Using 
\eqref{eq:h-and-K} and the inequality $\sigma_{j+1}<s_{j+1}$, we obtain 
\[ 
\widetilde\varepsilon_{j,\mu,\nu}\, <\,  2^{\nu+1}\, \kappa^{-\nu} \hat\varepsilon(b)\, E_j\,  \sigma_{j+1}^{-\mu-\nu(\tau+1)}\big(\ln(\sigma_{j+1})\big)^{2(\nu+1)(\tau +1)} .
 \]
Now Lemma \ref{lem:estimate-eps-b} implies 
\begin{equation}
\widetilde\varepsilon_{j,\mu,\nu}\, <\,  C  \kappa^{-\nu}\sigma_{j+1}^{M_{\mu,\nu}}\big(\ln(\sigma_{j+1})\big)^{2(\nu+1)(\tau +1)} \frac{1}{\kappa r } \sup_{0\le t \le a}\|P_t\|_{\ell(m);r,\kappa}\, ,
\label{eq:p-q}
\end{equation}
where 
$$M_{\mu,\nu}:= (m-\nu)(\tau+1)-\mu+ \vartheta_0-4\vartheta$$ 
and $C$ depends only on $m$, $\mu$, $\nu$, $n$, $\tau$, $\vartheta$  and $\vartheta_0$. 


Let $|\alpha|+|\beta|(\tau+1)\le m(\tau+1)$. 
Then $M_{|\alpha|,|\beta|}\ge \vartheta_0-4\vartheta$ and \eqref{eq:Cauchy} and  \eqref{eq:p-q} yield
\begin{equation} 
\label{eq:M}
\left| \overline{W}_0  \partial_t^p\partial_\theta^\alpha 
S_j^{\beta}(\theta,\omega,t)\right| \, \le   \, 
\displaystyle  C _m \kappa^{-|\beta|}\sigma_{j+1}^{\vartheta_0-4\vartheta}\big(\ln(\sigma_{j+1})\big)^{2(|\beta|+1)(\tau +1)} \frac{1}{\kappa r } \sup_{0\le t \le a}\|P_t\|_{\ell(m);r,\kappa},
\end{equation} 
where 
and $C_m>0 $ depends only on $m$, $n$, $\tau$, $\vartheta$ and $\vartheta_0$. This implies the first estimate. \\

We are going to prove the second estimate for $\omega, \omega' \in
\Omega_\kappa$.   Suppose firstly 
that $|\omega' - \omega| \le h_{j+1}/4$. 
Expanding  the analytic in $O_{j+1}$ function    
$\omega' \to \partial^p_t\partial^\alpha_\theta \partial^\beta_\omega S_j^{0}(\theta, \omega',t)$  
in Taylor series  at $\omega'=\omega$ 
and using the Cauchy estimates \eqref{eq:Cauchy1} as in \eqref{eq:Cauchy},  we  obtain  
\[
\begin{array}{lcrr}
A:= |\overline{W}_0 \partial_t^p \partial_\theta^\alpha \left(R^q_{\omega } 
{\cal S}_j\right)_\beta(\theta,\omega',t)| 
\\ [0.5cm]
\le 
\displaystyle{ \sum_{|\gamma|\ge  q  +1}\, 
	|\omega' - \omega|^{|\gamma|}\, \left| \overline{W}_0  \partial_t^p\partial_\theta^\alpha 
	S_j^{\beta+\gamma}(\theta,\omega',t)\right| /\gamma !}
\\ [0.5cm]
\le \displaystyle 
\sum_{|\gamma|\ge  q  +1}\, |\omega' -
\omega|^{|\gamma|} \frac{  C_0  \alpha!(\beta+\gamma)! \varepsilon_j}
{r_j h_j s_{j+1}^{|\alpha|} h_{j+1}^{|\beta+\gamma|}\gamma !}
\\ [0.5cm]
\le \displaystyle{ C_0\, 2^{q+|\beta|+1} \alpha!\beta! \,   |\omega' -
	\omega|^{q+1}}  
\frac{ \varepsilon_j}
{r_j h_j s_{j+1}^{|\alpha|} h_{j+1}^{q+|\beta|+1}} \\ [0.5cm]
\displaystyle  \times \sum_{|\gamma|\ge q  +1}\, 
\left(2 |\omega' - \omega|h_{j+1}^{-1}\right)^{|\gamma|-q-1}\\ [0.5cm]
\displaystyle  \le   C_{q,\alpha,\beta} \kappa^{-(|\beta|+q+1)}\,|\omega-\omega'|^{q+1} \widetilde\varepsilon_{j,|\alpha|,q+|\beta|+1}.
\end{array}
\]
for $\theta\in  {\T}^n,\ \omega,\, \omega' \in \Omega_\kappa$. 
We have used the estimate $(\beta+\gamma)! (\beta! \gamma!)^{-1}\le 2^{|\beta + \gamma|}$. 




Let $|\alpha| + (q+|\beta|+1)(\tau +1) \le m(\tau+1)$. 
Then  \eqref{eq:p-q} implies 
\[
 A\le  C_m \kappa^{-(q+|\beta|)}
|\omega-\omega'|^{q+1}  
\sigma_{j+1}^{\vartheta_0-4\vartheta} (\ln(\sigma_{j+1}))^{(2m+4)(\tau +1)} \frac{1}{\kappa r } \sup_{0\le t \le a}\|P_t\|_{\ell(m);r,\kappa}.  
\]
The constant $C_m$ depends only on $m$, $n$, $\tau$, $\vartheta$ and $\vartheta_0$.
If 
$|\omega' - \omega| \ge h_{j+1}/4$, we obtain the same inequality  
estimating $\partial_t^p \partial_\theta^\alpha \left(R^q_{\omega } 
 {\cal S}_j\right)_\beta$ term by term and using (\ref{eq:M}).  
This proves the lemma. \finishproof

According to Proposition \ref{Prop:IterativeLemma},  
Lemma \ref{Lemma:inverse-approximation} and Remark \ref{Remark:convergence},  the
limit 
$$
\partial_t^p\partial_\theta^\alpha {\cal H}^{\beta}(\theta;\omega,t)  := 
\lim_{j\to \infty} \partial_t^p\partial_\theta^\alpha
\partial_\omega^\beta \left[ {\cal F}^j(\theta,0;\omega,t) -
(\theta,0;\omega) \right]\, ,\quad 
(\theta,\omega)\in {\T}^n\times \Omega_\kappa\, ,\ t\in [0,a]\, ,
$$
exists for each $0\le q\le k$ and  $\alpha,\beta  \in {\N}$ and it is uniform.   
Moreover, the partial derivatives of $ {\cal
H}^{\beta}$ exist, they are continuous on ${\T}^n\times
\Omega_\kappa\times [0,a]$, and $ \partial_t ^p\partial_\theta ^\alpha ({\cal
H}^{\beta}) =  \partial_t ^p\partial_\theta ^\alpha {\cal
H}^{\beta}$. By Remark \ref{Remark:restriction} the jet ${\cal H}^{\beta}$ does not depend on $m$. To get rid of the exponents of $\kappa^{-1}$ in Lemma \ref{Lemma:inverse-approximation} we make a partial dilation $\omega \to \kappa \omega$. More precisely, 
set $X:= \T^n\times \kappa \Omega_\kappa$, where $\kappa\Omega_\kappa=\{w=\kappa\omega:\, \omega\in \Omega_\kappa\}$,  and consider the jet
\[
{\cal H}=\left({\cal H}^{(\alpha,\beta)}\right)_{(\alpha,\beta)\in \N^{2n}}\in C^k([0,a], C^\infty(\T^n\times \Omega_\kappa))
\]
where 
\[
{\cal H}^{(\alpha,\beta)}(\theta,w,t) = \kappa^{-|\beta|}\partial_\theta^\alpha {\cal H}^{\beta}(\theta;\kappa^{-1}w,t)\, ,\quad 
(t,\theta,w)\in [0,a]\times X . 
\]
The jet ${\cal H} $ does not depend on $m$ since ${\cal H}^{\beta}$ is independent of $m$ on $X\times  [0,a]$. Set $x=(\theta,w)\in X$ and $\gamma=(\alpha,\beta)\in\N^{2n}$, and denote
\[
\langle P\rangle_{p, \ell;r,\kappa} := \sup_{0\le q \le p} \ \sup_{0\le t \le a}\|\partial_t^q P_t\|_{\ell;r,\kappa} . 
\]

Then for any integer $m\ge 1$ we get by Lemma \ref{Lemma:inverse-approximation} and \eqref{eq:smallness3} the following estimates
\begin{equation}  
\left\{
\begin{array}{rcll} 
\displaystyle |\overline{W}_0 \partial_t ^p
{\cal H}^{(\gamma)}(x,t)|  &\le&   \displaystyle C_m (\kappa r )^{-1} \langle P_t\rangle_{p,\ell(m);r,\kappa}
\quad \mbox{for} \quad |\gamma|\le m,
 \\ [0.3cm]
\displaystyle |\overline{W}_0\left(R^q_{x } 
\partial_t ^p{\cal H}\right)_\gamma(y,t)|
&\le&   \displaystyle C_m (\kappa r )^{-1} \langle P_t\rangle_{p,\ell(m);r,\kappa} |x-y|^{m+1-|\gamma|} \quad \mbox{for} \quad q+ |\gamma|\le m-1
                                         \label{eq:Whitney} 
\end{array}
\right.
\end{equation} 
and for each $0\le p\le k$ and 
  $x,y \in  X$,  
where  $C_m>0$ depends only on $k$, $m$, $n$, $\tau$ and $\vartheta_0$. 
Then using Theorem \ref{Th:Whitney}
we extend the Whitney jet ${\cal H}$ to a smooth  function ${\cal H}$ on 
$ [0,a]\times \T^n\times\R^n$ such that
\[
|\overline{W}_0 \partial_t ^p\partial_x^\gamma
{\cal H}(x,t)|  \le  B_m  (\kappa r )^{-1} \sup_{0\le q \le p} \ \sup_{0\le t \le a}\|\partial_t^q P_t\|_{\ell(m);r,\kappa}
\]
  for  $0\le q\le p$ and 
$|\gamma|\le m$. Moreover, $B_m$ depends only on $k$, $m$, $n$, $\tau$ and $\vartheta_0$. 


Recall that $\overline{W}_0 = {\rm diag}\, \left({\sigma_0}^{-1}{\rm Id}, 
{r}^{-1}{\rm Id},{h_0}^{-1}{\rm Id}\right)$ and that $h_0 = \kappa (\sigma_0/x_0)^{\tau+1}/2<\kappa$. 
Then setting $\Psi_t(\theta,\omega) = {\cal H}(\theta,\kappa\omega,t)+(\theta,\omega)$ and rescaling back $t$ with $T\ge 1$ given by \eqref{eq:T} (see the comments in Case 1. Sect. \ref{Sec:analytic-smoothing}), we get (ii), Theorem \ref{Theo:A}. \finishproof

\noindent
{\em Proof of Remark \ref{rem:analiticity-t}. } To prove the analyticity of $\Psi$ with respect to $t\in B(0,a)$ we  use Remark \ref{rem:analyticity-t-iteration} and Theorem \ref{Th:Whitney}. 
The Hamiltonians $P^j$ satisfy the hypothesis of Remark \ref{rem:analyticity-t-iteration}  in view of Proposition \ref{Lemma:approximation-lemma}, item {\em 4}. \finishproof



==> s9-KAM1-2701.tex <==
\section{KAM theorems}\label{Sec:KAM}
In this Section we prove  KAM theorems and obtain BNF for $C^k$ smooth families of Hamiltonians $t\to H_t$ or exact symplectic maps $t\to P_t$. The main novelty in it can be briefly summarized as follows 
\begin{itemize}
	\item The constant  $\epsilon$ in the smallness condition depends only on the dimension of the configuration space and on the exponent in the Diophantine condition;
	\item $C^k$ smooth families of invariant tori $t\to \Lambda_t(\omega)$ with Diophantine frequencies are obtained;
	\item $C^k$ smooth with respect to the parameter $t$ BNF is obtained around the union of $\Lambda_t(\omega)$;
	\item Uniform estimates in the whole scale of H\"older spaces are obtained.  To this end a new approach to the iterative schema is proposed. The Modified Iterative  Lemma proven in Sect. \ref{Prop:IterativeLemma} provides in a limit smooth functions in the whole domain $\Omega$  (not only on the Cantor set $\Omega_{ \kappa}$) with a good control of the H\"older  norms. In particular, it avoids the Whitney $C^\infty$ extension theorem. 
\end{itemize}
In order to formulate the main results we recall the notion of the Legendre transform.
Let $D\subset \R^d$, $d\ge 1$, be an open set. 
We say that a real valued function $F\in C^\infty(D,\R)$   is {\em non-degenerate} if
\begin{equation}\label{eq:non-degenerate}
\mbox{$\nabla F  : D \longrightarrow  D^\ast:=\nabla F(D) \subset \R^d$ is a diffeomorphism.}
\end{equation}
The Legendre transform $F^\ast$ of $F$ is defined by
\[
F^\ast(\xi)\, :=\,  \mbox{Crit.val.\,}_{x\in D}\{\langle x,\xi\rangle - F(x)\}
\]
which is equivalent to 
\begin{equation}\label{eq:L-transform}
F(x) + F^\ast(\xi) = \langle x, \xi \rangle\, , \ \mbox{where $x\in D$ and $\xi = \nabla F(x)\in D^\ast$.}
\end{equation}
It is easy to see that  $F^\ast\in C^\infty(D^\ast,\R)$ and that $\nabla F^\ast : D^\ast \longrightarrow {D}$ is the inverse  to the map  \eqref{eq:non-degenerate}.
Moreover, $D^{\ast\ast}= D$ and $F^{\ast\ast}= F$.

The real valued function  $F$  defines a non-degenerate (in Kolmogorov sense) completely integrable Hamiltonian in $\T^d\times D$. Hereafter, $\T^d:=\R^d/2\pi\Z^d$.  The corresponding Hamiltonian flow is given by $(s,\theta,r) \to (\theta + s\nabla F(r), r)$. The frequency vector of the restriction of the flow to the invariant torus $\T^{d}\times \{r\}$ is $\omega= \nabla F(r)\in \Omega:=D^\ast$ and the corresponding rotation vector is $\omega/2\pi$. We work here with  frequency vectors instead of rotation vectors because they are more adapted to the Fourier analysis. One can parameterize the invariant tori by their frequency vectors $\omega\in \Omega$ since $F$ is non-degenerate. We are interested below in  families of non-degenerate completely integrable Hamiltonians $F_t$, $t\in [0,\delta]$, with frequency vectors in a fixed open set $\Omega\subset \R^d$. To this end we consider  a family of non-degenerate functions $F^{\ast}_t\in C^\infty(\Omega)$ and define $F_t$ as the Legendre transform of $F^{\ast}_t$ in $D_t:= \nabla F^{ \ast}_t(\Omega)$. The advantage is that the set of frequency vectors is independent of the parameter $t$. In particular,  the Diophantine conditions will be  the same for all $t$. 
The same discussion holds as well for  families of completely integrable exact symplectic maps.

 

This part is organized as follows. The basic KAM theorem is proved in Sect. \ref{Sec:KAM-parameters}.   ?????

\subsection{KAM theorems for $C^k$ families of Hamiltonians}\label{Subsec:KAM-hamiltonians}
Let $\Omega\subset \R^{n}$ be   an \emph{ open convex  bounded set},  $k\in\{0;1\}$, and $\delta>0$.   Denote by $ \overline{\Omega}$ the closure of $\Omega$ in $\R^n$. Consider  a $C^k$ family $H^{0\ast}$  of real valued   functions 
\[
[0,\delta]\ni t\to H^{0\ast}(\cdot, t)= H_t^{0\ast}(\cdot)\in C^\infty( \overline{\Omega},\R)
\]
satisfying the non-degeneracy condition 
\begin{equation}\label{eq:non-degenerate2}
\mbox{$\nabla H_t^{0\ast} : \Omega \longrightarrow   D_t:=\nabla H_t^{0\ast}(\Omega)$ is a diffeomorphism}.    ?????
\end{equation}
%Hereafter $\overline\Omega$ stands for the closure of $\Omega$ in $\R^n$. 
The corresponding  family $H^{0}$ of Legendre transforms 
\[
[0,\delta]\ni t\to H_t^{0} =  H_t^{0\ast\ast}\in C^\infty(D_t,\R)
\]
is $C^k$ as well and 
$ H_t^{0}$ satisfies  \eqref{eq:non-degenerate} on $D_t$ for each $t$.  Consider a $C^k$ family $H$ of perturbations 
\[
[0,\delta] \ni t \to H(\cdot,t) = H_t(\cdot) \in C^\infty(\A_t,\R)
\]
of $H^0$ where $\A_t:=\T^n\times D_t$. 

Let us introduce the arithmetic conditions on the frequency vectors. 
Fix $\kappa >0$ and $\tau>n-1$, and denote by  $\widetilde D(\kappa,\tau)$ the set of all $\omega\in \R^n$ satisfying the 
 $(\kappa,\tau)$-Diophantine  condition 
\begin{equation}  
\forall\, 0\neq k\in \Z^{n}\  :  \quad                    
|\langle\omega,k\rangle |\ \ge \ \frac{\kappa}{|k|^{\tau}}\, . 
                       \label{eq:sdc2}                                        
\end{equation}
Denote by $\Omega_\kappa$ the set of all $(\kappa,\tau)$-Diophantine vectors $\omega\in\Omega$ such that the distance from $\omega$ to the complement $\R^{n}\setminus \Omega$ of $\Omega$ is $\ge \kappa$.  
We will often use the following notation 
\begin{equation}\label{eq:omega-kappa}
\left\{
\begin{array}{llcr}
\Omega +\kappa &:=& \{\omega\in \R^n :\ \mbox{\rm dist} (\omega, \Omega) <\kappa\}
\\[0.3cm]
\Omega -\kappa &:=& \{\omega\in \Omega :\ \mbox{\rm dist} (\omega,\R^{n}\setminus \Omega) >\kappa\}.
\end{array}
\right.
\end{equation}
Then $\Omega_\kappa= \widetilde D(\kappa,\tau)\cap \overline{\Omega -\kappa}$. 

In order to formulate the smallness condition   we need the following notations. Firstly we define  weighted $C^\ell$ H\"older norms as in \cite{Poe}. 
Given   $\ell\ge 0$, $0<\kappa\le 1$, and a domain $D\subset \R^n$, we denote the weighted (with respect to the small parameter $\kappa$)  $C^\ell$-norm of $u\in C^\ell( \T^n\times D,\R^k)$ evaluated at $\T^n\times D$ by 
\begin{equation}
\big\|u\big\|_{\ell,\T^n\times D;\kappa}:= \big\|u\circ \sigma_{\kappa}\big\|_{\,  C^\ell\left(\sigma_{\kappa}^{-1}(\T^n\times D)\right) }
\label{eq:holder-norms}
\end{equation}
where  $\|\cdot\|_{C^\ell}$ is the corresponding H\"older norm (see Sect. \ref{Sec:ApprLemma}) and 
$\sigma_{\kappa}:\T^n\times \R^n\to \T^n\times \R^n$ is  the partial dilation  $\sigma_{\kappa}(\theta,r):= (\theta, \kappa r)$. If $\ell\in\N$ then
\[
\big\|u\big\|_{\ell,\T^n\times D;\kappa}\, = \, \sup_{|\alpha|+|\beta|\le \ell}\, \sup_{(\theta,r)\in \T^n\times D}\, |\partial_\theta^\alpha (\kappa \partial_r)^\beta u(\theta,r)|,
\]
where $|\cdot|$ is the Euclidean norm. 
In the same way we introduce the norm $\|u\|_{\ell,D;\kappa}$ for $u\in C^\ell(D, \R^k)$. 
We set as well
\begin{equation}\label{eq:3-norm}
|\!|\!|u |\!|\!|_{\ell,D;\kappa}\, =\, \sup_{0\le m \le \ell}\|u\|_{\ell-m,D;\kappa}, \quad \mbox{where}\ m\in \N .
\end{equation}
If $D$ is \emph{convex}, then $|\!|\!|u |\!|\!|_{\ell,D;\kappa}\, =\, \|u\|_{\ell,D;\kappa}$. 
Given $\ell\ge 1$ and a family of functions $$u:=\{u_t\in C^\infty(\Omega,\R): \ t\in [0,\delta]\}$$ we set
\begin{equation}
\label{eq:S-sequence}
S_{\ell}(u) := \sup_{0\le t\le \delta }\, \big(1+ \|u_t\|_{C^1(\Omega)}\big)^{\ell-1} \big(1+ \|u_t\|_{C^\ell(\Omega)}\big).
\end{equation}
This expression
 arises   when one evaluates the   $C^\ell$-norms of a composition of functions the form $f_t\circ u_t$  with $u_t=\nabla K_t^{0\ast}$ (see Appendix, Sect. \ref{subsec:interpolation}). If $\Omega$ is {\em convex} then $\|u_t\|_{C^\ell(\Omega)}\le \|u_t\|_{C^\mu(\Omega)}$ for $0\le \ell\le \mu$ and the function $\ell \to S_{\ell}(u)$ becomes increasing in $[1,+\infty)$. 
 
Fix  $\vartheta_0>1$  and set 
\begin{equation}
\ell_0:=2\tau + 2 + 2\vartheta_0\quad \mbox{and} \quad  \ell(m):=  2m(\tau + 1)+ \ell_0 \, , \quad m \ge 0. 
\label{eq:ell(m)}
\end{equation}  
 Given $0<\varrho,\kappa \le 1$ and $m\ge 0$, we denote by ${\mathcal A}_m^0 $ the expression 
\begin{equation}
\label{eq:A-0-sequence}
{\mathcal A}_m^0 \, := \,  \sup_{0\le t\le \delta }\, \left( \varrho^2 |\!|\!| \partial^2 H_t^0 |\!|\!|_{\ell(m), D_t;\kappa} \, +\,  |\!|\!| H_t-H_t^0|\!|\!|_{\ell(m),\A_t; \kappa}\right)
\end{equation}
and set 
\begin{equation}
\label{eq:A-sequence}
{\mathcal A}_m \, =\, S_{\ell(m)+1}(\nabla H^{0\ast})\, {\mathcal A}_m^0 \, . 
\end{equation}
Here $\partial^2 H_t^0(I)$ is the Hessian matrix of $H_t^0$ at $I\in D_t$. The role of the small parameter $\varrho$ is to compensate the norm of Hessian matrix which  could be very large. The function $m\to {\mathcal A}_m$, $m\ge 0$, is {\em increasing} when $\Omega$ is convex. 


Let $\Phi_{t}^s := \exp\left(s X_{H_{t}} \right)$, $s\in\R$, be 
the flow of the Hamiltonian vector field $X_{H_{t}}$ with Hamiltonian $H_{t}$ in $ \A_t= \T^n\times  D_t$.  
Recall that  
for any $\omega\in \Omega$ the map  $R_{\omega}:\T^n\to\T^n$ stands for the translation $R_{\omega}(\varphi) =\varphi + \omega \, \mbox{\rm (mod $2\pi$)}$. 
Fix  $k\in \{0,1\}$. 

\begin{Theorem}\label{Theo:KAM2} There exists $\epsilon = \epsilon(n,\tau,\vartheta_0)>0$ depending only on $n$, $\tau$ and $ \vartheta_0$ such that 
the following holds.\\
\noindent
Let  $ \Omega\subset \R^{n}$ be  an  open convex  bounded set,  $0<\varrho\le\kappa\le 1$ and $\Omega_\kappa\neq\emptyset$. Let $H^{0\ast}$ be a $C^k$ family  of real-valued functions $[0,\delta]\ni t\to H_t^{0\ast}\in C^\infty( \overline\Omega,\R)$   satisfying \eqref{eq:non-degenerate2},  and let  
 $[0,\delta]\ni t\to H_t\in C^\infty( \A_t,\R)$ be a $C^k$ family of Hamiltonians such that
\begin{equation}\label{eq:smallness-condition2}
S_{\ell_0}(\nabla H^{0\ast})\,{\mathcal A}_0^0\,  =\, \sup_{0\le t\le \delta }\, \left( \varrho^2 |\!|\!|\partial^2 H_t^0 |\!|\!|_{\ell_0, D_t;\kappa} \, +\,  |\!|\!| H_t-H_t^0|\!|\!|_{\ell_0,\A_t; \kappa}\right) S_{\ell_0}(\nabla H^{0\ast}) \, 
\le \, \epsilon \varrho \kappa .
\end{equation}
Then there exists  a $C^k$ mapping $[0,\delta]\ni t\to    \Psi_t\in C^\infty(\T^{n}\times  \Omega; \T^{n}\times  D_t)$ of the form $\Psi_t(\theta, \omega)= (\theta, F_t(\theta,\omega))$ such that
\begin{enumerate}
\item[(i)]
for any $\omega\in \Omega_{\kappa}$,  
$[0,\delta]\ni s\to  \Lambda_t(\omega)=  \Psi_{t,\omega}(\T^{n})$ is a $C^k $  family of Kronecker invariant tori 
of the Hamiltonian vector fields $X_{H_t}$ with a frequency vector $\omega$, where $   \Psi_{t,\omega}:= \Psi_t(\cdot; \omega)$. Moreover, 
for any $\omega\in\Omega_\kappa$ and  $s\in\R$ the following diagram is commutative
\[
\displaystyle{\begin{array}{cccl} 
\displaystyle \T^{n}&\stackrel{R_{s\omega}}{\longrightarrow}&\T^{n}\cr
\downarrow\lefteqn{ \Psi_{t,\omega}}& &\downarrow\lefteqn{ \Psi_{t,\omega}} \cr
\displaystyle \Lambda_t(\omega)&\stackrel{\Phi_{t}^s}{\longrightarrow}&\Lambda_t(\omega)&  
\end{array} }
\]
\item[(ii)] for any $m\in \{0\}\cup [1,+\infty)$ the following estimates hold 
\begin{equation}\label{eq:estimates-tilde-F}
\begin{array}{lcrr}
\displaystyle \big|\partial_\varphi^\alpha (\kappa\partial_\omega)^\beta \big(\widetilde U_t(\varphi;\omega)-\varphi\big)\big| \, \le\,  C_m \frac{{\mathcal A}_m}{\kappa\varrho}\\[0.3cm]
\displaystyle
  \big|\partial_\varphi^\alpha (\kappa\partial_\omega)^\beta   \big(\widetilde V_t(\varphi;\omega)-\nabla H_t^{0\ast} (\omega)\big)\big| 
\, \le\,  C_m \frac{{\mathcal A}_m}{\varrho} \left(1+\frac{{\mathcal A}_1}{\varrho}\right)^{m} 
\end{array}
\end{equation}
for each $t\in [0,\delta]$, $(\varphi,\omega)\in \T^{n}\times \Omega$  and $\alpha,\beta\in \N^{n}$  with  $|\alpha| +|\beta|(\tau+1)\le m(\tau+1) +1$, where the constant $C_m>0$ depends only on $n$, $\tau$, $\vartheta_0$  and $m$. 
\item[(iii)]
${\rm supp\, }\big((\widetilde U_t,\widetilde V_t) -({\rm id}, \nabla H_t^{0\ast} )\big) \subset \T^{n}\times (\Omega-\kappa/2)$.
\end{enumerate}
\end{Theorem}





\noindent
{\em Proof}. 
The idea of the proof is given by P\"oschel in \cite{Poe1}. It can be summarized as follows.  Let us  fix $\omega\in \Omega$ set $r= \nabla H_t^{0 \ast}(\omega) + I$ and apply Taylor's formula up to order two to the function  $I\to H_t^0(\nabla H_t^{0 \ast}(\omega) + I)$ at $I=0$. Then the afine linear with respect to $I$ term is just $N_t(I;\omega)=e_t(\omega)+\langle I,\omega\rangle$ and we  put the quadratic term in the perturbation. Multiplying the perturbation by suitable cut-off functions  we obtain a Hamiltonian $\widetilde H_t(\theta,I;\omega)=N(I;\omega) + P_t(\theta,I;\omega)$, where $t\to P_t\in C^\infty(\T^n\times\R^n\times\Omega)$ is $C^k$ and $P_t$ are compactly supported with respect to $(I;\omega)$.  The smallness condition allows one  to apply Theorem \ref{Theo:A}. The main difficulty in the proof is to obtain the corresponding estimates in $C^\ell$, $\ell\ge 0$.
We devide the proof in several steps.\\

\noindent
{\em Step 1. Construction of the Hamiltonian $\widetilde H_t(\theta,I;\omega)$.}
Given $\omega\in \Omega -\kappa/4$ 
and $I$ in the ball $B^n(0,\varrho)\subset\R^n$ of center $0$ and radius $\varrho$,   we set 
$r=\nabla H^{0\ast}_t(\omega) + I$.  Choosing $\epsilon=\epsilon(n,\tau,\vartheta_0)\le 1/9$ in  \eqref{eq:smallness-condition2} we will show that
\begin{equation} \label{eq:domain-H}
\omega\in \Omega-\kappa/4,\ I\in B^n(0,\varrho) \quad \Longrightarrow \quad  \left\{
\begin{array}{lcrr}
\nabla H^{0\ast}_t(\omega) + I\in D_t \quad \mbox{and}\\[0.3cm]
\displaystyle \nabla  H^{0}_t(\nabla H^{0\ast}_t(\omega) + I)\in \Omega-\frac{1}{8}\kappa  
\end{array}
\right.
\end{equation}
for each $t\in [0,\delta]$.  Fix $t\in [0,\delta]$.  
The smallness condition \eqref{eq:smallness-condition2} implies that $\|\partial^2  H^{0}_t\|_{C^0(D_t)} \le \epsilon \kappa /\varrho$ since $S_{\ell_0}(\nabla H^{0\ast})>1$. Then  for each  $\omega\in \Omega-\kappa/4$  there is a positive number $c\le \varrho$ such that for any  $I\in B^n(0,c)$ the following relation holds
\begin{equation} \label{eq:domain-H-1}
 \left\{
\begin{array}{lcrr}
\nabla H^{0\ast}_t(\omega) + I\in D_t \quad \mbox{and}\\[0.3cm]
\displaystyle |\nabla  H^{0}_t(\nabla H^{0\ast}_t(\omega) + I) -\omega|\,  \le \, \|\partial^2  H^{0}_t\|_{C^0(D_t)}\, |I|\,  \le\,  \epsilon \kappa \frac{c}{\varrho}\,  <\,  \frac{\kappa}{9}  \, .
\end{array}
\right.
\end{equation}
Using the notations \eqref{eq:omega-kappa} one obtains 
\[
\nabla  H^{0}_t(\nabla H^{0\ast}_t(\omega) + I)\in (\Omega-\kappa/4)+\kappa/9=(\Omega-\kappa/8)-\kappa/72
\] 
for any $I\in B^n(0,c)$. If $c<\varrho$, then there exists $c<c'\le\varrho$ such that  \eqref{eq:domain-H-1} still holds for each $I\in B^n(0,c')$. 
This  proves  \eqref{eq:domain-H}. 
Then  Taylor's formula yields
\[
H_t^0(r) = e_t(\omega) + \langle I,\omega\rangle + \int_0^1(1-s)\langle \partial^2H_t^0(\nabla H_t^{0\ast}(\omega) + sI)I,I\rangle\,  ds.
\]
for  $\omega\in \Omega-\kappa/4$ and $I\in B^n(0,\varrho)$,  
where $e_t(\omega) := H_t^0(\nabla H^{0\ast}_t(\omega))$. 

In order to apply Theorem \ref{Theo:A}  we need  suitable cut-off functions. 
\begin{Lemma}\label{lemma:cut-off-omega}
	For any open set $U\subset \R^n$ and $0<\varepsilon\le 1$ there exists a smooth cut-off function  $\psi^U_\varepsilon\in C_0^\infty(\R^{n}, [0,1])$
	such that 
	$\psi^U_\varepsilon=1$ on $U-\varepsilon$, $\psi^U_\varepsilon=0$ on the complement of $U + \varepsilon$, and
	\[
	\|\psi^U_\varepsilon\|_{\ell;\varepsilon} \le C_\ell
	\]
	for any $\ell\ge 0$, where the positive constants $C_\ell=C(\ell,n)$ depend only on $\ell$ and $n$.
\end{Lemma}
The proof of the Lemma is given in the Appendix, Sect. \ref{subsec:composition-inverse}. \\

Denote by $\psi_\kappa\in C_0^\infty(\R^{n}, [0,1])$ the function given by Lemma \ref{lemma:cut-off-omega} with $U=\Omega-\kappa/2$ and $\varepsilon=\kappa/4$. Then  $\psi_\kappa=1$ on $\Omega-3\kappa/4$, $\psi_\kappa=0$ on the complement of $\Omega-\kappa/4$, and
\begin{equation}\label{eq:estimates-psi-kappa}
\| \psi_\kappa\|_{\ell;\kappa} \le C_\ell
\end{equation}
for any $\ell\ge 0$, where the constants $C_\ell=C(\ell,n)$ depend only on $\ell$ and $n$. Let $\widetilde\psi_\varrho$ be the cut-off function given by  Lemma \ref{lemma:cut-off-omega} with $U=B^n(0, 3\varrho/4)$ and  $\varepsilon=\varrho/4$. Then the support of $ \widetilde\psi_\varrho$ is contained in   $B^n(0,\varrho)$, $\widetilde\psi_\varrho=1$ on $B^n(0,\varrho/2)$, and 
\begin{equation}\label{eq:estimates-psi-rho}
\|\widetilde\psi_\varrho\|_{\ell;\varrho} \le C_\ell
\end{equation}
for any $\ell\ge 0$, where the constants $C_\ell=C(\ell,n)$ depend only on $\ell$ and $n$.





It follows from \eqref{eq:domain-H} that the function 
\[
P_t^0(I;\omega):= \int_0^1(1-s)\langle \partial^2H_t^0(\nabla H_t^{0\ast}(\omega) + sI)I,I\rangle \psi_\kappa(\omega)\widetilde \psi_{\varrho}(I)\,  ds,
\]
is well defined and compactly supported in $B^n(0,\varrho)\times \Omega$. 
Setting
\[
P_t^1(\theta,I;\omega):= (H_t-H_t^0)(\theta, \nabla H^{0\ast}_t(\omega) + I)\psi_\kappa(\omega)\widetilde\psi_{\varrho}(I)\quad \mbox{and}  \quad P_t:= P_t^0 + P_t^1, 
\]
we consider the Hamiltonian
\[
\widetilde H_t(\theta,I;\omega)= e_t(\omega) + \langle I,\omega\rangle + P_t(\theta, I;\omega).
\]
We have 
\begin{equation}\label{eq:equality-for-H}
H_t(\theta,\nabla H^{0\ast}_t(\omega) + I)=\widetilde H_t(\theta,I;\omega)
\end{equation}
 for $I\in B^n(0,\varrho/2)$ and $\omega\in \Omega-3\kappa/4$. \\

\noindent
{\em Step 2. H\"older estimates of $P_t$.}
For any $\ell\ge 1$ we are going to evaluate  the weighted norm 
\[
\|P_t\|_{\ell;r,\kappa} := \|P_t\circ \sigma_{r,\kappa}\|_{C^\ell(U)}\, , \quad U:=\sigma_{r,\kappa}^{-1}(\T^n\times B^n(0,\varrho)\times \Omega), 
\]
introduced in \eqref{eq:norm-rho-kappa}. In order to estimate  $\|P_t^0\|_{\ell;r,\kappa}$ we 
set $\Gamma:= B^n(0,\varrho)\times (\Omega-8\kappa/9)$, $\Gamma_t:= B^n(0,\varrho)\times D_t$, 
\[
Q_t^1(I,r)=\int_0^1(1-s)\,  \partial^2H_t^0(r+sI)\, ds 
\]
and $Q_t^0(I,r)= \langle Q_t^1(I,r)I,I\rangle$ for $(I,r)\in \Gamma_t$. 
Then we write 
\[
P_t^0(I,\omega)=\psi_\kappa(\omega)\widetilde\psi_{\varrho}(I)Q_t^0(I, \nabla H_t^{0\ast}(\omega)). 
\] 
The function $Q_t^0\circ ({\rm id}, \nabla H_t^{0\ast}) $ belongs to $C^\infty(\overline \Gamma)$, where $\Gamma$ is convex. Then 
using Remark \ref{rem:interpolation}, \eqref{eq:estimates-psi-kappa} and \eqref{eq:estimates-psi-rho} we obtain
\[
\|P_t^0\|_{\ell;\varrho,\kappa}  \,  \le  \, 
C_{\ell} \|Q_t^0\circ ({\rm id}, \nabla H_t^{0\ast}) \|_{\ell;\varrho,\kappa}.
\]
Proposition \ref{prop:composition-holder1}, {\em 3}, and Remark \ref{rem:anisotrop}
imply for  any  $\ell\ge 1$  the estimate
\[
\|Q_t^0\circ ({\rm id}, \nabla H_t^{0\ast}) \|_{\ell;\varrho,\kappa} \, \le  \, 
C_{\ell} \,  |\!|\!| Q_t^0|\!|\!|_{\ell,\Gamma_t;\varrho,\kappa}  \, 
S_{\ell}(\nabla H^{0\ast}), 
\]
where the norm $ |\!|\!| \cdot |\!|\!|$ is defined in \eqref{eq:3-norm}. 
Using  \eqref{eq:Leibnitz1}  and the inequality $0<\varrho\le\kappa$ we obtain 
\[
\| Q_t^0\|_{\ell,\Gamma_t;\varrho,\kappa} \le  C_{\ell} \, \varrho^2 |\!|\!| Q_t^1|\!|\!|_{\ell, \Gamma_t;\varrho,\kappa}  \le  C_{\ell} \, \varrho^2 |\!|\!| Q_t^1|\!|\!|_{\ell, \Gamma_t;\kappa,\kappa} \le  C_{\ell} \, \varrho^2 |\!|\!| \partial^2 H_t^0 |\!|\!|_{\ell, D_t;\kappa} 
\]
as $|I|\le \varrho$ for $(I,r)\in\Gamma_t$. This inequality implies
\[
|\!|\!| Q_t^0|\!|\!|_{\ell,\Gamma_t;\varrho,\kappa} \le  C_{\ell} \, \varrho^2 |\!|\!| \partial^2 H_t^0 |\!|\!|_{\ell, D_t;\kappa} 
\]
and we obtain
\[
\|P_t^0\|_{\ell;\varrho,\kappa}  \,  \le  \, 
C_{\ell} \, \varrho^2\, |\!|\!| \partial^2H^0 |\!|\!|_{ \ell, D_t; \kappa}  \, 
S_{\ell}(\nabla H^{0\ast}).  
\]
On the other hand $\|P_t^1\|_{\ell;\varrho,\kappa} \le \|P_t^1\|_{\ell;\kappa,\kappa}$  since $0<\varrho\le \kappa\le 1$ and by the same argument we get
\[
\|P_t^1\|_{\ell;\varrho,\kappa} 
\le C_{\ell} |\!|\!|H_t-H_t^0|\!|\!|_{\ell,\A_t; \kappa}
S_{\ell}(\nabla H^{0\ast}).
\]
Finally we obtain
\begin{equation}\label{eq:estimate-P-with-H}
\|P_t\|_{\ell;\varrho,\kappa} 
\le \displaystyle C_{\ell} \left(\varrho^2\, |\!|\!| \partial^2H^0_t |\!|\!|_{ \ell, D_t; \kappa}\, +\, |\!|\!|H_t-H_t^0|\!|\!|_{\ell,\A_t; \kappa}\right)\ 
S_{\ell}(\nabla H^{0\ast}).
\end{equation}


\noindent
{\em Step 3. Application of Theorem \ref{Theo:A} .}
The estimate  \eqref{eq:smallness-condition2} gives 
\begin{equation} \label{eq:0-estimates-P}
\|P_t\|_{\ell_0;\varrho,\kappa} \, \le \, C\,  {\mathcal A}_0 S_{\ell_0}(\nabla H_t^{0\ast}) \, \le\,   C \, \epsilon \varrho \kappa \, .
\end{equation}
This allows us to apply Theorem \ref{Theo:A} to the Hamiltonian $(\theta,I)\to \widetilde H_t(\theta,I;\omega)$. 
Consider the map  $ \Psi_t = (U_t, \widetilde V_t)$, where $\widetilde V_t=(\nabla H^{0\ast}_t)\circ \phi_t +V_t$ while $(U_t,V_t,\phi_t)$ are given by Theorem  \ref{Theo:A}. Notice that $\|V_t\|_{C^0} \le c\epsilon \varrho$ in view of the estimates in (ii), Theorem \ref{Theo:A}, where the constant $c$ depends only on  $n$, $\tau$ and $\vartheta_0$, and taking $\epsilon<\min(1,1/c)/2$ we obtain $V_t(\theta;\omega)\in B^n(0,\varrho/2)$ for any $\theta\in \T^n$ and $\omega\in \Omega-\kappa$. In the same way we get $\phi_t(\omega)\in \Omega-3\kappa/4$ for $\omega\in \Omega-\kappa$. In particular, $\widetilde\psi_{\varrho}(V_t(\theta;\omega))=1$ and $\psi_{\kappa}(\phi_t(\omega))=1$ for any  $(\theta,\omega)\in \T^n\times (\Omega-\kappa)$. 

Now  Remark  \ref{rem:Kronecker} and \eqref{eq:equality-for-H} imply that for any $\omega\in \Omega_\kappa$ and $t\in [0,\delta]$ the Lagrangian manifold 
$ \Lambda_t(\omega):=  \Psi_{t}(\T^n;\omega)$
is a Kronecker invariant torus of $H_t$ of a frequency vector $\omega$ satisfying  (i) in Theorem \ref{Theo:KAM2}.  \\

\noindent
{\em Step 4. Writing $\Lambda_t(\omega)$ as graphs.}\quad  
We are going to solve the equation $\varphi=\widetilde U_t(\theta,\omega)$ with respect to $\theta$ and get the respective estimates of the solution. It follows from \eqref{eq:main-estimates} that
\[
|\partial_{\theta}^\alpha (U_t(\theta;\omega) - \theta)| \le C_0(n,\tau,\vartheta_0)  (\kappa  r )^{-1}\,   \sup_{t\in [0,a]} \, \|P_t\|_{\ell_0;r,\kappa} \le c \epsilon < 1/2
\]
choosing $\epsilon$ small enough. By the implicit function theorem, there exists $\psi_t: \A  \to \T^n$ such that $U_t(\theta+\psi_t(\theta;\omega);\omega) = \theta +\psi_t(\theta;\omega)$ 
for each $(\theta,\omega)\in \A =\T^n\times \R^n$. To estimate the derivatives of $\psi_t$ we consider 
 the map $w_t: \A\to\A$ defined by $w_t(\theta,\omega)=(\widetilde U_t(\theta,\omega),\omega)$. 
%Recall from Theorem \ref{Theo:KAM}, $(iii)$, that ${\rm supp}\, (w_t-{\rm id})\subset \T^{n-1}\times (\Omega-\kappa/2)$.
It follows from \eqref{eq:main-estimates}   that 
\[
\|\sigma_\kappa^{-1}(w_t-{\rm id})\|_{1;\kappa} = \|w_t-{\rm id}\|_{1;\kappa} \le C_1\epsilon <(2n-2)^{-1}
\]
choosing $\epsilon = \epsilon(n,\tau, \vartheta_0)$ small enough (recall that $C_1$ depends only on $n$, $\tau$ and $\vartheta_0$). Then 
applying Proposition \ref{prop:inverse-holder1} we obtain a solution $\theta_t(\varphi,\omega)=\varphi+\psi_t(\varphi,\omega)$ of the equation  $\varphi=u_t(\theta,\omega)$, where $(\varphi,\omega)\in\T^{n-1}\times \Omega$. Then ${\rm supp}\, \psi_t\subset \T^{n-1}\times (\Omega-\kappa/2)$ and 
\begin{equation}\label{eq:derivatives-theta}
\|\psi_t\|_{m;\kappa} \, \le \,  \frac{C_m}{\kappa\varrho }\,  {\mathcal B}_m 
\end{equation}
for any $m\in\N$, where the constant $C_m>0$ depends only on $n$, $\tau$, $\vartheta_0$ and $m$. Setting $\widetilde F_t(\varphi,\omega)= v_t(\theta_t(\varphi,\omega),\omega)$ and 
\begin{equation}
\label{eq:F}
F_t(\varphi,\omega):=  -\nabla K_t^{\ast}(\omega) + \widetilde F_t(\varphi,\omega)) 
\end{equation}
for $(\varphi,\omega)\in \T^{n-1}\times \Omega$ we write
\begin{equation}\label{eq:kam-tori-F}
\Lambda_t(\omega)=\{(\varphi, \widetilde F_t(\varphi,\omega)):\, \varphi\in \T^{n-1}\}=\{(\varphi, \nabla K_t^{\ast}(\omega) +  F_t(\varphi,\omega)):\, \varphi\in \T^{n-1}\},\ \omega\in \Omega_\kappa .
\end{equation}
Notice that that ${\rm supp}\, F_t\subset \T^{n-1}\times (\Omega-\kappa/2)$. 
We are going to prove that
\begin{equation}\label{eq:derivatives-F}
\|F_t\|_{m;\kappa}   \, \le \,  \frac{C_m}{\varrho}  \, {\mathcal B}_m ,
\end{equation}
for any $m\in\N$, where the constant $C_m>0$ depends only on $n$, $\tau$, $\vartheta_0$ and $m$. 
To this end we write
\[
F_t(\varphi,\omega) = \big(v_t(\varphi,\omega)- \nabla K_t^{\ast}(\omega)\big) + \big(v_t(\theta_t(\varphi,\omega),\omega)-v_t(\varphi,\omega)\big). 
\]
The estimate of $v_t(\varphi,\omega)- \nabla K_t^{\ast}(\omega)$ follows directly from \eqref{eq:estimates-F-1} using the inequality ${\mathcal B}_1\le {\mathcal B}_2 \le \varepsilon\kappa\varrho\le \varrho$. To obtain the estimate of the second term of \eqref{eq:F} we write
\[
v_t(\theta_t(\varphi,\omega),\omega)-v_t(\varphi,\omega) \, =\, \displaystyle \int_0^1 (d_\theta v_t)(\varphi+s\psi_t(\varphi,\omega))\, \psi_t(\varphi,\omega)\,  ds .
\]
Then one  uses \eqref{eq:interpolation-leibnitz}, Proposition \ref{prop:composition-holder1}, {\em 2},  and  \eqref{eq:smallness-condition-1} as well. \\



\noindent
{\em Step 5. H\"older Estimates of $\widetilde U_t$ and $\widetilde V_t$.}
The estimates (ii), Theorem \ref{Theo:A}, imply (ii) in Theorem \ref{Theo:KAM2} using the estimates of $\displaystyle\| P_t\|_{\ell;\varrho,\kappa}$ given above. To estimate the derivatives of 
\[
\widetilde V_t- \nabla H^{0\ast}_t = V_t+ (\nabla H^{0\ast}_t)\circ \phi_t - \nabla H^{0\ast}_t
\]
we use (ii), Theorem \ref{Theo:A} and the following
\begin{Lemma}\label{lemma:estimates-V}
For any $m\in \{0\}\cup [1,+\infty)$ the following estimate holds
\[
\|(\nabla H^{0\ast}_t)\circ \phi_t - \nabla H^{0\ast}_t\|_{m,\Omega;\kappa} \le C_{m} \frac{{\mathcal A}_m}{\varrho}\left(1+\frac{{\mathcal A}_1}{\varrho} \right)^m.
\]
\end{Lemma}
{\em Proof}. 
The proof of the lemma  is based on higher order  H\"older estimates of a composition of functions given in the Appendix. 
 We write
\[
\nabla H^{0\ast}_t(\phi_t(\omega))- \nabla H^{0\ast}_t(\omega) = u_t(\omega)\cdot v_t(\omega)
\]
where 
\[
u_t(\omega)= \phi_t(\omega)-\omega\in M_{1,n}(\R) \quad \mbox{and} \quad v_t(\omega)=\int_0^1 (\partial^2 H^{0\ast}_t)(\omega + s(\phi_t(\omega)-\omega))\,  ds \in M_{n,n}(\R). 
\]
Theorem \ref{Theo:A} and \eqref{eq:estimate-P-with-H} imply
\[
\|\phi_t-{\rm id}\|_{m,\Omega;\kappa}\,  \le\, C_m\frac{{\mathcal A}_m^0}{\varrho} S_{\ell(m)}(\nabla H^{0\ast}) 
\]
where
\[
S_{\ell(m)}(\nabla H^{0\ast}) = \sup_{0\le t\le \delta}\big(1+ \|\nabla H^{0\ast}_t\|_{1}\big)^{\ell(m)-1}\big(1+ \|\nabla H^{0\ast}_t\|_{\ell(m)}\big) 
\]
is increasing with respect to $m\in\N$ since $\Omega$ is convex. 
Moreover, \eqref{eq:smallness-condition2} yields $\|\phi_t-{\rm id}\|_{0} \le C \varepsilon \kappa$. 
Notice that $v_t$ is well-defined and $C^\infty$ smooth in the convex set $\overline \Omega$. Indeed, the image of $\Omega$ under the map $\omega\mapsto \omega + s(\phi_t(\omega)-\omega)$ is contained in  $\Omega$ when $\varepsilon<1/2C$ since 
${\rm supp\, }(\phi_t -{\rm id})\subset \Omega- \kappa/2$ and $\|\phi_t-{\rm id}\|_0 <\kappa/2$. 


Let $m=0$. Then
\[
\|(\nabla H^{0\ast}_t)\circ \phi_t - \nabla H^{0\ast}_t\|_{C^0(\Omega)}\, \le\,  C_0\frac{{\mathcal A}_0^0}{\varrho} S_{\ell_0}(\nabla H^{0\ast}) \|\nabla H^{0\ast}_t\|_{C^1(\Omega)} \, < \, C_0\frac{{\mathcal A}_0^0}{\varrho} S_{\ell_0+1}(\nabla H^{0\ast}) \, = \, 
C_{0} \frac{{\mathcal A}_0}{\varrho}
\]
since $\Omega$ is convex. 

Let $m\ge 1$. Using  Remark \ref{rem:interpolation} we get 
\[
\|\nabla H^{0\ast}_t\circ \phi_t- \nabla H^{0\ast}_t\|_{m,\Omega;\kappa}\,  \le\, C_m \big( \|\phi_t-{\rm id}\|_{m,\R^n;\kappa}\|v_t\|_{C^0(\Omega)} 
+\|\phi_t-{\rm id}\|_{C^0(\R^n)}\|v_t\|_{m,\Omega;\kappa}\big).
\]
We obtain as above
\[
\begin{array}{rcll}
\displaystyle \|\phi_t-{\rm id}\|_{m,\R^n;\kappa}\|v_t\|_{C^0(\Omega)} \, \le\, C_m\frac{{\mathcal A}_m^0}{\varrho} S_{\ell(m)}(\nabla H^{0\ast}) \|\nabla H^{0\ast}_t\|_{C^1(\Omega)}\\[0.3cm] 
\displaystyle  < \, C_m\frac{{\mathcal A}_m^0}{\varrho} S_{\ell(m)+1}(\nabla H^{0\ast})  = C_m\frac{{\mathcal A}_m}{\varrho}
  \end{array}
\]
since $\Omega$ is convex. 
On the other hand, Proposition \ref{prop:composition-holder-interpolation}, {\em 3}, applied to $f=({\rm id} +s(\phi_t-{\rm id}))\circ \sigma_\kappa$ and $g=\partial^2 H^{0\ast}_t\in C^\infty(\overline \Omega, M_{n,n}(\R))$ yields
\[
\begin{array}{rcll}
\|v_t\|_{m,\Omega;\kappa} &\le& C_m \big(1+  \|\phi_t-{\rm id}\|_{1;\kappa}^{m-1}\big)\\[0.3cm]
 &\times& \displaystyle  \, \big(\|\nabla H^{0\ast}\|_{m+1}(1+ \|\phi_t-{\rm id}\|_{1})+\|\nabla H^{0\ast}\|_{2}\|\phi_t-{\rm id}\|_{m;\kappa} \big)
 \end{array}
\]
where the corresponding  $C^\ell$ norms of $\nabla H^{0\ast}$  are evaluated on $\Omega$. Then
\[
\begin{array}{lcrr}
\displaystyle\|\phi_t-{\rm id}\|_{C^0(\R^n)}\|v_t\|_{m,\Omega;\kappa}\, \le\, C_m \frac{{\mathcal A}_0^0}{\varrho}\Big(1+\frac{{\mathcal A}_1}{\varrho}\Big)^{m-1}S_{\ell_0}(\nabla H^{0\ast}) \\[0.3cm]
 \displaystyle \times\, \left(\|\nabla H^{0\ast}\|_{m+1}\Big(1+\frac{{\mathcal A}_1}{\varrho}\Big) +  \|\nabla H^{0\ast}\|_{2} \frac{{\mathcal A}_m^0}{\varrho} S_{\ell(m)}(\nabla H^{0\ast})  \right)
\end{array}
\]
The interpolation inequalities \eqref{eq:interpolation} and  Remark \ref{rem:interpolation}  yield  for any $ r, s \ge 1$ and $f\in C^{r+s-1}(\overline\Omega)$ the estimate 
$\|f\|_r\|f\|_s \le C_{r,s} \|f\|_1\|f\|_{r+s-1}$, where $C_{r,s}>0$ depends only on $r,s$ and  $n$. Applying this inequality to $f= \nabla K_t^\ast$ and using the convexity of $\Omega$ we obtain
\[
S_{\ell_0}(\nabla H^{0\ast})\|\nabla H_t^{0\ast}\|_{m+1} < C_m S_{\ell_0+m}(\nabla H^{0\ast})< C_mS_{\ell(m)+1}(\nabla H^{0\ast})
\]
and 
\[
S_{\ell(m)}(\nabla H^{0\ast})\|\nabla H_t^{0\ast}\|_{2} \le C_m S_{\ell(m)+1}(\nabla H^{0\ast}).
\]
On the other hand ${\mathcal A}_0^0S_{\ell_0}(\nabla H^{0\ast}) \le \varepsilon \kappa\varrho$ by \eqref{eq:smallness-condition2} and ${\mathcal A}_0^0 \le {\mathcal A}_m^0$ for $m\ge 0$ by definition 
and  we obtain 
\[
\|\phi_t-{\rm id}\|_{C^0(\R^n)}\|v_t\|_{m,\Omega;\kappa}\, \le\, C_m \frac{{\mathcal A}_m}{\varrho}\Big(1+\frac{{\mathcal A}_1}{\varrho}\Big)^{m}
\]
This completes the proof of the Lemma. 
 \finishproof
 
 \noindent
 {\em Step 4. Writing $\Lambda_t(\omega)$ as graphs.}\quad  
 For any $\omega\in \Omega_\kappa$ and $t\in [0,\delta]$ the Lagrangian manifold 
 \[
 \Lambda_t(\omega):= \left\{\left(u_t(\theta;\omega), v_t(\theta;\omega)\right):\, \theta\in\T^n \right\}
 \]
 given by Theorem \ref{Theo:KAM}
 is a Kronecker invariant torus of $P_t$ of a frequency vector $\omega$ satisfying (i) of Theorem \ref{Theo:KAM}. 
 Firstly we will solve the equation $\varphi=u_t(\theta,\omega)$ with respect to $\theta$ and get the respective estimates of the solution. 
 To this end we consider the map $w_t: \A\to\A$ defined by $w_t(\theta,\omega)=(u_t(\theta,\omega),\omega)$, where $\A=\T^{n-1}\times \R^{n-1}$. Recall from Theorem \ref{Theo:KAM}, $(iii)$, that ${\rm supp}\, (w_t-{\rm id})\subset \T^{n-1}\times (\Omega-\kappa/2)$.
 It follows from \eqref{eq:estimates-F-1} and \eqref{eq:smallness-condition-1}  that 
 \[
 \|\sigma_\kappa^{-1}(w_t-{\rm id})\|_{1;\kappa} = \|w_t-{\rm id}\|_{1;\kappa} \le C_1\epsilon <(2n-2)^{-1}
 \]
 choosing $\epsilon = \epsilon(n,\tau, \vartheta_0)$ small enough (recall that $C_1$ depends only on $n$, $\tau$ and $\vartheta_0$). Then 
 applying Proposition \ref{prop:inverse-holder1} we obtain a solution $\theta_t(\varphi,\omega)=\varphi+\psi_t(\varphi,\omega)$ of the equation  $\varphi=u_t(\theta,\omega)$, where $(\varphi,\omega)\in\T^{n-1}\times \Omega$. Then ${\rm supp}\, \psi_t\subset \T^{n-1}\times (\Omega-\kappa/2)$ and 
 \begin{equation}\label{eq:derivatives-theta}
 \|\psi_t\|_{m;\kappa} \, \le \,  \frac{C_m}{\kappa\varrho }\,  {\mathcal B}_m 
 \end{equation}
 for any $m\in\N$, where the constant $C_m>0$ depends only on $n$, $\tau$, $\vartheta_0$ and $m$. Setting $\widetilde F_t(\varphi,\omega)= v_t(\theta_t(\varphi,\omega),\omega)$ and 
 \begin{equation}
 \label{eq:F}
 F_t(\varphi,\omega):=  -\nabla K_t^{\ast}(\omega) + \widetilde F_t(\varphi,\omega)) 
 \end{equation}
 for $(\varphi,\omega)\in \T^{n-1}\times \Omega$ we write
 \begin{equation}\label{eq:kam-tori-F}
 \Lambda_t(\omega)=\{(\varphi, \widetilde F_t(\varphi,\omega)):\, \varphi\in \T^{n-1}\}=\{(\varphi, \nabla K_t^{\ast}(\omega) +  F_t(\varphi,\omega)):\, \varphi\in \T^{n-1}\},\ \omega\in \Omega_\kappa .
 \end{equation}
 Notice that that ${\rm supp}\, F_t\subset \T^{n-1}\times (\Omega-\kappa/2)$. 
 We are going to prove that
 \begin{equation}\label{eq:derivatives-F}
 \|F_t\|_{m;\kappa}   \, \le \,  \frac{C_m}{\varrho}  \, {\mathcal B}_m ,
 \end{equation}
 for any $m\in\N$, where the constant $C_m>0$ depends only on $n$, $\tau$, $\vartheta_0$ and $m$. 
 To this end we write
 \[
 F_t(\varphi,\omega) = \big(v_t(\varphi,\omega)- \nabla K_t^{\ast}(\omega)\big) + \big(v_t(\theta_t(\varphi,\omega),\omega)-v_t(\varphi,\omega)\big). 
 \]
 The estimate of $v_t(\varphi,\omega)- \nabla K_t^{\ast}(\omega)$ follows directly from \eqref{eq:estimates-F-1} using the inequality ${\mathcal B}_1\le {\mathcal B}_2 \le \varepsilon\kappa\varrho\le \varrho$. To obtain the estimate of the second term of \eqref{eq:F} we write
 \[
 v_t(\theta_t(\varphi,\omega),\omega)-v_t(\varphi,\omega) \, =\, \displaystyle \int_0^1 (d_\theta v_t)(\varphi+s\psi_t(\varphi,\omega))\, \psi_t(\varphi,\omega)\,  ds .
 \]
 Then one  uses \eqref{eq:interpolation-leibnitz}, Proposition \ref{prop:composition-holder1}, {\em 2},  and  \eqref{eq:smallness-condition-1} as well. 
 
 
\noindent 
Statement  (iii) follows from the definition of $\widetilde U$ and $\widetilde V$ using Theorem  \ref{Theo:A}.  \finishproof

\subsection{KAM theorem with parameters for  symplectic maps}\label{Subsec:KAM-maps-parameters}
We are going to prove an analogue of Theorem \ref{Theo:A} for symplectic maps. More precisely, given a $C^k$ family of ``small'' exact symplectic  perturbations $(\theta,r) \to P_t(\theta,r;\omega)$ of the translation  $(\theta,r)\to R_\omega(\theta,r):= (\theta+\omega,r)$ with a Diophantine frequency $\omega$, we are going to find a $C^k$ family of Kronecker invariant tori of $P_t(\theta,r;\phi_t(\omega))$, where $t\to \phi_t$ is a $C^k$ family of diffeomorphisms close to the identity map. Moreover, we will estimate the $C^m$, $m\in\N$,  norm of $\phi_t -{\rm id}$, and of the displacement of the Kronecker tori with respect to the corresponding inperturbed tori.

Let $\Omega \subset [0,2\pi)^{n-1}$ be an open convex set.  We identify $\Omega$ with an open convex subset of $\T^{n-1}$. Fix $k\in \{0, 1\}$ and $\varrho_0>0$ and  consider a $C^k$ family of exact symplectic maps 
\[
[0,\delta]\ni t\to P_t(\cdot;\omega)\in C^\infty(\T^{n-1}\times B^{n-1}(0,\varrho_0), \T^{n-1}\times \R^{n-1})
\]
 depending smoothly on a parameter $\omega\in \Omega$. 
 We suppose that  $P_t(\cdot;\omega)$ is defined by a generating functions $\widetilde G_t(\cdot;\omega)$ of the form
\begin{equation} 
\label{eq:generating-function-of P}
\widetilde G_t(\theta,r;\omega):= \langle \theta,r\rangle -\langle \omega,r\rangle -G_t(\theta,r;\omega)
\end{equation}
i.e. 
\[
P_t(\theta-\omega-\nabla_{r}G_t(\theta,r;\omega),r;\omega)=(\theta, r-\nabla_{\theta}G_t(\theta,r;\omega),r)
\]
for any $(\theta,r)\in \T^{n-1}\times B^{n-1}(0,\varrho_0)$ and $\omega\in \Omega$ and  that the $C^2$ norm of $G_t(\cdot;\omega)$ is  sufficiently small. 
 If $G_t=0$ then $P_t(\cdot;\omega)$ becomes a translation with $\omega$, namely, 
$R_\omega(\theta,r)=(\theta+\omega,r)$.  In general we consider $G_t$ as a small perturbation  depending smoothly on the frequency $\omega$ as well. 
Thus the perturbation is a  real valued function $(\theta,I;\omega,t) \mapsto G(\theta,I;\omega,t)$ defined in $\A\times \Omega\times [0,\delta]$, where $\A:= \T^n\times B(0,\varrho_0)$. Hereafter, we assume that
\begin{equation}
G\in C^k\left([0,\delta];C^\infty(\A\times  \Omega)\right)
\label{eq:families-of-perturbations-maps}
\end{equation}
with $k=0$ or $k=1$, 
i.e. the map 
  $t\to G_t:=G(\cdot,t)\in C^\infty(\T^{n-1}\times B(0,\rho_0)\times  \Omega)$ is  $C^k$-smooth on the interval $[0,\delta]$.  

Given  $\ell>0$ and $0<\varrho,\kappa\le 1$ we denote by $\|G_t\|_{\ell;\varrho,\kappa}$ the  weighted H\"older norm 
\begin{equation}\label{eq:norm-rho-kappa-maps}
\|G_t\|_{\ell;\varrho,\kappa} := \|G_t\circ \sigma_{\varrho,\kappa}\|_{C^\ell(\sigma_{\varrho,\kappa}^{-1}(\A\times  \Omega))}
\end{equation}
where  $\sigma_{\varrho,\kappa}$ is  the partial dilation  $\sigma_{\varrho,\kappa}(\varphi,I;\omega):= (\varphi, \varrho I; \kappa \omega)$ and the  H\"older norms are defined in Section \ref{Sec:ApprLemma}. Note that the function $\ell \to \|G_t\|_{\ell;\varrho,\kappa}$ is {\em increasing} in the interval $[0,+\infty)$ since the set $B(0,\rho_0)\times  \Omega$ is {\em convex}. 

Fix $\tau > n-1$ and $\kappa\in (0,1)$, and 
define   $\Omega_\kappa$ as  the set of all $(\kappa,\tau)$-Diophantine vectors  satisfying \eqref{eq:sdc} and such that ${\rm dist}\, (\omega,\T^{n-1}\setminus \Omega)\ge \kappa$, i.e.
\begin{equation}
\label{eq:sdc3}
\Omega_\kappa =  D(\kappa,\tau)\cap \overline{\Omega -\kappa}.   
\end{equation}
Recall that $\vartheta_0$, $\ell_0$ and $\ell(m)$ are defined in \eqref{eq:ell(m)}. The following statement is a counterpart of Theorem \ref{Theo:A} in the case of exact symplectic mappings. 
\begin{Theorem}\label{Theo:A-for-maps}
 There is a positive constant $\epsilon= \epsilon(n,\tau,\vartheta_0)$  depending only  on $n$, $\tau$ and on $\vartheta_0$ such that for any $\delta>0$, $0<\kappa<1$ and $0<\varrho \le \rho_0$ the following holds.\\
 
\noindent 
Let $P_t$ be a  $C^k$ family of exact symplectic maps with generating functions  $\widetilde G_t$ satisfying \eqref{eq:generating-function-of P} and  \eqref{eq:families-of-perturbations-maps}   and such that 
\begin{equation}
   \sup_{t\in [0,\delta]} \, \| G_t\|_{\ell_0+1;\varrho,\kappa} \  \le \ \epsilon \varrho \kappa  \, .
\label{eq:smallness-condition-maps}
\end{equation}
Then there exists a $C^k$ family of maps 
\[
[0,\delta]\ni t \mapsto \phi_t\in C^\infty(\Omega;\Omega), \quad \ [0,\delta]\ni t \mapsto \Psi_t=(U_t,V_t)\in C^\infty(\T^{n-1} \times \Omega;\T^{n-1}\times B^{n-1}(0,\varrho)) \ 
\] 
such that   
\begin{enumerate}
\item [(i)]  ${\rm supp}\, (\phi_t-{\rm id})\subset \Omega-\kappa/2$, ${\rm supp}\, \big((U_t,V_t)-({\rm id},0)\big) \subset  \T^{n-1}\times (\Omega-\kappa/2)$; 
\item[(ii)]  
For each $\omega \in \Omega_\kappa$ and $t\in [0,\delta]$ the map 
$\Psi_{t,\omega} := \Psi_t(\cdot,\omega):{\T}^{n-1}  \rightarrow
 {\T}^{n-1}\times B(0,\varrho)$ 
is a smooth embedding, 
$\Lambda_t(\omega)  := \Psi_{t,\omega}({\T}^{n-1})$ is an embedded Lagrangian 
torus invariant  with respect to the exact symplectic map given by 
$ P_{t,\phi_t(\omega)}(\theta,I) := P(\theta, I; \phi_t(\omega),t)$, and 
\[
P_{t,\phi_t(\omega)} \circ \Psi_{t,\omega} = 
\Psi_{t,\omega} \circ R_{\omega} \quad \mbox{on}\  {\T}^n ;  
\]
\item[(iii)]
For any $m\in \N$ there is $C_m>0$ depending only on $m$, $n$, $\tau$ and $\vartheta_0$ such that
for any $\alpha,\beta\in \N^n$ with  $|\alpha|+|\beta|(\tau+1)\le m(\tau+1) +1$  the following estimate holds
\begin{equation}\label{eq:estimates-F}
\begin{array}{lrc}
\left|\partial_\theta^{\alpha}(\kappa \partial_\omega)^{\beta}(U_t(\theta;\omega) - \theta)\right|\,  + \,
\varrho ^{-1}
\left|\partial_\theta^{\alpha}(\kappa \partial_\omega)^{\beta} V_t(\theta;\omega)\right|  
+ \kappa^{-1} \left|(\kappa \partial_\omega)^{\beta}(\phi_t(\omega) - \omega)\right|
\\    [0.5cm]  
\displaystyle \leq\    C_{m}\, 
 (\varrho \kappa   )^{-1}\, \,\| G_t\|_{\ell(m)+1;\varrho,\kappa} 
\end{array}
\end{equation}
 uniformly in  $(\theta,\omega,t)\in {\T}^{n-1}\times \Omega_\kappa\times [0,\delta]$. 
\end{enumerate}
\end{Theorem}	
{\em Proof.} To simplify the notations we fix $k=1$. The first step in the proof will be to modify $P_t$ by multiplying $G_t$ by suitable cut-off functions without changing the corresponding estimates. This allows us to work with compactly supported functions. 
To this end we use the cut-off functions $\widetilde\psi_{\varrho}$ and $\psi_{\kappa}$ constructed in the previous sub-section by means of  Lemma \ref{lemma:cut-off-omega}. We set $G^1_t(\theta,I;\omega):= G_t (\theta,I;\omega) \widetilde\psi_{\varrho}(I) \psi_{\kappa}(\omega)$ and denote by $P_t^1$ the exact symplectic map with generating function 
\[
\widetilde G_t^1(\theta,r;\omega):= \langle \theta,r\rangle -\langle \omega,r\rangle -G_t^1(\theta,r;\omega). 
\]
The function $\ell \to \|G_t\|_{\ell;\varrho,\kappa}$ is {\em increasing} in the interval $[0,+\infty)$ since the set $B(0,\rho_0)\times  \Omega$ is {\em convex}. Then using \eqref{eq:Leibnitz1} one obtains
\[
\|G_t^1\|_{\ell;\varrho,\kappa} \le C_\ell \|G_t\|_{\ell;\varrho,\kappa} ,
\]
where $C_\ell$ depends only on $n$ and $\ell$. In particular, 
it follows from \eqref{eq:smallness-condition-maps} that
\[
\|\sigma_\varrho^{-1}{\rm sgrad}\,  G_t^1\|_{1;\varrho,\kappa} \le C_1\|\sigma_\varrho^{-1}{\rm sgrad}\,  G_t\|_{\ell_0-1;\varrho,\kappa} \le C_1\epsilon \kappa
\]
which allows one to apply Lemma \ref{rem:with-parameters}. Hereafter
\[{\rm sgrad\, }G_t^1(\theta,r;\omega):= (\nabla_r G_t^1(\theta,r;\omega), -\nabla_\theta  G_t^1(\theta,r;\omega))\]
is the simplectic gradient of $G_t^1$. 
We have 
$$
P_t^1(\theta,r;\omega)=(\theta+\omega,r) \quad \mbox{for} \quad (r,\omega)\notin  B^{n-1}(0,7\varrho/8)\times (\Omega-\kappa/4).
$$
Moreover, 
$$
P_t^1(\theta,r;\omega)= P_t(\theta,r;\omega) \quad \mbox{for} \quad (\theta,r;\omega)\in \T^{n-1}\times B^{n-1}(0,\varrho/2)\times (\Omega-\kappa)
$$ 
since $G_t^1=G_t$ on that set.  
This allows us to replace $G_t$ by $G_t^1$ and $P_t$ by $P_t^1$ in the theorem. 
From now on we suppose that 
\[
{\rm supp}\, G_t\subset \A':=\T^{n-1}\times B^{n-1}(0,\varrho)\times (\Omega-\kappa/4). 
\]
Set 
\[
{\mathcal N}_{\omega,\omega_n}(r,r_n):=  \langle \omega, r\rangle + \omega_nr_n, \quad (\omega,\omega_n)\in \Omega\times I, \quad I=(\pi, 3\pi),
\] 
Using an argument of Douady \cite{Dou} (see also Theorem 1.1 \cite{P2} and Theorem 3.1 \cite{P3}), 
we are going  to find a $C^1$ family of  Hamiltonians 
\begin{equation}\label{eq:inclusion-map-hamiltonian}
(\theta,\theta_n,r,r_n)\to H_t(\theta,\theta_n,r,r_n; \omega,\omega_n) =  \langle \omega, r\rangle + \omega_nr_n + h_t(\theta,\theta_n,r;\omega)
\end{equation}
 in $\T^n\times\R^n$ depending smoothly on parameters $(\omega,\omega_n)\in \Omega\times I$ with the following properties - $h_t$ is ``small'' and   the corresponding   Poincar\'e map is given by $P_t$ at any energy surface. Then we will apply Theorem \ref{Theo:A} to the family $H_t$.   
We set $y=(y',y_n)\in \R^n$, $(\theta,\theta_n)=\mathrm{pr}(y)\in \T^n$,  $\eta=(\eta',\eta_n)=(r,r_n)$ and $\widetilde \omega:= (\omega,\omega_n)\in \widetilde \Omega:= \Omega\times I$. We shall denote by $\Sigma_c$ the energy surface $ \Sigma_c:=\{H_t=c\} \subset \T^n\times\R^n$ for $c\in\R$ and by $\imath_c:\T^{n-1}\times\R^{n-1}\to\ \Sigma_c\cap \{\theta_n=0\}$ the corresponding inclusion map, i.e. 
$$\imath_c(\theta,r)=(\theta,0,r,(c-\langle \omega,r\rangle- h_t(\theta,0,r;\omega))/\omega_n).$$ 



\begin{Prop}\label{Prop:H}
There is a $C^1$ family of  Hamiltonians 
$$
H_t(\theta,\eta;\widetilde \omega):=  {\mathcal N}_{\widetilde \omega}(\eta) + h_t(\theta,\eta';\omega)\, ,\quad h_t\in C^\infty (\T^n\times\R^{n-1}\times \Omega)\, ,\  \widetilde \omega\in \Omega\times (\pi, 3\pi),
$$  
such that 
\begin{itemize}
	\item[(i)] $P_t = \imath^{-1}_{c}\circ \Phi_t^{\frac{2\pi}{\omega_n}}\circ\imath_{c}$ for any $c\in\R$, where 
	$\imath_c$ is the corresponding inclusion map 
	and $\Phi_t^{x}$,  $x\in\R$, is the Hamiltonian flow of $H_t$, 
	\item[(ii)] $\mathrm{supp\, } (h_t) \subset A'':= \T^n\times B^{n-1}(0,\varrho)\times \Omega$ and 
	the following estimate holds 
	\[
	\|h_t\|_{\ell,\A'';\varrho,\kappa} \le C_{\ell}  \|G_t\|_{\ell+1,\A' ;\varrho,\kappa} 
\]	 
	for any  $\ell\ge 2$ and $0<\varrho,\kappa\le 1$, where $\T^n\times\R^{n-1}\times \Omega$,  $C_\ell>0$ depends only on $\ell$ and $n$. 
	\item[(iii)] $h_t(\theta,\eta';\omega)= 0$ for $|\theta_n|\le \pi/2$.  
\end{itemize}
\end{Prop}
{\em Proof.}
Choose $\eta\in C^\infty(\R)$ such that $0\le \eta \le 1$, $\eta(s)=0$ for $|s|\le 1/4$ and $\eta(s)=1$ for $|s|\ge 1/2$.
 Consider the family of exact symplectic maps $s\to P_t^s$ in $\A=\T^{n-1}\times\R^{n-1}$ for $s\in \R$ having  generating functions of the form
\[
\widetilde G_t^s(\theta,r;\omega):= \langle \theta,r\rangle - s\langle \omega,r\rangle   - \eta(s)G_t(\theta,r;\omega),\ (\theta,r;\omega)\in \R^{n-1}\times\R^{n-1}\times \Omega.
\] 
We have $P_t^s=Q^s\circ W_t^s$, where $Q^s(\theta,r;\omega)=(\theta +s\omega,r)$ and the generating function of $W_t^s$ is 
$ \langle \theta,r\rangle   - \eta(s)G_t(\theta,r;\omega)$. 
Set $G(\theta,r;\omega,t)=G_t(\theta,r;\omega)$ and denote the symplectic gradient of $G$ with respect to $(\theta,r)$ by
\[
{\rm sgrad\, }G(\theta,r;\omega,t):= (\nabla_r G(\theta,r;\omega,t), -\nabla_\theta  G(\theta,r;\omega,t)).
\]
Notice that
\begin{equation}\label{eq:P-s}
\begin{array}{rcll}
P_t^s(\theta,r;\omega) &=& (\theta +s\omega,r)\quad \forall\, s\in [-1/4,-1/4]\\[0.3cm]
P_t^s(\theta,r;\omega) &=& P_t(\theta,r;\omega) \quad \forall\, s\in (-\infty,-1/2]\cup [1/2,+\infty) .
\end{array}
\end{equation}
Denote by 
$$\xi_t^s \, := \, \frac{d P_t^s}{ds}  \circ (P_t^s)^{-1}, \quad s\in \R$$  
the corresponding  vector field and set $v(\theta,s,r;\omega) =(\omega,0)$. Then
\[
\xi_t^s(\theta,r;\omega) = v(\theta,s,r;\omega) = (\omega, 0)\quad \forall\, s\in (-\infty,-1/2]\cup [-1/4,1/4]\cup [1/2,+\infty) .
\]
%and we can consider $ s$  as a variable on $\T_1:=\R/\Z$. 
We set $\xi_t(\theta,s,r;\omega)=\xi_t^s(\theta,r)$ where $(\theta, s)\in\T^{n-1}\times [0,1]$. 
\begin{Lemma}\label{lemma:zeta}
We have $\xi_t^s(\theta,r;\omega) = (\omega, 0)$ for $s\in [0,1/4]\cup [1/2,1]$ and  
$$\mathrm{supp\, }(\xi_t-v) \subset \A':= \T^{n-1}\times  (0 , 1)  \times B^{n-1}(0,\varrho)\times \Omega.$$ 
Moreover, the following estimates hold
\[
 \|\sigma_\varrho^{-1}(\xi_t-v)\|_{\ell, \A';\rho,\kappa} \le  C_{\ell} \, 
\|\sigma_\varrho^{-1}{\rm sgrad\, }G_t(\cdot;\omega)\|_{\ell,\A';\rho, \kappa} 
\]
where $\ell\ge 1$ and $C_{\ell}>0$ depends only on $\ell$ and $n$.
\end{Lemma}
{\em Proof.}    We have $\xi_t^s =v + dW_t^s/ds \circ (W_t^s)^{-1}$. By  Lemma \ref{lemma:generating-functions} the support of $W_t^s -\mathrm{id}$ is contained in $\A'$. 
The estimates of $dW_t^s/ds$ and $(W_t^s)^{-1}$ follow from Proposition \ref{prop:composition-holder1}, Lemma \ref{lemma:generating-functions} and Lemma \ref{rem:with-parameters} taking into account \eqref{eq:smallness-condition-maps}. To obtain the corresponding estimates for the composition $dW_t^s/ds\circ (W_t^s)^{-1}$ we use Proposition \ref{prop:composition-holder1}.   \finishproof

\noindent
Notice  that the one-form $\imath(\xi_t^s)d\theta\wedge dr$ is exact, where $d\theta\wedge dr=\sum_{j=1}^{n-1}d\theta_j\wedge dr_j$ is the standard symplectic two-form in $T^\ast \T^{n-1}$ and $\imath(v)$ is the inner product with the vector field $v$. This follows from the identity 
$$\imath(\xi_t^s)d\theta\wedge dr=(P_t^s)_\ast(\frac{d}{ds}\, (P_t^s)^\ast ( r d\theta)-d(\imath(\xi_t^s)r d\theta)) $$
 since $(P_t^s)^\ast ( r d\theta) -  r d\theta$ is exact. 
Let $h_t^s$ be a primitive of 
\begin{equation}\label{eq:primitive-h}
\left\{
\begin{array}{lcrr}
\imath(\xi_t^s-v)d\theta\wedge dr= - dh_t^s\\[0.3cm]
h_t^s(0,0;\omega)=	0.
\end{array}
\right.
\end{equation}
The first equality in \eqref{eq:primitive-h} means that
\[
\begin{pmatrix}
\partial_{\varphi}h_t^s\cr
\partial_{r}h_t^s
\end{pmatrix}
=
\begin{pmatrix}
0 & I\cr
-I & 0
\end{pmatrix}
(\xi_t^s -v) .
\]
The second one combined with  Lemma \ref{lemma:zeta}   implies $\mathrm{supp\, }(h_t) \subset \A'$ and
\[
\begin{array}{lcrr}
\displaystyle \|h_t\|_{\ell,\A';\varrho,\kappa}  \le C \big(\|\partial_\theta h_t\|_{\ell,\A';\varrho,\kappa} + \|(\varrho \partial_I )h_t\|_{\ell,\A';\varrho,\kappa}  \\[0.3cm]
\displaystyle \le\,  C_\ell^\prime\big(\|\partial_\theta h_t\|_{\ell,\A';\varrho,\kappa} + \|(\varrho \partial_I )h_t\|_{\ell-1,\A';\varrho,\kappa}\big)\\[0.3cm]
\displaystyle \le  C_{\ell} \|G_t\|_{\ell+1,\A';\varrho,\kappa} .
\end{array}
\]
% which proves (ii). ???

We denote as above
$y=(y',y_n)\in \R^n$, where $y_n = 2\pi s$, $(\theta,\theta_n)= \mbox{pr}(y) \in \T^n$, $\eta=(\eta',\eta_n)=(r,r_n)$,   and set 
\[
h_t(y,\eta';\omega):=h_t^{y_n/2\pi}(y',\eta';\omega),  \ H_t(y,\eta;\omega,\omega_n):= \langle \omega, \eta'\rangle+ \omega_n \eta_n + h_t(y,\eta';\omega). 
\]
Let 
${\mathcal N}(\eta;\omega,\omega_n)= \langle \omega,\eta'\rangle + \omega_n\eta_n$ be the corresponding normal form. 
The  H\"{o}lder norms of $H_t-{\mathcal N}=h_t$ have been estimated above which proves (ii). 


Notice that $
h_t^s(\theta,r)= 0$ for  $s\in [0,1/4]\cup [1/2,1]$ 
since $\xi_t^s(\theta,r;\omega)=(\omega,0)$ there. 
Then 
\[
h_t(\theta,\eta_n,r,\omega)= 0 \quad \forall\, \theta_n \in  [0,\pi/2]\cup [\pi,2 \pi]
\]
which gives (iii). To obtain (i), consider the Hamiltonian vector field $X_{H_t}$ given by 
\[
\imath(X_{H_t})dy\wedge d\eta= - dH_t(y,\eta).
\]
By \eqref{eq:primitive-h} we get 
\[
(\partial_r H_t(\theta,y_n,r,r_n), - \partial_\theta H_t(\theta,y_n,r,r_n)) = (\partial_r h_t^{y_n/2\pi}(\theta,r)+\omega, - \partial_\theta h_t^{y_n/2\pi}(\theta,r)) = \xi_t^{y_n/2\pi}(\theta,r).
\]
Moreover, $\partial_{r_n} H_t(\theta,y_n,r,r_n)=\omega_n$. Setting $P_t^s(\theta,r)= (p_t^s(\theta,r),  q_t^s(\theta,r))$ we obtain that the Hamiltonian flow $\Phi_t^s$ of $H_t$ is given by 
\[
\Phi_t^x(\theta,y_n,r,r_n)= (p_t^{x\omega_n/2\pi}(\theta,r),y_n+x\omega_n, q_t^{x\omega_n/2\pi}(\theta,r), q_n^{x\omega_n/2\pi}(\theta,y_n,r,r_n))
\]
for $x\in \R$, where $t\to q_n$ is a $C^1$ family of smooth functions. 
%Given $c\in\R$ we denote by $\Sigma_{c}:= \{H_t=c\}$ the corresponding level set of the Hamiltonian $H_t$. 
This yields
\[
\Phi_t^{\frac{2\pi}{\omega_n}}(\theta,0,r,r_n)= (p_t^{1}(\theta,r),2\pi, q_t^{1}(\theta,r), q_n^{1}(\theta,0,r,r_n)). 
\]
%for $(\theta,0,r,r_n)\in \Sigma_c$. On the other hand $|1-\omega_n/2\pi|<1/2$ if the interval $I$ is sufficiently small and taking into account \eqref{eq:P-s} we get 
%\[\Big(p_t^{\frac{1}{\omega_n}}(\theta,r),q_t^{\frac{1}{\omega_n}}(\theta,r)\Big)=  P_t(\theta,r) \quad \forall\, \omega_n\in I.\]
This implies (i) and  completes the proof of the proposition. \finishproof

In particular, we have
\[
\|h_t\|_{\ell_0,\A'';\varrho,\kappa} \le C \epsilon \kappa \varrho
\]
for $t\in [0,a]$, where $C>0$ depends only on $\ell_0$ and $n$. Then 
Proposition  \ref{Prop:H} allows us to apply Theorem \ref{Theo:A} to the perturbation $H_t$ of ${\mathcal N}$ in 
$\T^n\times  B^n(0,\varrho)\times \tilde \Omega$, where $\tilde \Omega:=\Omega\times (\pi,3\pi)$.   Denote by 
\[
\tilde \Psi_t=(\tilde U_t,\tilde V_t,\tilde \phi_t): \T^n\times  B^n(0,\varrho)\times \tilde \Omega\to \T^n\times  B^n(0,\varrho)\times \tilde \Omega
\] 
the map given by Theorem \ref{Theo:A}. 
To obtain the map $\Psi_t$ from $\tilde \Psi_t$ we use an argument of  Douady \cite{Dou}.  Fix $\omega\in \Omega_\kappa$ and $t\in [0,\delta]$. 
Then $\tilde \omega:=(\omega,2\pi)\in \tilde\Omega_\kappa:=\widetilde D(\kappa,\tau)\cap (\tilde \Omega-\kappa)$, where $\widetilde D(\kappa,\tau)$ is given by \eqref{eq:sdc2}. By  Theorem \ref{Theo:A} there exists  a $C^1$ family of Kronecker invariant tori $\tilde\Lambda_t(\tilde\omega)$  of the flow $\Phi^s_{t}(\cdot; \tilde \phi_t(\tilde\omega))$ of the Hamiltonian $H_t(\cdot; \tilde \phi_t(\tilde\omega))$ with a frequency  vector $\tilde\omega$ lying on a certain energy surfaces  $\Sigma_{t}:=\{  H_t = c_t\}$. Moreover, 
\begin{equation}
\left(\tilde U_t(y + x \tilde\omega; \tilde \omega),\tilde V_t(y+x \tilde\omega; \tilde\omega)\right) \, =\, \Phi^x_{t}\left(\tilde U_t(y,\tilde\omega), \tilde V_t(y, \tilde\omega);\tilde \phi_t(\tilde\omega)\right)\,  
\label{eq:g}
\end{equation}
for any $x\in \R$ and $y\in \T^n$. On the other hand,  $\Phi^x_{t}$ is of the form
\[
\Phi^x_{t}(y',y_n,\eta;\tilde \phi_t(\tilde\omega))= (z_t'(x,y,\eta;\tilde \omega),y_n + x\omega_n, \zeta_t(x,y,\eta;\tilde \omega))
\]
since $\partial H_t/\partial \eta_n=  \omega_n$, hence,   the last coordinate 
$\tilde U_{t,n}$ of $\tilde U_t$ satisfies the equality
$$\tilde U_{t,n}(y + x \tilde \omega;\tilde \omega)= \tilde U_{t,n}(y;\tilde \omega) +x\omega_n $$ 
for any $y\in \T^n$ and $x\in \R$. 
Then $\nabla_y\tilde U_{t,n}(y + x \tilde \omega;\tilde \omega)= \nabla_y\tilde U_{t,n}(y;\tilde \omega)$, and since the flow $x\mapsto x \tilde \omega$ is ergodic on $\T^n$ (recall that $\tilde \omega$ is a Diophantine frequency) we get 
$$\nabla_y\tilde U_{t,n}(y;\tilde \omega)=\nabla_y\tilde U_{t,n}(0;\tilde \omega):=a_t(\tilde \omega)$$
 for any $y\in\T^n$. The function $\T^n \ni y\mapsto U_{t,n}(y ;\tilde \omega)\in \T$ is  determined   up to a translation and we fix it by $U_{t,n}(0;\tilde \omega)=0$. Then    $\tilde U_{t,n}(y;\tilde \omega) = \langle a_t(\tilde \omega),y \rangle$ and $a_t(\tilde \omega)\in\Z^n$. On the other hand,   $|\nabla_y\tilde U_t(y;\tilde \omega)- \mathrm{Id}| \le C(n,\tau,\vartheta_0)\epsilon$ in view of \eqref{eq:main-estimates}  and \eqref{eq:smallness-condition3}. 
 Taking $\epsilon=\epsilon(n,\tau,\vartheta_0)$ small enough we obtain  that $a_t=(0,\ldots,0,1)$  and  $\tilde U_{t,n}(y; \tilde \omega) = y_n$. Now we set 
 \[
 \Psi_{t}(\theta,r) =(U_t(\theta,\omega),V_t(\theta,\omega) ) :=  \mathrm{p} (\tilde U_t(\theta,0,\tilde\omega), \tilde V_t(\theta,0,\tilde\omega)),\quad \phi_t(\omega)=\tilde \phi_t(\tilde\omega),\quad  \tilde\omega=(\omega, 2\pi), 
 \]
 where $\mathrm{p}$ is the projection given by $\mathrm{p}(\theta,\theta_n,r, r_n)= (\theta,r)$.


Using Proposition \ref{Prop:H}  one  obtains that for each $ \omega\in \Omega_\kappa$, the torus 
 \[
 \Lambda_t(\omega):= \mathrm{p} (\tilde\Lambda_t(\tilde\omega))  
 \]   
 is a Kronecker invariant torus of $P_{t,\phi_t(\omega)}$ with a frequency vector $\omega$ and  we obtain (ii). Moreover, \eqref{eq:estimates-tilde-F} implies \eqref{eq:estimates-F}. This completes the proof of Theorem \ref{Theo:KAM}. \finishproof
\\


\subsection{KAM theorems for $C^k$ families of symplectic maps}\label{Subsec:KAM-maps}
The aim of this section is to obtain $C^k$ families of Kronecker invariant tori of $C^k$ families of exact  maps close to the family  $(\theta,r) \to (\theta +\nabla K_t(r),r)$, $t\in [0,\delta]$. 

Let $\Omega \subset [0,2\pi]^{n-1}$ be an open convex set which we  identify with an open convex subset of $\T^{n-1}$.
Fix $k\in\{0,1\}$ and consider  a $C^k$-family  of real-valued functions 
\[
[0,\delta]\ni t\to K_t^\ast\in C^\infty( \overline \Omega,\R)
\]  
 satisfying the non-degeneracy condition 
\begin{equation}\label{eq:non-degenerate1}
\nabla K_t^\ast : \Omega \longrightarrow  D_t:=\nabla K^\ast_t(\Omega) \ \mbox{is a diffeomorphism.}
\end{equation}
where $\overline \Omega$ is the closure of $\Omega$. 
For any $t\in [0,\delta]$ the Legendre transform $K_t:  D_t\to  \Omega$ of $K_t^\ast$ is in $C^\infty(  D_t,\R)$ and it satisfies the non-degenerate condition \eqref{eq:non-degenerate}. Moreover, the corresponding family of functions    $[0,\delta]\ni t\to K_t\in C^\infty( D_t,\R)$ is $C^k$ smooth. 
We set $\A_t:=\T^{n-1}\times D_t$ and   denote by
\begin{equation}\label{eq:Q}
Q_t:\A_t\to \A_t, \quad Q_t(\theta,r)= (\theta +\nabla K_t(r),r)
\end{equation}
the corresponding family of exact symplectic maps on $\A_t$.   The frequency vector of $Q_t$ on the invariant torus $\T^{n-1}\times \{r\}$ is $\omega=\nabla K_t(r)\in \Omega$.


We consider  a $C^k$-family   of exact symplectic maps 
\begin{equation}\label{eq:P-t-family-1}
[0,\delta]\ni t\to P_t \in C^\infty( \A_t, \T^{n-1}\times \R^{n-1})
\end{equation}
close $Q_t$.   We suppose  that  $P_t$ is defined by  a generating function $\widetilde G_t$ of the form
\begin{equation} 
\label{eq:generating-function-of-P-1}
\widetilde G_t(\theta,r):= \langle \theta,r\rangle - K_t(r) -G_t(\theta,r)
\end{equation}
which  means that 
\[
P_t(\theta-\nabla K_t(r)-\nabla_{r}G_t(\theta,r),r)=(\theta, r-\nabla_{\theta}G_t(\theta,r))
\]
for any $(\theta,r)\in \A_t$. We suppose as well that
the map
\[
[0,\delta] \ni t\to G_t \in C^\infty (\T^{n-1}\times D_t, \R)
\]
is $C^k$ smooth with $k=0$ or $k=1$. 

We assume as well that the $C^2$ norm of $G_t$ is  sufficiently small. Then  the inverse function theorem implies that the map $\theta \to\theta-\nabla_{r}G_t(\theta,r)$ is a diffeomorphism of  $\T^{n-1}$ for any fixed $r\in D_t$ and $P_t$ is well defined. 

Denote by $R_t$ the exact symplectic map with generating function $(\theta,r)\to \langle \theta,r\rangle  -G_t(\theta,r)$, i.e. $R_t(\theta-\nabla_{r}G_t(\theta,r),r)=(\theta, r-\nabla_{\theta}G_t(\theta,r))$.  One can show that 
 $P_t=R_t\circ Q_t$ on $\A_t$ (see Lemma \ref{Lemma:decomposition}). 





Given $\varrho,\kappa\in (0,1)$ and $m\ge 0$ we set
\begin{equation}
\label{eq:B-0-sequence}
{\mathcal B}_m^0 \, := \,   \sup_{0\le t\le \delta }\, \left( \varrho^2 |\!|\!| \partial^2 K_t |\!|\!|_{\ell(m)+1,  D_t;\kappa} \, +\,  |\!|\!|  G_t|\!|\!|_{\ell(m)+1,\A_t; \kappa}\right), 
\end{equation}
where  $\|G_t\|_{\ell, \A_t;\kappa} := \|G_t\circ \sigma_{\kappa}\|_{C^\ell(\sigma_{\kappa}^{-1}(\A_t))}$, 
 $\sigma_\kappa$ is defined by $\sigma_\kappa(x,\xi)=(x,\kappa \xi)$, and
\[
|\!|\!| u |\!|\!|_{\ell,D;\kappa}\, =\, \sup_{0\le m\le \ell}\|u\|_{\ell-m,D;\kappa}.
\]
 Recall that $\vartheta_0$, $\ell_0$ and $\ell(m)$ are defined in \eqref{eq:ell(m)}. The sequence ${\mathcal B}_m^0$, $m\in\N$, is increasing by definition. 
 
  To formulate the smallness condition in the KAM theorem below we need as well  the notation 
\begin{equation}\label{eq:S-K-sequence}
S_{\ell}(\nabla K^{\ast}) := \sup_{0\le t\le \delta }\, \big(1+ \|\nabla K^{\ast}_t\|_{C^1(\Omega)}\big)^{\ell-1} \big(1+ \|\nabla K^{\ast}_t\|_{C^\ell(\Omega)}\big)
\end{equation}
introduced  in \eqref{eq:S-sequence}. This in an increasing sequence with respect to $\ell\in [1,+\infty)$ since $\Omega$ is convex. 
For any $m\in\N$ we set
\begin{equation}
\label{eq:B-sequence}
{\mathcal B}_m \, := \,   {\mathcal B}_m^0 S_{\ell(m)+2}(\nabla K^{\ast}). 
\end{equation}



\begin{Theorem}\label{Theo:KAM} There exists $\epsilon = \epsilon(n,\tau,\vartheta_0)>0$ depending only on $n$, $\tau$ and $\vartheta_0$ such that 
the following holds.\\

\noindent
Let  $\Omega\subset \T^{n-1}$ be an open convex  set,  $[0,\delta]\ni t\to K_t^\ast\in C^\infty( \overline \Omega,\R)$  a $C^k$ family  satisfying \eqref{eq:non-degenerate1} and let $\varrho>0$ and $\kappa>0$ be such that $0<\varrho\le \kappa\le 1$ and $\Omega_\kappa\neq\emptyset$. 
Consider a  $C^k$ family  of  exact symplectic maps  
$[0,\delta]\ni P_t\in C^\infty( \A_t,  \T^{n-1}\times\R^{n-1})$  with generating functions $\widetilde G_t$ of the form \eqref{eq:generating-function-of-P-1} such that
\begin{equation}\label{eq:smallness-condition-maps-2}
{\mathcal B}_0^0S_{\ell_0+1}(\nabla K^{\ast})\, =\,   \sup_{0\le t\le \delta }\, \left( \varrho^2 |\!|\!| \partial^2 K_t |\!|\!|_{\ell_0+1,  D_t;\kappa} \, +\,  
|\!|\!| G_t|\!|\!|_{\ell_0+1,\A_t; \kappa}\right)\, 
S_{\ell_0+1}(\nabla K^{\ast})\ 
\le \ \epsilon \varrho \kappa .
\end{equation}
Then there is a $C^k$ family $[0,\delta]\ni t\to    f_t=( u_t, v_t)\in C^\infty(\T^{n-1}\times \Omega; \T^{n-1}\times  D_t)$ such that 
\begin{enumerate}
\item[(i)]
for any $\omega\in \Omega_{\kappa}$,  
$[0,\delta]\ni s\to \Lambda_t(\omega)=  f_{t,\omega}(\T^{n-1})$ is a $C^k $  family of Kronecker invariant tori 
of of $P_t$ with a frequency vector $\omega$, where $  f_{t,\omega}:=  f_t(\cdot; \omega)$, and 
the following diagram is commutative
\[
\displaystyle{\begin{array}{cccl} 
\displaystyle \T^{n-1}&\stackrel{R_{\omega}}{\longrightarrow}&\T^{n-1}\cr
\downarrow\lefteqn{ f_{t,\omega}}& &\downarrow\lefteqn{  f_{t,\omega}} \cr
\displaystyle \Lambda_t(\omega)&\stackrel{P_t}{\longrightarrow}&\Lambda_t(\omega)&  
\end{array} }
\]
\item[(ii)] for any $m\in \{0 \}\cup [1,+\infty)$ the following estimates hold 
\begin{equation}\label{eq:estimates-F-1}
\begin{array}{lcrr}
\displaystyle \big|\partial_\varphi^\alpha (\kappa\partial_\omega)^\beta \big(u_t(\varphi;\omega)-\varphi)\big)\big| \, \le\,  C_m \frac{{\mathcal B}_m}{\kappa\varrho}\\[0.3cm]
\displaystyle
  \big|\partial_\varphi^\alpha (\kappa\partial_\omega)^\beta   \big(v_t(\varphi;\omega)-\nabla K_t^{\ast} (\omega)\big)\big| 
\, \le\,  C_m \frac{{\mathcal B}_m}{\varrho} \left(1+\frac{{\mathcal B}_1}{\varrho}\right)^{m} 
\end{array}
\end{equation}
for any $(\varphi,\omega)\in \T^{n-1}\times \Omega_\kappa$, $t\in [0,\delta]$,   and multi-indices $\alpha,\beta\in \N^{n-1}$ with  $|\alpha|+|\beta|(\tau+1)\le m(\tau+1)+1$, where  the constant $C_m>0$ depends only on $n$, $\tau$,  $\vartheta_0$ and $m$,  
\item[(iii)]
${\rm supp\, }\big((u_t,v_t) -({\rm id}, \nabla K_t^\ast \big) \subset \T^{n-1}\times (\Omega-\kappa/2)$.
\end{enumerate}
\end{Theorem}
We note that the $C^1$ families of invariant tori $\Lambda_t(\omega)$, $t\in [0,\delta]$, given by the theorem are uniquely defined. \\

\noindent
{\em Proof}. The proof is similar to that of Theorem \ref{Theo:KAM2} and we give only the main steps in it. We are going to apply Theorem \ref{Theo:A-for-maps}. To this end we will firstly construct the function $\widetilde G_t(\theta,r;\omega)$ in \eqref{eq:generating-function-of P}. \\



\noindent
{\em Step 1. Construction of the generating function $\widetilde G_t(\theta,r;\omega)$.}
Given $\omega\in \Omega -\kappa/4$ 
and $I$ the ball $B^{n-1}(0,\varrho)$,   we set 
$r=\nabla K_t^{\ast}(\omega) + I$. 
Choosing $\epsilon=\epsilon(n,\tau,\vartheta_0) < 1/9$ in  \eqref{eq:smallness-condition-maps-2} we obtain as in the proof of of Theorem \ref{Theo:KAM2} the following relation
\begin{equation} \label{eq:domain-G}
\forall\,  \omega\in \Omega-\kappa/4,\ \forall\, I\in B^{n-1}(0,\varrho), \quad  \left\{
\begin{array}{lcrr}  
\nabla K^{\ast}_t(\omega) + I\in D_t \quad \mbox{and}\\[0.3cm] 
\displaystyle \nabla  K_t(\nabla K^{\ast}_t(\omega) + I)\in \Omega-\frac{1}{8}\kappa  . 
\end{array}
\right.
\end{equation}
By Taylor's formula we obtain
\begin{equation}\label{eq:generating-function-G}
\widetilde G_t(\theta,r) = \langle \theta, \nabla K_t^\ast(\omega)\rangle + \langle \theta, I\rangle - K_t(\nabla K_t^\ast(\omega))  - \langle \omega, I\rangle - G_t^0(I;\omega) - G_t^1(\theta,I;\omega),
\end{equation}
where
\[
G_t^0(I;\omega) = \int_0^1(1-s)\langle \partial^2K_t(\nabla K_t^{\ast}(\omega) + sI)I,I\rangle\,  ds 
\]
and 
\[
G_t^1(\theta,I;\omega):= G_t(\theta, \nabla K^{\ast}_t(\omega) + I). 
\]
It follows from \eqref{eq:domain-G} that the functions  $G_t^0$ and $G_t^1$ are well defined  for $I\in B^{n-1}(0,\varrho)$ and $\omega\in \Omega-\kappa/4$.
 Denote by $P_{t,\omega}:\A_t\to \T^{n-1}\times \R^{n-1}$ the exact symplectic map defined by means of the  generating function 
\[
\begin{array}{rcll}
(\theta,I)\to \widetilde G_{t,\omega}(\theta,I)&:=& \langle \theta, I\rangle - \langle \omega, I\rangle - G_t^0(I;\omega) - G_t^1(\theta,I;\omega)\\[0.3cm]
 &=& \widetilde G_t(\theta,\nabla K_t^\ast(\omega)+I) -\langle \theta, \nabla K_t^\ast(\omega)\rangle - K_t(\nabla K_t^\ast(\omega))
\end{array}
\]
and set $\psi_\omega(\theta,I)= (\theta, \nabla K_t^\ast(\omega)+ I)$. 
\begin{Lemma}\label{lemma:equality-for-P}  For any $\omega\in \Omega-\kappa/4$ the map $P_{t,\omega}:\A_t\to \T^{n-1}\times \R^{n-1}$ is well defined and 
\[
 P_{t,\omega} = \psi_\omega^{-1}\circ P_t \circ \psi_\omega
\]
on $\T^{n-1}\times B^{n-1}(0,\varrho)$ provided that the constant  $\epsilon = \epsilon(n,\tau,\vartheta_0)$ in \eqref{eq:smallness-condition-maps-2} is sufficiently small. 
\end{Lemma}
{\em Proof}. The smallness condition \eqref{eq:smallness-condition-maps-2} implies that   
$\|\nabla_\theta \nabla_I \widetilde G_{t,\omega}(\theta,I)-{\rm Id}_n\| \le C\epsilon$  for $(\theta,I;\omega)\in \T^{n-1}\times B^{n-1}(0,\varrho)\times (\Omega-\kappa/4)$, where $C=C(n)$ depends only on the dimension $n$ and ${\rm Id}_n\in M_n(\R^{n-1})$ is the identity matrix. Choosing   $\epsilon = \epsilon(n,\tau,\vartheta_0)$ sufficiently small we obtain that the map $\theta\to \varphi=\nabla_I \widetilde G_{t,\omega}(\theta,I)$ is a diffeomorphism on $\T^{n-1}$ for any fixed $I\in B^{n-1}(0,\varrho)$ and $\omega\in \Omega-\kappa/4$, hence, $ P_{t,\omega}$ is well-defined. Notice that
$\nabla_I \widetilde G_{t,\omega}(\theta,I)=\nabla_r \widetilde G_t(\theta,\nabla K_t^\ast(\omega)+I)$ and $\nabla_\theta \widetilde G_{t,\omega}(\theta,I)=\nabla_\theta \widetilde G_t(\theta,\nabla K_t^\ast(\omega)+I)- \nabla K_t^\ast(\omega)$. Then
\[
 (\psi_\omega \circ P_{t,\omega})\big(\nabla_r \widetilde G_t(\theta,\nabla K_t^\ast(\omega)+I),I\big)=\big(\theta, \nabla_{\theta}\widetilde G_t(\theta,\nabla K_t^\ast(\omega)+I)\big).
\]
On the other hand,
\[
\begin{array}{rcll}
( P_t\circ\psi_\omega) \big(\nabla_r \widetilde G_t(\theta,\nabla K_t^\ast(\omega)+I),I\big)&=&P_t\big(\nabla_r \widetilde G_t(\theta,\nabla K_t^\ast(\omega)+I),\nabla K_t^\ast(\omega)+I\big)\\[0.3cm]
&=&\big(\theta, \nabla_{\theta}\widetilde G_t(\theta,\nabla K_t^\ast(\omega)+I)\big)
\end{array}
\]
and we obtain that $ \psi_\omega \circ P_{t,\omega} =  P_t \circ \psi_\omega$ since the map $\theta\to \nabla_r \widetilde G_t(\theta,r)$ is a diffeomorphism. \finishproof
\\

\noindent
{\em Step 2. H\"older estimates of $\widetilde G_t$.}
We are going to apply Theorem \ref{Theo:A-for-maps} to the family of exact symplectic maps $ P_t(\cdot;\omega):=\widetilde P_{t,\omega}(\cdot)$. 
To this end  we evaluate  the weighted norms of  $G_t^0$ and $G_t^1$. We have  $G_t^0=Q_t^0\circ ({\rm id}, \nabla K_t^{\ast})$, where
\[
Q_t^0(I;r)=\int_0^1(1-s)\langle \partial^2K_t(r+sI)I,I\rangle\, ds 
\]
is well defined and smooth in $\overline\Gamma$, $\Gamma:= B^{n-1}(0,\varrho)\times (\Omega-\kappa/4)$. 
As in the proof of Theorem \ref{Theo:KAM2} we obtain that 
\[
 |\!|\!|  Q_t^0 |\!|\!| _{\ell,\Gamma;\varrho,\kappa} \le  C_{\ell} \, \varrho^2 |\!|\!| \partial^2 K_t |\!|\!|_{\ell, D_t;\kappa} . 
\]
Since $\Omega$ is convex and $K^{\ast}_t\in C^\infty(\overline \Omega)$ using  Proposition \ref{prop:composition-holder1}, {\em 3.}, and Remark \ref{rem:anisotrop} as in the proof of Theorem \ref{Theo:KAM2}we obtain  for  any  $\ell\ge 1$ the estimate
\[
\|G_t^0\|_{\ell;\varrho,\kappa} \le 
C_{\ell} \, \varrho^2\, |\!|\!| \partial^2K_t |\!|\!|_{ \ell, D_t; \kappa}
S_{\ell}(\nabla K^{\ast}).  
\]
Moreover,  $\|G_t^1\|_{\ell;\varrho,\kappa} \le \|G_t^1\|_{\ell;\kappa,\kappa} \le C_\ell |\!|\!|G_t|\!|\!|_{\ell;\kappa}S_{\ell}(\nabla K^{\ast})$  since $0<\varrho\le \kappa\le 1$ and we obtain
\begin{equation}\label{eq:estimate-G-0-1}
\begin{array}{rcll}
\displaystyle\|G_t^0\|_{\ell;\varrho,\kappa} + \|G_t^1\|_{\ell;\varrho,\kappa}
\le \displaystyle C_{\ell} \left(\varrho^2\, |\!|\!| \partial^2 K_t |\!|\!|_{ \ell, D_t; \kappa}\, +\, |\!|\!| G_t |\!|\!|_{\ell,\A_t; \kappa}\right)\ 
S_{\ell}(\nabla K^{\ast}).
\end{array}
\end{equation}
\\

\noindent
{\em Step 3. Applying  Theorem \ref{Theo:A-for-maps}}. 
Now \eqref{eq:smallness-condition-maps-2} gives 
\[
\|G^0_t\|_{\ell_0+1;\varrho,\kappa} + \|G^1_t\|_{\ell_0+1;\varrho,\kappa} \le {\mathcal B}_0 S_{\ell_0+1}(\nabla K^{\ast})\le \epsilon \varrho \kappa .
\]  
This allows us to apply Theorem \ref{Theo:A-for-maps} to  the family of exact symplectic maps $ P_t(\cdot;\omega)=\widetilde P_{t,\omega}(\cdot)$. 
Set $ \Psi_t = (u_t, v_t)$, where $u_t= U_t$, $v_t=(\nabla K^{\ast}_t)\circ \phi_t +V_t$ and  $(U_t,V_t,\phi_t)$ are given by Theorem  \ref{Theo:A-for-maps}. Notice that $\|V_t\|_{C^0} \le c\epsilon \varrho$ in view of the estimates in (ii), Theorem \ref{Theo:A-for-maps}, where the constant $c$ depends only on  $n$, $\tau$ and $\vartheta_0$, and taking $\epsilon<\min(1,1/c)$ we obtain $V_t(\theta;\omega)\in B^{n-1}(0,\varrho)$ for any $\theta\in \T^{n-1}$ and $\omega\in \Omega-\kappa$. In the same way we get $\phi_t(\omega)\in \Omega-\kappa/4$ for $\omega\in \Omega-\kappa$. 

Now  Lemma \ref{lemma:equality-for-P} implies that for any $\omega\in \Omega_\kappa$ and $t\in [0,\delta]$ the Lagrangian manifold 
$ \Lambda_t(\omega):=  \Psi_{t}(\T^{n-1};\omega)$
is a Kronecker invariant torus of $P_t$ of a frequency vector $\omega$ satisfying  (i) in Theorem \ref{Theo:KAM}.  \\



\noindent
{\em Step 4. Estimates of $u_t$ and $v_t$.}

The estimates (ii), Theorem \ref{Theo:A-for-maps}, imply (ii) in Theorem \ref{Theo:KAM}. To estimate the derivatives of 
\[
v_t- \nabla K^{\ast}_t = V_t+ (\nabla K^{\ast}_t)\circ \phi_t - \nabla K^{\ast}_t
\]
we use (ii), Theorem \ref{Theo:A-for-maps} 
and the following Lemma which is an analogue of Lemma \ref{lemma:estimates-V}.
\begin{Lemma}\label{lemma:estimates-v}
For any $m\in \N$ the following estimate holds
\[
\|(\nabla K^{\ast}_t)\circ \phi_t - \nabla K^{\ast}_t\|_{m,\Omega;\kappa} \le C_{m} \frac{{\mathcal B}_m}{\varrho}\left(1+\frac{{\mathcal B}_1}{\varrho} \right)^m.
\]
\end{Lemma}
To prove (iii) we use suitable cut-off functions in $\omega$ given by Lemma \ref{lemma:cut-off-omega}. 
\finishproof 


\subsection{Birkhoff Normal Forms for $C^k$-families of symplectic maps}\label{Subsec:BNF-for-maps}
Let $\Omega \subset [0,2\pi]^{n-1}$ be an open convex set which we  identify with an open convex subset of $\T^{n-1}$. Fix $\tau>n-1$ and denote by $\kappa_0(\Omega)$ the supremum of all $0<\kappa\le 1$ such that the set $\Omega_\kappa= D(\kappa,\tau)\cap \overline{\Omega-\kappa}$ is of  positive Lebesgue measure. Given $0<\kappa<\kappa_0(\Omega)$ we denote by $\Omega_\kappa^0$ the set of points of $\Omega_\kappa$ of {\em positive Lebesgue density}. Recall that $\omega\in \Omega_\kappa^0$ if  the Lebesgue measure of $\Omega_\kappa\cap U$ is positive for any neighborhood $U$ of $\omega$. Then $\Omega_\kappa\setminus\Omega_\kappa^0$ is a set of measure zero.  Fix $0<\vartheta_0\le 1$ such that $2\tau + \vartheta_0\notin\Z$  and define $\ell_0$ and $\ell(m)$, $m\in\N$ as in \eqref{eq:ell(m)}, i. e. $\ell_0:=2\tau + 2 + \vartheta_0$ and $\ell(m):=  2m(\tau + 1)+ \ell_0$ for $m \in \N$. 

We are going to use as well the notations ${\mathcal B}_{m}$  and $S_{\ell}(\nabla K_t^{\ast})$  introduced  in  \eqref{eq:B-sequence}  and  \eqref{eq:S-K-sequence}. 

To construct a BNF we have to deal with the second differential $d^2K_t$ of the Legendre transform $K_t$ of $K_t^\ast$. 
We denote by $\partial^2 K_t(I)$ its Hessian matrix. Its norm  could be very large and to measure it we introduce a parameter $\lambda>1$. More precisely, we suppose below that 
\begin{equation}\label{eq:non-degeneracy-BNF}
  \sup_{t\in [0,\delta]} \|\partial^2 K_t\|_{2,D_t; \kappa}\,  \le \, \lambda \, < \, \infty\, , 
\end{equation}
where $\lambda\ge 1$. 
 
\begin{Theorem}\label{Theo:BNF}  There exists $\epsilon = \epsilon(n,\tau,\vartheta_0)>0$ depending only on $n$, $\tau$, and $\vartheta_0$ such that 
the following holds. 
\\

\noindent
Let $\Omega\subset \T^{n-1}$ be an  open convex set and  $0<\varrho<\kappa< \kappa_0(\Omega)$.
Let    $[0,\delta]\ni t\to K_t^\ast\in C^\infty( \overline {\Omega},\R)$ be a $C^k$ family  satisfying the non-degeneracy condition \eqref{eq:non-degenerate1} and suppose that its Legendre transform $K_t$ satisfies \eqref{eq:non-degeneracy-BNF}.
Let  
$[0,\delta]\ni P_t\in C^\infty( \A_t,  \A)$,   be a  $C^k$ family  of  exact symplectic maps defined by generating functions $\widetilde G_t(\theta,r)=\langle \theta,r\rangle -K_t(r)-G_t(\theta,r)$
such  that  
\begin{equation}\label{eq:smallness-condition-1}
{\mathcal B}_2\ \le \ \epsilon \varrho \kappa\lambda^{-4} . 
\end{equation} 
Then 
\begin{enumerate}
\item[(i)] there exist  $C^k$-smooth with respect to $t\in [0,\delta]$ families of exact symplectic maps 
$\chi_t:\A_t \to \A_t$ and of real valued functions  $L_t\in C^\infty(D_t)$ and $R_t^0\in C^\infty(\A_t)$  such that 
\begin{enumerate}
\item $(\varphi,I)\mapsto \langle\varphi, I\rangle -L_t(I) - R_t^0(\varphi,I)$ is a generating function of $P_t^0:= \chi_t^{-1}\circ P_t\circ \chi_t$;
\item $\nabla L_t: D_t \to \Omega$ is a diffeomorphism, $L_t=K_t$  outside $D_t^1:= \nabla K_t^\ast(\Omega-\kappa/2)$, and  $\nabla L_t^\ast(\omega)=I_t(\omega)$ is given by \eqref{eq:momentum-I} for each $\omega\in \Omega_{ \kappa}^0$;
\item $R_t^0$ is flat at $\T^{n-1}\times \nabla L_t( \Omega_{ \kappa}^0$; 
\end{enumerate}
\item[(ii)] For any $t\in [0,\delta]$ and $m\in N$ the following estimates hold
\begin{equation}\label{eq:estimates-chi}
\begin{array}{lcrr}
\|\sigma_\kappa^{-1}(\chi - {\rm id})\|_{m,\A_t;\kappa} + \|\sigma_\kappa^{-1}(\chi^{-1} - {\rm id})\|_{m,\A_t;\kappa}\\[0.3cm]
\displaystyle
\le \frac{C_m}{\varrho\kappa} \,  {\mathcal B}_{m+1} \lambda^{2m}  \big(\lambda +\|\partial^2 K_t\|_{m+1,D_t;\kappa}\big)
\end{array}
\end{equation}
and
\begin{equation}\label{eq:estimates}
\begin{array}{llcrr}
 \|\nabla L_t - \nabla K_t\|_{m,D_t;\kappa}   + \|\sigma_\kappa \nabla R_t^0\|_{m,D_t;\kappa}  \\[0.3cm]
 \le\,  \displaystyle \frac{C_m}{\varrho } \,  {\mathcal B}_{m+1}  \lambda^{2m}   \big(\lambda+\|\partial^2 K_t\|_{m+1,D_t; \kappa}\big)\,   , 
\end{array}
\end{equation}
where the constant $C_m>0$ depends only on $n$, $\tau$, $\vartheta_0$ and $m$.
\end{enumerate}
\end{Theorem}
Before proving the Theorem we observe that
\begin{Remark}\label{rem:inv-tori} (Birkhoff Normal Form) Let $k=1$. Then 
for any $\omega\in \Omega_\kappa^0$ the map 
\[
[0,\delta]\ni t\to \Lambda_t(\omega):=\chi_t(\T^{n-1}\times \{I_t(\omega)\})
\] 
provides  a $C^1$ family of invariant tori of $P_s$ with a frequency vector $\omega$ and taking into account Lemma \ref{Lemma:flat} we obtain
\[
P_t^0(\varphi,I)= (\varphi + \nabla L_t(I),I) + O_N(|I-\nabla L_t^\ast(\omega)|^N)
\] 
for any $N\in\N$ . Moreover,  the last formula can be differentiated $N-1$ times with respect to $(\varphi,I)$. Hence, Theorem \ref{Theo:BNF} gives a simultaneous Birkhoff Normal Form  of $P_t$ on the invariant tori $\Lambda_t(\omega)$, where $t\in [0,\delta]$ and the frequency vectors $\omega$ are in $\Omega_\kappa^0$. Recall as well that the complement of  $\Omega_\kappa^0$ in  $\Omega_\kappa$ is of Lebesgue measure zero. 
\end{Remark}
\noindent
{\em Proof of Theorem \ref{Theo:BNF}.} Without loss of generality we consider only the case when $k=1$. We devide the proof in several staps.\\ 


 
Denote by $p:{\R}^{n-1} \to  {\T}^{n-1}$ the natural
projection. 
\begin{Lemma}\label{Lemma:averaging}
There is a $C^1$ family of real-valued functions 
$h_t\in  C^\infty( {\R}^{n-1}\times \Omega)$ and 
$I_t\in   C^\infty(\Omega)$ in $t\in [0,\delta]$ such that 
$h_t^0(x,\omega):= h_t(x,\omega)-\langle x,I_t(\omega)\rangle$ is $1$-periodic with respect to $x$ and 
\begin{itemize}
\item[(i)] $\forall (x,\omega)\in{\R}^{n-1}\times \Omega_\kappa$, 
 $\nabla_x h_t(x,\omega)= \widetilde F_t(p(x),\omega)$,
\item[(ii)] $\nabla_x h_t^0(x,\omega) = 0$ and $I_t(\omega)=\nabla K_t^\ast(\omega)$ for $\omega\notin \Omega-\kappa/2$, 
\item[(iii)]   
$\displaystyle
 \|h_t^0\|_{m;\kappa}  \, +\, \|I_t - \nabla K_t^\ast\|_{m;\kappa} 
\, \le \,  \frac{C_m}{\varrho }   \, {\mathcal B}_m$
\end{itemize} 
for $m\in\N$ , where $C_m$ is a positive constant depending only on $n$, $\tau$, $\vartheta_0$ and $m$. 
\end{Lemma}
{\em Proof.}
To obtain $h_t$ we consider the function
$$ 
\widetilde h_t (x,\omega)\  =\  \int_{\gamma_x}^{}\, \sigma\ 
=\ \int_{0}^{1}\, \langle \widetilde F_t(p(sx),\omega),\, x\rangle\, ds\ =\ \langle \nabla K_t^\ast(\omega),x\rangle + \int_{0}^{1}\, \langle  F_t(p(sx),\omega),\, x\rangle\, ds\quad 
$$ 
for  $(x,\omega)\in {\R}^{n-1}\times \Omega$, 
where $\gamma_x = \{(sx, \widetilde  F_t(p(sx),\omega)): 0\leq s\leq 1\}$ and $\sigma =\xi dx$ is the canonical one-form on $T^\ast{\R}^{n-1}$. In view of 
\eqref{eq:derivatives-F},  the function 
$Q_t^0(x,\omega):=\widetilde h_t(x, \omega) - \langle \nabla K_t^\ast(\omega),x \rangle$
satisfies the 
estimate
\begin{equation}\label{eq:estimate-Q-0}
 \| Q_t^0\|_{m;\kappa} 
\, \le \,  \frac{C_m}{\varrho }   \, {\mathcal B}_m
\end{equation}
for  $m\in \N$.  We set 
\[
 I_{tj} (\omega) = \widetilde h_t( e_j,\omega), \quad \omega\in \Omega, 
\]
where 
$\{e_1,\ldots, e_{n-1}\}$ is the canonical  basis in ${\R}^{n-1}$. Then \eqref{eq:estimate-Q-0} implies
\begin{equation}\label{eq:estimate-I-K}
 \| I_t-\nabla K_t^\ast\|_{m;\kappa}
\, \le \,  \frac{C_m}{\varrho }   \, {\mathcal B}_m
\end{equation}
for $m\in \N$ and $t\in [0,\delta	]$.  

  
As $\Lambda_t(\omega)$ 
is a Lagrangian torus for $\omega\in \Omega_\kappa$, we get 
\begin{equation}\label{eq:integral-for-h}
\forall\, y\in {\R}^{n-1} ,  \quad \widetilde h_t (x+y,\omega) -\widetilde h_t(x,\omega)\ =\ 
\int_{l_t(x,y)}\, \sigma
\end{equation}
where $l_t(x,y) = \{(x+sy,\widetilde F_t(p(x+sy),\omega)):\, 0\leq s\leq 1\}$ and $\sigma$ is the pull-back to $\Lambda_t(\omega)$ of the fundamental one-form $Idx$.  The 
integral in \eqref{eq:integral-for-h} is equal to 
$$ 
\int_{l_t(x,y)}\, \sigma=\int_{0}^{1}\, \langle \widetilde  F_t(p(x+sy),\omega), y\rangle ds\ =\ 
\langle \widetilde F_t(p(x),\omega),y\rangle + O(y^2), 
$$ 
and we obtain  $\nabla_x \widetilde h(x,\omega)= \widetilde F_t(p(x),\omega)$  for any  $\omega\in \Omega_\kappa$. 
In particular, the function 
$\nabla_x \widetilde h_t(x,\omega)$ is $1$-periodic with
respect to $x$ and using \eqref{eq:integral-for-h} we get
\[
\forall\, \omega\in\Omega_\kappa,\ \forall\, m\in {\Z}^{n-1}, \quad \widetilde h_t (x+m,\omega) - \widetilde h_t (x,\omega) = \widetilde h_t (m,\omega) - \widetilde h_t (0,\omega)
=\langle m, I_t(\omega)\rangle.
\] 
Consider the function 
\[
\widetilde h_t^0(x,\omega) = 
\widetilde h_t(x,\omega) - \langle x, I_t(\omega) .
\]
It  is $1$-periodic with respect to
$x$ for $\omega\in \Omega_\kappa$ and $\widetilde h_t^0$ satisfies the  estimates \eqref{eq:estimate-Q-0} in 
$[0,\delta]\times \R^{n-1}\times \Omega$. 
We are going to average  $\widetilde h_t^0$ on ${\T}^{n-1}$ using the following 
\begin{Lemma}\label{Lemma:averaging function} There exists 
$f\in C^\infty({\R}^{n-1})$ with ${\rm supp}\, f \subset [\pi,
7\pi]^{n-1}$ such that 
\[
\sum_{k\in {\Z}^{n-1}} f(x -  2\pi k) = 1
\]
for each $x\in {\R}^{n-1}$. 
\end{Lemma}
Consider the function 
\[
h_t^0(x,\omega) =
\sum_{k\in {\Z}^{n-1}} (f \widetilde h_t^0)(x -  k,\omega).
\] 
It is $1$-periodic with respect to $x$ by
construction  and 
$h_t^0(x,\omega) = \widetilde h_t^0(x,\omega)$ for $(x,\omega)\in 
{\R}^{n-1}\times \Omega_\kappa$.
Moreover,  $h_t^0$ satisfies \eqref{eq:estimate-Q-0} in 
$[0,\delta]\times\R^{n-1}\times \Omega$.  
 We set
\[
h_t(x,\omega)=h_t^0(x,\omega) + \langle x, I_t(\omega)\rangle .
\] 
Recall that  
\[
\mbox{dist}\, (\Omega_\kappa, {\R}^{n-1}\setminus
\Omega) \ge  \kappa. 
\]
Then multiplying $h_t^0$ and $I_t- \nabla K_t^\ast$ by
a suitable 
cut-off function  which is equal to  one on 
$\Omega-3\kappa/4$ and zero outside $\Omega-\kappa/2$, we can
assume that $h_t(x,\omega) =  \langle x, \nabla K_t^\ast(\omega)\rangle$ and $I_t(\omega) = \nabla K_t^\ast(\omega)$ outside $\Omega-\kappa/2$  (see Lemma \ref{lemma:cut-off-omega}). This proves $(ii)$.  The statement $(iii)$ follows from \eqref{eq:estimate-Q-0}, the definition of $h_t^0$ and \eqref{eq:estimate-I-K}.\finishproof
\\


\noindent
{\em Step 2. Inverting $I_t$.}
\begin{Lemma}\label{Lemma:action} Choosing $\epsilon=\epsilon(n,\tau,\vartheta_0)>0$ small enough one has  the following for each $t\in [0,\delta]$. 
\begin{enumerate}
\item The map $I_t:\Omega \rightarrow D_t$ is a diffeomorphism  and its inverse $\omega_t: D_t\to \Omega$ satisfies the estimates 
$\|\omega_t -\nabla K_t\|_{1,D_t;\kappa} \le C_0\epsilon\kappa$ and 
\begin{equation}\label{eq:omega}
 \| \omega_t -\nabla K_t\|_{m, D_t;\kappa}\, 
 \le \,  \frac{C_m}{\varrho}  \,{\mathcal B}_{m} \lambda^{m}\big(\lambda+\|\partial^2 K_t\|_{m,D_t;\kappa}\big)
\end{equation}
for any $m\in\N_\ast$. Moreover, $\omega_t=\nabla K_t$ outside the set $\overline D_t^1:= \nabla K_t^\ast(\Omega-\kappa/2)$. 
\item For any $x\in \R^{n-1}$ the map $\Omega\ni\omega\rightarrow \nabla_x h_t(x,\omega)\in D_t$ is a diffeomorphism.
\end{enumerate}
\end{Lemma}
{\em Proof}. We are going to show that the map $\Omega\ni \omega\to I_t(\omega)$ a diffeomorphism. To this end we write
\[
I_t = ({\rm id} +\varphi_t)\circ \nabla K_t^\ast,\quad \varphi_t:= (I_t -\nabla K_t^\ast)\circ \nabla K_t.
\]
Moreover, Lemma \ref{Lemma:averaging}, \eqref{eq:non-degeneracy-BNF} and  \eqref{eq:smallness-condition-1} imply
\[
\|\varphi_t\|_{C^1} \le \|I_t -\nabla K_t^\ast\|_{C^1}(1+\|\nabla K_t\|_{C^1}) \le C_1 \epsilon \lambda^{-2}
\]
where $C=C(n,\tau,\vartheta_0)>0$. Recall that $I_t=\nabla K_t^\ast$ outside $\Omega-\kappa/2$, hence ${\rm supp\,}\varphi_t\subset D_t$. Then choosing $0<\epsilon<1/(2C)$ and  applying Proposition \ref{prop:inverse-holder1} we obtain that ${\rm id} +\varphi_t:\R^{n-1}\to \R^{n-1}$ is invertible and that
$({\rm id} +\varphi_t)^{-1} ={\rm id} +\psi_t$, where ${\rm supp\,}\psi_t\subset D_t$. Hence, $I_t(\Omega)= D_t$ and 
 $I_t:\Omega\to D_t$ is a diffeomorphism with inverse 
 \[
 \omega_t=\nabla K_t\circ ({\rm id} +\psi_t):D_t\to \Omega.
 \]
\begin{Lemma}\label{Lemma:estimates-phi} 
For any $m\in\N_\ast$ there exists $C_m>0$ depending only on $m$, $n$, $\tau$ and $\vartheta_0$ such that
\[
\|\varphi_t\|_{m,\kappa} \le \frac{C_m}{\varrho}  \,{\mathcal B}_{m}  \lambda^{m-1}   \big(\lambda+\|\partial^2 K_t\|_{m-1,D_t;\kappa}\big). 
\]
\end{Lemma}
{\em Proof}. The support of $\varphi_t$ is contained in the closure of  $D_t^1:= \nabla K_t^\ast (\Omega-\kappa/2)$. Set $2r_t:= {\rm dist}\, (D_t^1, \R^{n-1}\setminus D_t)$ and fix $I^0$ in $\overline D_t^1$. Applying Remark \ref{rem:interpolation} to the restriction of $K_t$ to the closed ball 
$\overline B(I^0, r_t)$ as well as the  Proposition \ref{prop:composition-holder1}, {\em 2},    \eqref{eq:non-degeneracy-BNF} and  \eqref{eq:smallness-condition-1} one obtains 
\[
\begin{array}{cclr}
\displaystyle |\partial_\theta^\alpha(\kappa\partial_I)^\beta\varphi_t(\theta,I)|\le 
 C_m^\prime\left(1+ \|\partial^2 K_t\|_{C^0(D_t)}^{m-1}\right) \\[0.3cm]
\displaystyle \times \left(\|I_t -\nabla K_t^\ast\|_{m,\kappa}\| \partial^2 K_t\|_{{C^0(D_t)}}+\|I_t -\nabla K_t^\ast\|_{C^1}\|\partial^2 K_t\|_{m-1,D_t;\kappa}\right)\\[0.3cm]
\displaystyle \le \frac{C_m}{\varrho}  \,{\mathcal B}_{m}   \lambda^{m-1}   \big(\lambda+\| \partial^2 K_t\|_{m-1,D_t;\kappa}\big),
\end{array} 
\]
for $(\theta,I,t)\in \T^{n-1}\times B(I^0, r_t)\times [0,\delta]$ and $\alpha,\beta\in \N^{n-1}$, $|\alpha|+ |\beta|=m\in\N_\ast$, 
where $C_m^\prime>0$ depends only on $m$ and $n$ and $C_m>0$ depends only on $m$, $n$, $\tau$ and $\vartheta_0$. 
On the other hand, $\varphi_t=0$ outside $D_t^1$ which completes the proof of the Lemma. This argument will be used many times in the sequel.
\finishproof

\noindent
Proposition \ref{prop:inverse-holder1} applied to ${\rm id} + \kappa^{-1}\varphi_t \circ\sigma_\kappa$  implies that ${\rm supp}\, \psi_t\subset \overline D_t^1$, $\|\psi_t\|_{C^0}\le C_0\epsilon/\lambda$  and 
\[
\|\psi_t\|_{m,\kappa} \le \frac{C_m}{\varrho}  \,{\mathcal B}_{m}   \lambda^{m-1}  \big(\lambda+\|\partial^2 K_t\|_{m-1,D_t;\kappa}\big)
\]
for $m\in\N^\ast$. In particular, $\|d \psi_t\|_{C^0} \le C_1\epsilon$. 
Consider
\[
\omega_t(I) -\nabla K_t(I) = \int_0^1   d(\nabla K_t)(I + s\psi_t(I)) \,  \psi_t(I)\,  ds, \quad I\in D_t. 
\]
The support of $\omega_t -\nabla K_t$ is contained in $\overline D_t^1$. Moreover, $|\omega_t -\nabla K_t\|_{C^0(D_t)} \le C_0\epsilon\kappa$ and 
arguing as in the proof of Lemma \ref{Lemma:estimates-phi}
one obtains for any $m\in \N_\ast$ and $\alpha\in\N^{n-1}$ with $|\alpha|=m$ the estimate
\[
\begin{array}{cclr}
\displaystyle
\|(\kappa \partial)^\alpha(\omega_t -\nabla K_t)\|_{C^0} \le C_m \|\partial^2 K_t\|_{C^0(D_t)}\|\psi_t\|_{m,\kappa} \\[0.3cm]
\displaystyle +\,  C_m\|\psi_t\|_{C^0}\big(1+ \|d \psi_t\|_{C^0}^{m-1}\big)\big(\|\partial^2 K_t\|_{1,D_t;\kappa}\|d\psi_t\|_{m-1,\kappa} +
\|\partial^2 K_t\|_{m,D_t;\kappa}\|d\psi_t\|_{C^0(D_t)}\big).
\end{array}
\]
Then 
using \eqref{eq:non-degeneracy-BNF}, \eqref{eq:smallness-condition-1} and the previous estimates we obtain \eqref{eq:omega}. The estimate  
$\|d\omega_t- d\nabla K_t\|_{C^0(D_t)} \le C \epsilon\lambda$ follows from \eqref{eq:omega} with $m=1$ and \eqref{eq:smallness-condition-1}. 
We are going to prove that for each $x\in \R^{n-1}$ the map $\Omega\ni\omega\rightarrow \nabla_x h_t(x,\omega)$ is a diffeomorphism. 
To this end we fix $x$ and we write the map $\omega\to \nabla_x h_t(x,\omega)$ as follows 
\[
\nabla_x h_t= ({\rm id} +\varphi_t^1)\circ \nabla K_t^\ast, \quad
\varphi_t^1:= (\nabla_x h_t^0 + I_t -\nabla K_t^\ast)\circ \nabla K_t .
\]
Then ${\rm supp\,}\varphi_t^1\subset \overline D_t^1$  and 
\[
\|\varphi_t^1\|_{C^1} \le (\|\nabla_x h_t^0\|_{C^1}+\|I_t -\nabla K_t^\ast\|_{C^1})(1+\|\partial^2 K_t\|_{C^0}) \le C_1 \epsilon/\lambda
\]
and we complete the proof of {\em 2} as above. 
\finishproof
\\


\noindent
{\em Step 3. Construction of $\chi_t$.}\quad 
The second statement of the Lemma implies that there is 
a $C^\infty$-foliation of ${\T}^{n-1}\times D_t$ 
by  Lagrangian tori 
\[
\Lambda_t(\omega)\ =\ \{(p(x),\nabla_x h_t(x,\omega)) :\, 
x\in{\R}^{n-1}\},\ \omega\in \Omega
\]
which is a smooth extension of the family of the Kronecker invariant  tori \eqref{eq:kam-tori-F} of $P_t$. 
Notice that  $I_t(\omega)$ is the action along the basis of cycles $[\gamma_{t,j}(\omega)], \ldots, [\gamma_{t,n-1}(\omega)]$ of   $H_1(\Lambda_t(\omega),\R)$, where $\gamma_{t,j}(\omega) = 
\{(p(se_j),\, \nabla_x h_t(se_j,\omega))\, :\, 
0\leq s\leq 1\}$. Indeed, it follows from the definition of $h_t$ that $I_t(\omega)=\nabla_x h_t(x,\omega)-\nabla_x h_t^0(x,\omega)$, where $h_t^0$ is $1$-periodic in $x$ and we obtain
\begin{equation}\label{eq:momentum-I-2}
I_{t}(\omega)\ =\ \left(\int_{\gamma_{t,1}(\omega)}\, \sigma ,\ldots, \int_{\gamma_{t,n-1}(\omega)}\, \sigma \right)
\end{equation}
for  $\omega\in \Omega$.   
Now we set $\Phi_t(x,I) = h_t(x,\omega_t(I))$. Then  
\[
\Phi^0_t(x,I):=\langle x, I\rangle -\Phi_t(x,I)  = - h^0_t(x,\omega_t(I))
\]
is $1$-periodic with
respect to $x$, and  it has a compact support in $\T^{n-1}\times D_t$. Moreover, it follows from Lemma \ref{Lemma:averaging},  Lemma \ref{Lemma:action}, Remark \ref{rem:interpolation} and Proposition \ref{prop:composition-holder-interpolation} that
\[
\begin{array}{lcrr}
\|\Phi^0_t\|_{m,\A_t;\kappa}\, 
\le \, C_m \left(1+ \|d \omega_t\|_{C^0(D_t)}^{m-1} \right) \Big(\|h_t^0\|_{m,\kappa}\|d \omega_t\|_{C^0(D_t)}\\[0.3cm]
\displaystyle
  + \|h_t^0\|_{1,\kappa}\|\partial^2 K_t\|_{m-1,D_t;\kappa}+ \|h_t^0\|_{1,\kappa}\|(d \omega_t- d\nabla K_t)\|_{m-1,D_t;\kappa}\Big) \\[0.3cm]
\displaystyle
\le \frac{C_m}{\varrho}  \,{\mathcal B}_{m}  \lambda^{2m-2}  \big(\lambda +\|\partial^2 K_t\|_{m,D_t;\kappa}\big)
\end{array}
\]
for  $t\in [0,\delta]$ and  $m\in\N_\ast$, where $C_m$ depends only on $m$, $n$, $\tau$ and $\vartheta_0$. This implies 
\begin{equation}\label{eq:estimates-Phi-0}
\|\sigma_\kappa^{-1}{\rm sgrad}\Phi^0_t\|_{m,\A_t;\kappa}\, 
\le \,  \frac{C_m}{\kappa\varrho}  \,{\mathcal B}_{m+1}  \lambda^{2m}  \big(\lambda +\|\partial^2 K_t\|_{m+1,D_t;\kappa}\big)
\end{equation}
for  $t\in [0,\delta]$ and  $m\in\N$, where $C_m$ depends only on $m$, $n$, $\tau$ and $\vartheta_0$.
In particular, one obtains by means of \eqref{eq:non-degeneracy-BNF} and \eqref{eq:smallness-condition-1} that
\begin{equation}\label{eq:estimates-Phi-0-2}
\|\sigma_\kappa^{-1}{\rm sgrad}\, \Phi^0_t\|_{1,\A_t;\kappa}  \le c\epsilon/\lambda  
\end{equation}
for $t\in [0,\delta]$, where $c=c(n,\tau,\vartheta_0)>0$. Using  Lemma \ref{lemma:generating-functions} we obtain
\begin{Lemma}\label{Lemma:chi} Choosing $\epsilon=\epsilon(n,\tau,\vartheta_0)>0$ small enough we have the following
\begin{enumerate}
\item $\Phi_t$ is a generating function of a symplectic transformation $\chi_t:\T^{n-1}\times D_t \to \T^{n-1}\times D_t$ and the map $[0,\delta]\ni t\to \chi_t\in C^\infty(\A_t,\A_t)$ is $C^1$; 
\item $\chi_t(\Lambda_t(\omega))=\T^{n-1}\times \{I_t(\omega)\}$ for any  $\omega\in \Omega$ and $t\in [0,\delta]$;
\item $\chi_t-{\rm id}$ and $\chi_t^{-1}-{\rm id}$ are compactly supported in $\T^{n-1}\times \overline D_t^1$, where $D_t^1=\nabla K_t^\ast(\Omega-\kappa/2)$ and they satisfy the estimates \eqref{eq:estimates-chi}. Moreover,
\[
\|\sigma_\kappa^{-1}(\chi -{\rm id})\|_{1,\A_t;\kappa} + \|\sigma_\kappa^{-1}(\chi -{\rm id})\|_{1,\A_t;\kappa} \, \le\,   c\epsilon/\lambda  . 
\] 
\end{enumerate}
\end{Lemma}
{\em Proof}. Using  Lemma \ref{lemma:generating-functions}  one  
obtains a symplectic transformation $\chi_t: {\T}^{n-1}\times D_t\to {\T}^{n-1}\times \R^{n-1}$ defined  by 
\[
\chi_t(\nabla_I\Phi_t(\theta,I), I)= (\theta, \nabla_\theta\Phi_t(\theta,I)), \quad (\theta,I)\in  {\T}^{n-1}\times \R^{n-1}. 
\]
Notice that the map
\[
D_t \ni I \to \nabla_\theta\Phi_t(\theta,I)= I + \nabla_\theta h_t^0(\theta,\omega_t(I))\in D_t
\] 
is a diffeomorphism since the map 
$\Omega \ni \omega \to I_t(\omega) + \nabla_\theta h_t^0(\theta,\omega)= \nabla_\theta h_t(\theta,\omega)\in D_t$ is a diffeomorphism in view of Lemma \ref{Lemma:action}, {\em 2}, hence,  $\chi_t(\A_t)=\A_t$. 
For any $\omega\in
\Omega$ and any $\theta$ we
have 
\[
(\theta, \nabla h_t(\theta,\omega)) = (\theta, \nabla_\theta\Phi_t(\theta,I_t(\omega)))
= \chi_t(\nabla_I\Phi_t(\theta,I_t(\omega)), I_t(\omega)).
\] 
hence, $\Lambda_t(\omega) =
\chi_t({\T}^{n-1}\times \{I_t(\omega)\})$. Moreover,  $\chi_t(\varphi, I_t(\omega))= (\varphi, I_t(\omega))= (\varphi,\nabla K_t^\ast(\omega))$ if  $\mbox{dist}\, (\omega, {\R}^{n-1}\setminus \Omega) \le \kappa/2$, hence, the support of both $\chi_t-{\rm id}$ and  $\chi_t^{-1}-{\rm id}$ is contained in $\T^{n-1}\times \overline D_t^1$. The estimate    \eqref{eq:estimates-chi} follows from \eqref{eq:estimates-Phi-0} and Lemma \ref{lemma:generating-functions}. 
\finishproof
\\


\noindent
{\em Step 4. Estimates.}\quad 
Consider the exact symplectic map $P_t^0 = \chi_t^{-1} P_t\chi_t$. Using Lemma \ref{Lemma:decomposition} we write $P_t$ in as the  composition $P_t=W_t Q_t$, where $W_t$ is the exact symplectic map defined by the  generating function $(x,r)\to \langle x, r\rangle - G_t(x,r)$ and $Q_t(\theta,r)=(\theta +\nabla K(r),r)$. 
Then  
\[
P_t^0 = W_t^1 Q_t,
\] 
where  
\[
W_t^0 = \chi_t^{-1} W_t + \chi_t^{-1} W_t Q_t (\chi_t^{-1} - {\rm id}) Q_t^{-1}.
\]
\begin{Lemma}\label{Lemma:W-1} The exact symplectic map $W_t^1$, $t\in [0,\delta]$,  admits a generating function of the form 
\[
(x,I) \to \langle x, I\rangle - G_t^1(x,I)
\]
 such that the map $[0,\delta]\ni t \to G_t^1\in C^\infty(\A)$ is $C^1$, ${\rm supp}\, (dG_t^1) \subset \T^{n-1}\times \overline D_t^1$ and 
\[
\|\sigma_\kappa^{-1}{\rm sgrad}\, G^1_t\|_{m,\A_t;\kappa} \, \le\,  
\frac{C_m}{\varrho\kappa } \,{\mathcal B}_{m+1}  \lambda^{2m} \big(\lambda+\|\partial^2 K_t\|_{m+1,D_t;\kappa}\big)
\]
for any $m\in\N$, where  $C_m$ depends only on $m$, $n$, $\tau$ and $\vartheta_0$.
\end{Lemma}
{\em Proof}. 
We have 
\begin{equation}\label{eq:identity-for-W-1}
\begin{array}{lcrr}
W_t^1 - {\rm id}\,  =\,  \big(W_t - {\rm id} + (\chi_t^{-1}- {\rm id}) W_t\big)\, +\, \big( Q_t(\chi_t- {\rm id})Q_t^{-1}\big) \\[0.3cm]
+ \big( W_t - {\rm id} + (\chi_t^{-1}- {\rm id}) W_t\big)\, \circ\, \big(Q_t(\chi_t- {\rm id})Q_t^{-1}\big).
\end{array}
\end{equation}
We estimate the $C^m$ norms of it term by term. 
Notice that the support of each term is contained in $\T^{n-1}\times \overline D_t^1$. 

Lemma \ref{lemma:generating-functions} and \eqref{eq:smallness-condition-1} imply $\|\sigma_\kappa^{-1}(W_t - {\rm id})\|_{1,\A_t;\kappa}< C\epsilon/\lambda$ and 
\[
\|\sigma_\kappa^{-1}(W_t - {\rm id})\|_{m,\A_t;\kappa}\, \le\,  \frac{C_m}{\varrho\kappa}  \,{\mathcal B}_{m}  . 
\]
The last estimate, Lemma \ref{Lemma:chi}, {\em 3}, and Lemma \ref{prop:composition-holder1}, {\em 2}, imply
\[
\|\sigma_\kappa^{-1}(\chi_t^{-1}- {\rm id}) W_t\|_{m,\A_t;\kappa}\, \le\,  
\frac{C_m}{\varrho\kappa }  \,{\mathcal B}_{m+1} \lambda^{2m} \big(\lambda+\|\partial^2 K_t\|_{m+1,D_t;\kappa}\big).   
\]
and 
\[
\|\sigma_\kappa^{-1}(\chi^{-1} -{\rm id})W_t\|_{1,\A_t;\kappa}  \, \le\,   c\epsilon/\lambda  . 
\] 
Using the argument in the proof of Lemma \ref{Lemma:estimates-phi} first to $ (\chi_t- {\rm id})Q_t^{-1}$ and then to  $Q_t(\chi_t- {\rm id})Q_t^{-1}$ we obtain the estimate
\[
\|\sigma_\kappa^{-1}Q_t(\chi_t- {\rm id})Q_t^{-1}\|_{m,\A_t;\kappa}\, \le\,  
\frac{C_m}{\varrho\kappa } \,{\mathcal B}_{m+1} \lambda^{2m}\big(\lambda+\|\partial^2 K_t\|_{m+1,D_t;\kappa}\big) .  
\]
This yields the  estimate of the first line of \eqref{eq:identity-for-W-1}. To obtain the estimates for the composition in the second line one uses the preceding estimates and the argument of Lemma \ref{Lemma:estimates-phi}. It remains to apply Lemma \ref{lemma:generating-functions} in order to complete  the proof of the Lemma.  \finishproof
\\

\noindent
{\em Step 4. Proof of $(i)$.}\quad  
Now Lemma \ref{Lemma:decomposition} implies that the function $\widetilde G^0_t(x,I)= \langle x, I\rangle -  K_t(I) - G_t^1(\varphi,I)$ is a generating function of $P_t^0$. The function  $\widetilde G^0_t$ is uniquely defined modulo a constant depending only on $t$ which is chosen  appropriately in order to obtain a $C^1$-smooth  the map $t\to \widetilde G^0_t$. Set $L_t(I):= K_t(I)- G^1_t(0, I)$ and $R_t(\theta, I)= G^1_t(\theta, I)- G^1_t(0, I)$. We have 
\[
P_t^0({\T}^{n-1}\times \{I_t(\omega)\}) = (\chi_t^{-1}\circ P_t) (\Lambda_t(\omega))= \chi_t^{-1}(\Lambda_t(\omega))= {\T}^{n-1}\times \{I_t(\omega)\}
\]
for any $\omega\in \Omega_\kappa$, which implies 
\[
I_t(\omega) - \nabla_x R_t^0(x,I_t(\omega))= \nabla_x \widetilde G_t^0(x,I_t(\omega))=I_t(\omega)
\]
for any such $x\in\R^{n-1}$. On the other hand, $R_t^0(0,I)=0$, hence, $R_t^0(\theta,I)=0$ on ${\T}^{n-1}\times E_{t,\kappa}$, where  $E_{t,\kappa}:= I_t(\Omega_\kappa)$. 
Now Lemma \ref{Lemma:flat} implies that $\partial_I^\beta R_t^0(\theta,I)=0$ for any  $(\theta, I)\in {\T}^{n-1}\times E_{t,\kappa}^0$, where  $E_{t,\kappa}^0:= I_t(\Omega_\kappa^0)$ is the set of points of   positive Lebesgue density in $E_{t,\kappa}$. 
Now $P_t^0(\theta + \nabla L_t(I), I)= (\theta,I)$ on ${\T}^{n-1}\times E_{t,\kappa}^0$, and we obtain that $\nabla_I L_t(I_t(\omega))=\omega$ for each $\omega\in  \Omega_{\kappa}^0$.  Then $\nabla L_t^\ast(\omega)= I_t(\omega)$ for each $\omega\in  \Omega_{\kappa}^0$ and it satisfies  \eqref{eq:momentum-I} according to \eqref{eq:momentum-I-2}.  
The estimates of the derivatives of $L_t$ and $R_t^0$ follow from that of Lemma \ref{Lemma:W-1}. 
\finishproof


